On Extremal Problems Associated with Random Chords on a Circle

Inspired by the work of Karamata, we consider an extremization problem associated with the probability of intersecting two random chords inside a circle of radius $r, \, r \in (0,1]$, where the endpoints of the chords are drawn according to a given probability distribution on $\mathbb{S}^1$. We show that, for $r=1,$ the problem is degenerated in the sense that any continuous measure is an extremiser, and that, for $r$ sufficiently close to $1,$ the desired maximal value is strictly below the one for $r=1$ by a polynomial factor in $1-r.$ Finally, we prove, by considering the auxiliary problem of drawing a single random chord, that the desired maximum is $1/4$ for $r \in (0,1/2).$ Connections with other variational problems and energy minimization problems are also presented.

==> Bibliography/karamata.tex <==
%------------------------------------------------------------------------------%
%
% Bibliography pasted from paperpile
%
%------------------------------------------------------------------------------%

@INCOLLECTION{Karamata1962-ec,
title = "{On the Distribution of Intersections of Diagonals in Regular Polygons}",
booktitle = "{Studies in Mathematical Analysis and Related Topics: Essays in Honor of George Pólya}",
author = "Karamata, Jovan",
publisher = "Stanford University Press",
pages = "170--174",
year =  1962
}


%------------------------------------------------------------------------------%


==> To-do <==
We need: 

1. To include a discussion on the reduced problem (maximising probability that chord intersects disk of radius r) for r slightly larger than 1/2; (DONE)

2. Expand on the discussion to why our results need to be slightly different when compared to the ones by Bylik and others; 

3. Compute (in light of the other articles) expected value of the distance between chord and origin, using classical stuff; 

4. At end of Section 3: the result is, as a matter of fact, continuous! That is, if we have a pure point measure \mu such that its close to being continuous (in the sense that its atoms are all 'small'), then the probability of intersections being inside the unit disk is 'almost' 1/3. A stability result (i.e., probability of intersections inside the unit disk close to 1/3 implies close to being continuous) probably holds as well. It is interesting and important to add these findings! (DONE)

5. Prove that, as r approaches 1, there is an upper bound like 1/3 - c \cdot r^a, for some a constant strictly larger than 0, on the maximum. (DONE)

==> tikz-euclide/drawings/tkz-draw-eu-angles.tex <==
% tkz-tool-eu-angles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tool-eu-angles.tex} 
\makeatletter
%<--------------------------------------------------------------------------–>
%                    tkzSetUpArc  
%<--------------------------------------------------------------------------–>
\pgfkeys{/tkzsetuparc/.cd,
   color/.store in        =    \tkz@arc@color,
   line width/.store in   =    \tkz@arc@lw,
   style/.store in        =    \tkz@arc@style,
   line width             =    \tkz@euc@linewidth,
   color                  =    \tkz@euc@linecolor,
   style                  =    \tkz@euc@linestyle,
   /tkzsetuparc/.search also = {/tikz,/tkzcompass},
 } 
\def\tkzSetUpArc{\pgfutil@ifnextchar[{\tkz@SetUpArc}{\tkz@SetUpArc[]}}
\def\tkz@SetUpArc[#1]{%
\pgfqkeys{/tkzsetuparc}{#1}
\tikzset{arc style/.style={color          = \tkz@arc@color,
                           line width     = \tkz@arc@lw,
                           style          = \tkz@arc@style
                           }}
}% end setup 
%<------------------------------  Arcs -------------------------------------–
% options : delta 
% \def\tkz@delta{0}
% \tikzset{arc style/.style={#1}}
% \pgfkeys{/tikz/.cd,delta/.code={\def\tkz@delta{#1}}}
\newif\iftkz@reverse
\gdef\tkz@numa{0}
\pgfkeys{/tkzdrawarc/.cd,
      type/.is choice,
      type/towards/.code               = \def\tkz@numa{0},
      type/rotate/.code                = \def\tkz@numa{1},
      type/angles/.code                = \def\tkz@numa{2}, 
      type/R/.code                     = \def\tkz@numa{3},
      type/R with nodes/.code          = \def\tkz@numa{4},
      towards/.style                   = {type=towards},
      rotate/.style                    = {type=rotate},
      R/.style                         = {type=R},
      angles/.style                    = {type=angles},
      R with nodes/.style              = {type=R with nodes},
      diameter/.code                   = {},
      arc/.code                        = {},
      size/.code                       = {},
      mark/.code                       = {},
      mkpos/.code                      = {},
      mksize/.code                     = {},
      mkcolor/.code                    = {},
      type/.default                    =  towards,
      delta/.store in                  = \tkz@delta,
      delta                            = 0,
      reverse/.is if                   = tkz@reverse,
      reverse/.default                 = true,
      reverse                          = false,
      /tkzdrawarc/.search also         = {/tikz}
}  
\def\tkzDrawArc{\pgfutil@ifnextchar[{\tkz@DrawArc}{\tkz@DrawArc[]}}
\def\tkz@DrawArc[#1](#2,#3)(#4){% 
\begingroup    
\pgfqkeys{/tkzdrawarc}{#1} 
\ifcase\tkz@numa%
   \tkzDrawArcTowards[#1](#2,#3)(#4)  
\or% 1
   \tkzDrawArcRotate[#1](#2,#3)(#4)  
\or% 2
   \tkzDrawArcAngles[#1](#2,#3)(#4) 
\or% 3
   \tkzDrawArcRAngles[#1](#2,#3)(#4)
\or% 4
   \tkzDrawArcR[#1](#2,#3)(#4)  
\fi    
\endgroup
}
%<--------------------------------------------------------------------------–>
%  ARC    nodes        #2 center #3 first point last point #4
% delta un peu plus à chaque extrémité 
% example : \tkzDrawArc(A,B)(C)      
%<--------------------------------------------------------------------------–>
\def\tkzDrawArcTowards{\pgfutil@ifnextchar[{\tkz@DrawArcN}{\tkz@DrawArcN[]}} 
\def\tkz@DrawArcN[#1](#2,#3)(#4){%
\begingroup
  \tkz@@CalcLengthcm(#2,#3){tkz@radius}
  \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstAngle}  
  \tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@SecondAngle}
  \tkz@DrawArcRAngles[#1](#2,\tkz@radius)(\tkz@FirstAngle,\tkz@SecondAngle) 
\endgroup
} 
%<--------------------------------------------------------------------------–>
%    nodes                 #2 center #3 first point rotate #4 with Angle
% delta un peu plus à chaque extrémité 
% tkzDrawArcRotate(O,A)(60)
%<--------------------------------------------------------------------------–>
\def\tkzDrawArcRotate{\pgfutil@ifnextchar[{\tkz@DrawArcRotate}{%
                                           \tkz@DrawArcRotate[]}}  
\def\tkz@DrawArcRotate[#1](#2,#3)(#4){%
\begingroup
  \tkz@@CalcLength(#2,#3){tkz@radius} 
  \tkzFindSlopeAngle(#2,#3)   \tkzGetAngle{tkz@FirstA}
  \pgfmathadd{\tkz@FirstA}{#4}
  \edef\tkz@SecondA{\pgfmathresult}
    \pgfmathgreaterthan{#4}{0}
  \ifdim\pgfmathresult pt=1 pt\relax%
    \tkz@DrawArcRAngles[#1](#2,\tkz@radius pt)(\tkz@FirstA,\tkz@SecondA)
  \else
    \tkz@DrawArcRAngles[#1](#2,\tkz@radius pt)(\tkz@SecondA,\tkz@FirstA)
  \fi
  \endgroup
}   
%<--------------------------------------------------------------------------–>
%  deux angles 
% \tkzDrawArcAngles(O,A)(0,60)
%<--------------------------------------------------------------------------–>
\def\tkzDrawArcAngles{\pgfutil@ifnextchar[{\tkz@DrawArcAngles}{%
                                           \tkz@DrawArcAngles[]}}  
\def\tkz@DrawArcAngles[#1](#2,#3)(#4,#5){%
\begingroup
    \tkz@@CalcLength(#2,#3){tkzLengthResult}
    \tkz@DrawArcRAngles[#1](#2,\tkzLengthResult pt)(#4,#5)      
\endgroup
}   
%<--------------------------------------------------------------------------–>
%    Degree      #2 center #4 - #3 radius from #5 (degree) to #6(degree) 
%<--------------------------------------------------------------------------–>
\def\tkzDrawArcRwithNodes{\pgfutil@ifnextchar[{\tkz@DrawArcRwithNodes}{%
                                            \tkz@DrawArcRwithNodes[]}}  
\def\tkz@DrawArcRwithNodes[#1](#2,#3,#4)(#5,#6){%
\begingroup
  \tkz@@CalcLength(#3,#4){tkzLengthResult}  
  \tkzFindSlopeAngle(#2,#5)\tkzGetAngle{tkz@FirstAngle}  
  \tkzFindSlopeAngle(#2,#6)\tkzGetAngle{tkz@SecondAngle}
  \tkz@DrawArcRAngles[#1](#2,\tkzLengthResult)(\tkz@FirstAngle,\tkz@SecondAngle)
\endgroup   
} 
%<--------------------------------------------------------------------------–>
%    Nodes R  #2 center #3 radius en cm  from #4(node) to #5(node)
%  \tkzDrawArcR(O,2)(A,B)
%<--------------------------------------------------------------------------–>
\def\tkzDrawArcR{\pgfutil@ifnextchar[{\tkz@DrawArcR}{\tkz@DrawArcR[]}} 
\def\tkz@DrawArcR[#1](#2,#3)(#4,#5){%
\begingroup
   \tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@FirstAngle}  
   \tkzFindSlopeAngle(#2,#5)\tkzGetAngle{tkz@SecondAngle} 
   \tkz@DrawArcRAngles[#1](#2,#3)(\tkz@FirstAngle,\tkz@SecondAngle)  
\endgroup   
}
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% #1 center #2 radius #4 first angle (degree) #5 second angle  (degree)  
% angles  0 .. 180 or -180 .. 0
%<--------------------------------------------------------------------------–>
% example : \tkzDrawArc(A,2)(30,90)    
\def\tkzDrawArcRAngles{\pgfutil@ifnextchar[{\tkz@DrawArcRAngles}{%
                                            \tkz@DrawArcRAngles[]}} 
\def\tkz@DrawArcRAngles[#1](#2,#3)(#4,#5){% 
 \begingroup
 \tkzNormalizeAngle(#4,#5)    
 \pgfmathsubtract{\tkz@FirstAngle}{\tkz@delta}
 \edef\tkz@FirstAngle{\pgfmathresult}%
 \pgfmathadd{\tkz@SecondAngle}{\tkz@delta}
 \edef\tkz@SecondAngle{\pgfmathresult} 
 \iftkz@reverse 
   \let\tkztemp\tkz@FirstAngle 
   \let\tkz@FirstAngle\tkz@SecondAngle
   \let\tkz@SecondAngle\tkztemp
  \fi
  \draw[shift = {(#2)},arc style,/tkzdrawarc/.cd,#1]%
  (\tkz@FirstAngle:#3) arc (\tkz@FirstAngle:\tkz@SecondAngle:#3);
\endgroup  
}
%<--------------------------------------------------------------------------–>
\pgfkeys{
  /@tkzmarkarc/.cd,
     pos/.store in       = \tkz@mkarcpos,
     color/.store in     = \tkz@mkcolor,
     mark/.store in      = \tkz@markarcseg,
     size/.store in      = \tkz@mkarcsize,
     color               = teal!20,
     size                = 4pt,
     pos                 = .5,
     mark                = none,
    /@tkzmarkarc/.search also={/tikz},
}
\def\tkzMarkArc{\pgfutil@ifnextchar[{\tkz@MarkArc}{\tkz@MarkArc[]}}   
\def\tkz@MarkArc[#1](#2,#3,#4){% 
\begingroup
 \pgfqkeys{/@tkzmarkarc}{#1} \def\tkz@mymarkarc{\pgfsetplotmarksize{\tkz@mkarcsize}\pgfuseplotmark{\tkz@markarcseg}}
\tkz@@CalcLength(#2,#3){tkz@radius}
\tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstAngle}  
\tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@SecondAngle}
\tkzNormalizeAngle(\tkz@FirstAngle,\tkz@SecondAngle)
 \pgfmathsubtract{\tkz@FirstAngle}{\tkz@delta}
 \edef\tkz@FirstAngle{\pgfmathresult}%
 \pgfmathadd{\tkz@SecondAngle}{\tkz@delta}
 \edef\tkz@SecondAngle{\pgfmathresult} 
\begin{scope}[decoration={markings,mark=at position \tkz@mkarcpos with {\tkz@mymarkarc}}]     
\path[shift = {(#2)},\tkz@mkcolor,/@tkzmarkarc/.cd,#1,postaction={decorate}]%
(\tkz@FirstAngle:\tkz@radius pt) arc (\tkz@FirstAngle:\tkz@SecondAngle:\tkz@radius pt);
\end{scope}
\endgroup 
}

\def\tkzLabelArc{\pgfutil@ifnextchar[{\tkz@LabelArc}{\tkz@LabelArc[]}}
\def\tkz@LabelArc[#1](#2,#3,#4)#5{%
\begingroup
\pgfqkeys{/@tkzmarkarc}{#1}
\tkz@@CalcLength(#2,#3){tkz@radius}
\tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstAngle}  
\tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@SecondAngle}
\tkzNormalizeAngle(\tkz@FirstAngle,\tkz@SecondAngle)
\pgfmathsubtract{\tkz@FirstAngle}{\tkz@delta}
\edef\tkz@FirstAngle{\pgfmathresult}%
\pgfmathadd{\tkz@SecondAngle}{\tkz@delta}
\edef\tkz@SecondAngle{\pgfmathresult} 
\begin{scope}[decoration={markings,mark=at position \tkz@mkarcpos with \node{#5};}]
 \path[shift = {(#2)},/@tkzmarkarc/.cd,#1,postaction={decorate}]%
  (\tkz@FirstAngle:\tkz@radius pt) arc (\tkz@FirstAngle:\tkz@SecondAngle:\tkz@radius pt); \end{scope}
\endgroup 
}
%<--------------------------------------------------------------------------->
%                       tkzDrawArcRAN                                        >
%<--------------------------------------------------------------------------->
\def\tkzDrawArcRAN[#1](#2,#3)(#4,#5){% 
\begingroup 
    \draw[shift = {(#2)},/tkzdrawarc/.cd,#1] (#4:#3) arc (#4:#5:#3); 
\endgroup  
}
%<--------------- tkzPathArcRAN ----------------------------------
\def\tkzPathArcRAN[#1](#2,#3)(#4,#5){% 
\begingroup     
    \path[shift = {(#2)},/tkzdrawarc/.cd,#1] (#4:#3) arc (#4:#5:#3); 
\endgroup  
}
%<--------------------------------------------------------------------------->
%       Mark an angle modi 3.03 suppression de \tkz@mksize,
%<--------------------------------------------------------------------------->
%                \tkzMarkAngle(B, A, C)
%
% Marque d'angle
% arc de cercle (simple/double/triple) et marque d'églité.
%
% Par défaut: 
%                 arc       = simple
%                 size     = 1 (rayon de l'arc)
%                 style traits pleins
%                 mkpos ?  position: 0.5 (position de la marque)
%                 mark rien du tout (ignoré si type est utilisé)
%
% Paramètres (optionnels)
%             arc     : l, ll, lll
%             mksize  : 1
%             gap     : 3pt
%             dist ?
%             style   : type de traits
%             position: 0.5
%             mark    : none  , |, ||,|||, z, s, x, o, oo mais tous les 
%  % symboles de tikz sont permis
%<------------------------- Label on angle -------------------------------->
\def\tkz@arcsimple{l} 
\def\tkz@arcdouble{ll}
\def\tkz@arctriple{lll} 

%\tikzset{lbstyle/.style = {color=\tkz@mainlinecolor}}

\pgfkeys{/tkzmkangle/.cd,
      arc/.estore in          = \tkz@arc,
      size/.store in          = \tkz@size,
      mark/.store in          = \tkz@markang,
      mkpos/.estore in        = \tkz@mkpos,
      mksize/.store in        = \tkz@mksize,
      mkcolor/.store in       = \tkz@mkcolor,
      arc                     = l,
      size                    = 1,
      mark                    = none,
      mksize                  = 4pt,
      mkcolor                 = black,
      mkpos                   = 0.5,
  /tkzmkangle/.search also={/tikz}   
}                        
\def\tkzMarkAngle{\pgfutil@ifnextchar[{\tkz@MarkAngle}{\tkz@MarkAngle[]}}   
\def\tkz@MarkAngle[#1](#2,#3,#4){%
\begingroup
\pgfqkeys{/tkzmkangle}{#1}
\tkzFindSlopeAngle(#3,#2)\tkzGetAngle{tkz@dirOne}
\tkzFindSlopeAngle(#3,#4)\tkzGetAngle{tkz@dirTwo}
\tkzNormalizeAngle(\tkz@dirOne,\tkz@dirTwo)

\def\tkz@mymark{\pgfsetplotmarksize{\tkz@mksize}\pgfuseplotmark{\tkz@markang}}
% draw the arcs
\begin{scope}[veclen]
  \begin{scope}[decoration= {markings,
                          mark=at position \tkz@mkpos with {\tkz@mymark}}]
    \ifx\tkz@arc\tkz@arcsimple
      \tkzDrawArcRAN[#1,fill=none]%
      (#3,\tkz@size)(\tkz@FirstAngle,\tkz@SecondAngle)%
      \tkzPathArcRAN[\tkz@mkcolor,postaction={decorate}]%
      (#3,\tkz@size)(\tkz@FirstAngle,\tkz@SecondAngle)
    \else
      \ifx\tkz@arc\tkz@arcdouble     
       \tkzDrawArcRAN[#1,fill=none](#3,\tkz@size cm-2.5\pgflinewidth)%
              (\tkz@FirstAngle,\tkz@SecondAngle) 
       \tkzPathArcRAN[\tkz@mkcolor,postaction={decorate}]%
             (#3,\tkz@size)(\tkz@FirstAngle,\tkz@SecondAngle)%
       \tkzDrawArcRAN[#1,fill=none](#3,\tkz@size cm+2.5\pgflinewidth)%
                       (\tkz@FirstAngle,\tkz@SecondAngle)% 
      \else 
         \ifx\tkz@arc\tkz@arctriple
            \tkzDrawArcRAN[#1,fill=none]%
            (#3,\tkz@size)(\tkz@FirstAngle,\tkz@SecondAngle)% 
            \tkzPathArcRAN[\tkz@mkcolor,postaction={decorate}]%
            (#3,\tkz@size)(\tkz@FirstAngle,\tkz@SecondAngle)%             
            \tkzDrawArcRAN[#1,fill=none](#3,\tkz@size cm-2.5\pgflinewidth)%
                      (\tkz@FirstAngle,\tkz@SecondAngle)%
            \tkzDrawArcRAN[#1,fill=none](#3,\tkz@size cm+2.5\pgflinewidth)%
                      (\tkz@FirstAngle,\tkz@SecondAngle)%   
         \fi
       \fi
    \fi
  \end{scope}
\end{scope}

\endgroup
}
%<--------------------------------------------------------------------------->
% multiple
\def\tkz@multiMA#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzMarkAngle[\tkz@optma](#1)}\tkz@temp%    
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------->
\def\tkzMarkAngles{\pgfutil@ifnextchar[{\tkz@MarkAngles}{\tkz@MarkAngles[]}}   
\def\tkz@MarkAngles[#1](#2){% 
\xdef\tkz@optma{#1} 
  \begingroup
   \let\next\tkz@multiMA
   \next#2 \@nil %    
\endgroup 
} 
% fin de \tkzMarkAngle
%<--------------------------------------------------------------------------->
%                        Pic Angle
%<--------------------------------------------------------------------------->
\def\tkzPicAngle{\pgfutil@ifnextchar[{\tkz@PicAngle}{\tkz@PicAngle[]}}   
\def\tkz@PicAngle[#1](#2,#3,#4){% 
\begingroup  
\draw pic [#1]{angle=#2--#3--#4};
\endgroup 
}
\def\tkzPicRightAngle{\pgfutil@ifnextchar[{\tkz@PicRightAngle}{\tkz@PicRightAngle[]}}   
\def\tkz@PicRightAngle[#1](#2,#3,#4){% 
\begingroup  
\draw pic [#1]{right angle=#2--#3--#4};
\endgroup 
}
%<--------------------------------------------------------------------------->
%                        FillAngle
%<--------------------------------------------------------------------------->
\pgfkeys{/tkzFill/.cd,
    size/.store in        = \tkz@size,
    size                  = 1,
    /tkzFill/.search also = {/tikz}
  } 

\def\tkzFillAngle{\pgfutil@ifnextchar[{\tkz@FillAngle}{\tkz@FillAngle[]}}   
\def\tkz@FillAngle[#1](#2,#3,#4){% 
\begingroup
\pgfqkeys{/tkzFill}{#1}   
  \tkzFindSlopeAngle(#3,#2)\tkzGetAngle{tkz@dirOne}   
  \tkzFindSlopeAngle(#3,#4)\tkzGetAngle{tkz@dirTwo}   
  \tkzNormalizeAngle(\tkz@dirOne,\tkz@dirTwo)
    \path[shift  = {(#3)},fill=\tkz@euc@linecolor!10,/tkzFill/.cd,#1]%
          (#3) -- (\tkz@FirstAngle:\tkz@size) arc%
          (\tkz@FirstAngle:\tkz@SecondAngle:\tkz@size)--cycle;
\endgroup 
}
%<--------------------------------------------------------------------------->
% multiple
\def\tkz@multiFA#1 #2\@nil{\protected@edef\tkz@temp{%
   \noexpand \tkzFillAngle[\tkz@optfa](#1)}%
   \tkz@temp%    
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------->
\def\tkzFillAngles{\pgfutil@ifnextchar[{\tkz@MFillAngles}{\tkz@MFillAngles[]}}   
\def\tkz@MFillAngles[#1](#2){% 
\xdef\tkz@optfa{#1} 
\begingroup
   \let\next\tkz@multiFA
   \next#2 \@nil %    
\endgroup 
} 
%<------------------------- Label on angle -------------------------------->
\pgfkeys{/tkzlabelangle/.cd,
    dist/.store in                  = \tkzlabeldist, 
    angle/.store in                 = \tkzlabelangle, 
    dist                            = 1,
    angle                           = {},
  /tkzlabelangle/.search also={/tikz}   
}  
\def\tkzLabelAngle{\pgfutil@ifnextchar[{\tkz@LabelAngle}{\tkz@LabelAngle[]}}
\def\tkz@LabelAngle[#1](#2,#3,#4)#5{%2016 added normalize from karu's code
\begingroup
  \pgfqkeys{/tkzlabelangle}{#1}
  \ifx\tkzutil@empty\tkzlabelangle% no value so calc angle of bisector
      \tkzFindSlopeAngle(#3,#2)\tkzGetAngle{tkz@dirOne}
      \tkzFindSlopeAngle(#3,#4)\tkzGetAngle{tkz@dirTwo}
      \tkzNormalizeAngle(\tkz@dirOne,\tkz@dirTwo)
      \edef\tkzlabelAngle{\fpeval{(\tkz@SecondAngle+\tkz@FirstAngle)/2}}
  \fi
  \path  (#3) --+(\tkzlabelAngle:\tkzlabeldist) node[label angle style,%
  /tkzlabelangle/.cd,#1] {#5};
\endgroup
}
%<--------------------------------------------------------------------------->
%<--------------------------------------------------------------------------->
% multiple labels
\def\tkz@multiLBA#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzLabelAngle[\tkz@optlba](#1){\tkz@labelangle}}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
% %<---------------------------------------------------------------------
\def\tkzLabelAngles{\pgfutil@ifnextchar[{\tkz@LabelAngles}{%
                                         \tkz@LabelAngles[]}}
\def\tkz@LabelAngles[#1](#2)#3{% 
 \def\tkz@optlba{#1}
 \def\tkz@labelangle{#3} 
   \begingroup
      \let\next\tkz@multiLBA
      \next#2 \@nil %
 \endgroup
}
%<-----------------------------------------------------------------------
%                     Symbole droites perpendiculaires      
%<---------------------------------------------------------------------- 
\pgfkeys{/tkzrightangle/.cd,
         norm tkz code/.is if            = normtkzcode@execute,
         german/.code                    = \normtkzcode@executefalse,
         size/.store in                  = \tkz@ra@size,
         dotsize/.store in               = \tkz@dotsize,
         size                            = .25,
         dotsize                         = 3 pt,
  /tkzrightangle/.search also={/tikz},
}
\newcommand*{\tkzMarkRightAngle}[1][]{\tkz@MarkRightAngle[#1]}
\def\tkz@MarkRightAngle[#1](#2,#3,#4){% 
\begingroup
\normtkzcode@executetrue
\pgfqkeys{/tkzrightangle}{#1} 
    \tkzpointnormalised{\pgfpointdiff{\pgfpointanchor{#3}{center}}{%
                                      \pgfpointanchor{#2}{center}}}
    \tkz@ax=\pgf@x\relax%
    \tkz@ay=\pgf@y\relax%
    \tkzpointnormalised{\pgfpointdiff{\pgfpointanchor{#3}{center}}{%
                                      \pgfpointanchor{#4}{center}}}
    \tkz@bx=\pgf@x\relax%
    \tkz@by=\pgf@y\relax%
  \ifnormtkzcode@execute%
      \draw[/tkzrightangle/.cd,#1]
    (#3) --++( 28.45274*\tkz@ra@size\tkz@ax , 28.45274*\tkz@ra@size\tkz@ay)
         --++( 28.45274*\tkz@ra@size\tkz@bx , 28.45274*\tkz@ra@size\tkz@by)
         --++(-28.45274*\tkz@ra@size\tkz@ax ,-28.45274*\tkz@ra@size\tkz@ay)
         -- (#3);
  \else%
    % find angles
      \tkzFindSlopeAngle(#3,#2)\tkzGetAngle{tkz@dirOne}
      \tkzFindSlopeAngle(#3,#4)\tkzGetAngle{tkz@dirTwo}
      \tkzNormalizeAngle(\tkz@dirOne,\tkz@dirTwo)
      \edef\tkzCircleAngle{\fpeval{(\tkz@SecondAngle+\tkz@FirstAngle)/2}}
      \tkzDrawArcRAN[/tkzrightangle/.cd,#1](#3,\tkz@ra@size)%
            (\tkz@FirstAngle,\tkz@SecondAngle)
      \path (#3) --+ (\tkzCircleAngle:\tkz@ra@size/2)
      node[fill,circle,minimum size=\tkz@dotsize,
           inner sep=0 pt,/tkzrightangle/.cd,#1] {};
\fi%
\endgroup
}
%<--------------------------------------------------------------------------->
\def\tkz@multiRA#1 #2\@nil{% 
\protected@edef\tkz@temp{
  \noexpand \tkzMarkRightAngle[\tkz@optRA](#1)}\tkz@temp% 
\def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
      \let\next\@gobble
   \fi
\next#2\@nil
}
%<--------------------------------------------------------------------------->
\def\tkzMarkRightAngles{\pgfutil@ifnextchar[{\tkz@RightAngles}{%
                                         \tkz@RightAngles[]}} 
\def\tkz@RightAngles[#1](#2){% 
\xdef\tkz@optRA{#1} 
\begingroup
    \let\next\tkz@multiRA
    \next#2 \@nil %    
\endgroup 
}    
%<--------------------------------------------------------------------------->
% tkzdefMidArc center and two points
\def\tkzDefMidArc(#1,#2,#3){%
\begingroup
\tkz@@CalcLength(#1,#2){tkz@radius}
\tkzFindSlopeAngle(#1,#2)\tkzGetAngle{tkz@FirstAngle}
\tkzFindSlopeAngle(#1,#3)\tkzGetAngle{tkz@SecondAngle}
\tkzNormalizeAngle(\tkz@FirstAngle,\tkz@SecondAngle)
 \path[shift = {(#1)}](\tkz@FirstAngle:\tkz@radius pt) arc
           (\tkz@FirstAngle:\tkz@SecondAngle:\tkz@radius pt)  coordinate[midway] (tkzPointResult);
\endgroup
}
\makeatother

\endinput

==> tikz-euclide/drawings/tkz-draw-eu-circles.tex <==
% tkz-obj-eu-draw-circles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-draw-circles.tex} 
\makeatletter 
%<--------------------------------------------------------------------------–>
%                    tkzSetUpCircle  
%<--------------------------------------------------------------------------–>
\pgfkeys{%
    /tkzsetupcirc/.cd,
    color/.code              =   \def\tkz@circle@color{#1},
    line width/.code         =   \def\tkz@circle@linewidth{#1},
    style/.code              =   \def\tkz@circle@style{#1},
  /tkzsetupcirc/.search also =   {/tikz}
 } 
 %<--------------------------------------------------------------------------–>
 
\def\tkzSetUpCircle{\pgfutil@ifnextchar[{\tkz@SetUpCircle}{\tkz@SetUpCircle[]}}
\def\tkz@SetUpCircle[#1]{%
\pgfkeys{%
    tkzsetupcirc/.cd,
    line width                  = \tkz@euc@circlelw,
    color                       = \tkz@euc@circlecolor,
    style                       = \tkz@euc@circlestyle
}
\pgfqkeys{/tkzsetupcirc}{#1}
\tikzset{%
    circle style/.append style   = { %
    color                        = \tkz@circle@color,
    line width                   = \tkz@circle@linewidth,
    style                        = \tkz@circle@style,
    #1}
    }
}% end setup 
 %<--------------------------------------------------------------------------–>

\def\tkzDrawCircle{\pgfutil@ifnextchar[{\tkz@DrawCircle}{\tkz@DrawCircle[]}}
\def\tkz@DrawCircle[#1](#2,#3){%  
\begingroup 
\node [draw,circle through=(#3), circle style,#1] at (#2) {};  
%perhaps I need to use the last method
     %  \tkzCalcLength(#2,#3) \tkzGetLength{tkz@ncradius}
			% \draw[circle style,#1](#2) circle (\tkz@ncradius);
\endgroup
}
%<--------------------------------------------------------------------------–> 
\def\tkz@multicircles#1 #2\@nil{% 
\protected@edef\tkz@temp{
\noexpand \tkzDrawCircle[\tkz@optcircle](#1)}\tkz@temp% 
\def\tkz@nextArg{#2}%
\ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
\fi
\next#2\@nil
}%
%<--------------------------------------------------------------------------–>
\def\tkzDrawCircles{\pgfutil@ifnextchar[{\tkz@DrawCircles}{\tkz@DrawCircles[]}} 
\def\tkz@DrawCircles[#1](#2){%
\xdef\tkz@optcircle{#1} 
\begingroup
   \let\next\tkz@multicircles
   \next#2 \@nil %    
\endgroup     
}% 
%<--------------------------------------------------------------------------–>
% #2 #3 rayon

\def\tkzDrawSemiCircle{\pgfutil@ifnextchar[{\tkz@DrawSemiCircle}{%
                                            \tkz@DrawSemiCircle[]}}
\def\tkz@DrawSemiCircle[#1](#2,#3){% 
\begingroup 
    \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                 {\pgfpointanchor{#3}{center}}%
    \tkz@ax=\pgf@x%
    \tkz@ay=\pgf@y%
    \path(#2)--++(-\tkz@ax,-\tkz@ay) coordinate (tkz@pt); 
    \tkzDrawArc[#1,delta=0](#2,#3)(tkz@pt)
\endgroup
}%
%<--------------------------------------------------------------------------–> 
\def\tkz@multisemicircles#1 #2\@nil{% 
\protected@edef\tkz@temp{
\noexpand \tkzDrawSemiCircle[\tkz@optsemicircle](#1)}\tkz@temp% 
\def\tkz@nextArg{#2}%
\ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
\fi
\next#2\@nil
}%
%<--------------------------------------------------------------------------–>
\def\tkzDrawSemiCircles{\pgfutil@ifnextchar[{\tkz@DrawSemiCircles}{%
\tkz@DrawSemiCircles[]}} 
\def\tkz@DrawSemiCircles[#1](#2){%
\xdef\tkz@optsemicircle{#1} 
\begingroup
   \let\next\tkz@multisemicircles
   \next#2 \@nil %    
\endgroup     
}% 
%<---------------------------- Fill Circle  --------------------------------–>
\def\tkzFillCircle{\pgfutil@ifnextchar[{\tkz@FillCircle}{\tkz@FillCircle[]}}
\def\tkz@FillCircle[#1](#2,#3){%
\begingroup      
   \node [fill,circle through=(#3),#1] at (#2) {};   
\endgroup
}%
\def\tkz@multifillcircles#1 #2\@nil{% 
\protected@edef\tkz@temp{
\noexpand \tkzFillCircle[\tkz@optfillcircle](#1)}\tkz@temp% 
\def\tkz@nextArg{#2}%
\ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
\fi
\next#2\@nil
}%
\def\tkzFillCircles{\pgfutil@ifnextchar[{\tkz@FillCircles}{%
\tkz@FillCircles[]}} 
\def\tkz@FillCircles[#1](#2){%
\xdef\tkz@optfillcircle{#1} 
\begingroup
   \let\next\tkz@multifillcircles
   \next#2 \@nil %    
\endgroup     
}% 

%<--------------------------- Clip Circle  ---------------------------------–>
\pgfkeys{/tkzclipc/.cd,    
         out code/.is if         =  tkzClipOutCircle,
         out/.code               =  \tkzClipOutCirclefalse
}%
%<--------------------------------------------------------------------------–>
\def\tkzClipCircle{\pgfutil@ifnextchar[{\tkz@ClipCircle}{\tkz@ClipCircle[]}}
\def\tkz@ClipCircle[#1](#2,#3){%    
\tkzClipOutCircletrue
\pgfqkeys{/tkzclipc}{#1}
   \tkz@@CalcLength(#2,#3){tkzLengthResult}
   \iftkzClipOutCircle
     \clip (#2) circle (\tkzLengthResult pt);
   \else
     \clip (#2) circle (\tkzLengthResult pt) [tkzreverseclip] ;
    \fi
} 
%<--------------------------- Label Circle  --------------------------------–>
\def\tkzLabelCircle{\pgfutil@ifnextchar[{\tkz@LabelCircle}{%
                                         \tkz@LabelCircle[]}}
% [option]  (#2,#3) #2 center #3  un point du cercle  #4 angle #5 the label
\def\tkz@LabelCircle[#1](#2,#3)(#4)#5{%
\begingroup      
   \tkzURotateAngle(#2,#4)(#3)
   \node[label style,#1] at (tkzPointResult) {#5};        
\endgroup
}
\makeatother 
\endinput

==> tikz-euclide/drawings/tkz-draw-eu-compass.tex <==
% tkz-obj-eu-compass.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-compass.tex}  
\makeatletter
%<--------------------------------------------------------------------------–>
%  Author Alain Matthes  
%   idea from Y. Combe   
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                Utilisation du Compas : Compass   
%<--------------------------------------------------------------------------–>
%                                Setup   Compass
%<--------------------------------------------------------------------------–>
\pgfkeys{tkzsucompass/.cd,
  line width/.store in          =   \tkz@compass@lw,
  color/.store in               =   \tkz@compass@color,
  style/.store in               =   \tkz@compass@style,
  line width                    =   \tkz@euc@compasswidth,
  color                         =   \tkz@euc@compasscolor,
  style                         =   \tkz@euc@compassstyle,
   /tkzsucompass/.search also   =   {/tikz,/tkzcompass}
  } 
%<--------------------------------------------------------------------------–>
\def\tkzSetUpCompass{\pgfutil@ifnextchar[{\tkz@SetUpCompass}{\tkz@SetUpCompass[]}}
%<--------------------------------------------------------------------------–>
\def\tkz@SetUpCompass[#1]{% 
\pgfqkeys{/tkzsucompass}{#1}
\tikzset{compass style/.style={%
    color       = \tkz@compass@color,
    line width  = \tkz@compass@lw,
    style       = \tkz@compass@style
                            }}
}
%<--------------------------------------------------------------------------–> 
%                \tkzCompass(A, B)
%
% Marque de compas auto-ajustée en longueur
%               #2 center #3 le point
% Par défaut: 
%                 longueur : 1cm, mais avec un maximum d'un angle de 180°
%                 angle calculé pour la longueur
%                 style traits pleins

%<--------------------------------------------------------------------------–> 
 \pgfkeys{/tkzcompass/.cd,
    delta/.store in      = \tkz@delta,
    length/.store in     = \tkz@length,
    length = 1,
    delta  = 0,
    /tkzcompass/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
    \pgfkeysalso{\searchname/.try=#1, /tikz/\searchname/.retry=#1}}
}
                                        
\def\tkzCompass{\pgfutil@ifnextchar[{\tkz@Compass}{\tkz@Compass[]}}
\def\tkz@Compass[#1](#2,#3){%   
\begingroup
\pgfkeys{tkzcompass/.cd,#1}  
\tkz@@CalcLength(#2,#3){tkz@tempLen}  
\ifnum\tkz@delta=0 %
   \pgfmathsetmacro{\tkz@delta}{min(deg(\tkz@length cm/ \tkz@tempLen pt),180)/2}
\fi 
\tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@angle}%
\draw[shift ={(#2)},compass style,/tkzcompass/.cd,#1]%
    (\tkz@angle-\tkz@delta:\tkz@tempLen pt)%
  arc (\tkz@angle-\tkz@delta:\tkz@angle+\tkz@delta:\tkz@tempLen pt);
\endgroup}
%<--------------------------------------------------------------------------–> 
\def\tkz@multiCompass#1 #2\@nil{% 
 \protected@edef\tkz@temp{
   \noexpand \tkzCompass[\tkz@optcompass](#1)}\tkz@temp% 
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
\def\tkzCompasss{\pgfutil@ifnextchar[{\tkz@Compasss}{\tkz@Compasss[]}}   

\def\tkz@Compasss[#1](#2){%
\global\edef\tkz@optcompass{#1} 
\begingroup
   \let\next\tkz@multiCompass
   \next#2 \@nil %    
\endgroup
}%

\makeatother
\endinput 

==> tikz-euclide/drawings/tkz-draw-eu-lines.tex <==
% tkz-obj-eu-draw-lines.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-draw-lines.tex}   
\makeatletter

%<--------------------------------------------------------------------------–>
%                                Setup   Line
%<--------------------------------------------------------------------------–>
\pgfkeys{%
   tkzsuline/.cd,
   line width/.code       =   \def\tkz@line@width{#1},
   color/.code            =   \def\tkz@line@color{#1},
   style/.code            =   \def\tkz@line@style{#1},
   add/.code args         =   {#1 and #2} {\def\tkz@line@left{#1}
                                           \def\tkz@line@right{#2}},
  /tkzsuline/.search also = {/tikz}
} 
%<--------------------------------------------------------------------------–>
\def\tkzSetUpLine{\pgfutil@ifnextchar[{\tkz@SetUpLine}{\tkz@SetUpLine[]}}
\def\tkz@SetUpLine[#1]{%
\pgfkeys{%
      tkzsuline/.cd,
      line width   = \tkz@euc@linewidth,
      color        = \tkz@euc@linecolor,
      style        = \tkz@euc@linestyle,
      add          = {\tkz@euc@lineleft} and {\tkz@euc@lineright}}  
\pgfqkeys{/tkzsuline}{#1}
\tikzset{%
        line style/.append style ={%
        line width        = \tkz@line@width,
        color             = \tkz@line@color,
        style             = \tkz@line@style,
        add               = {\tkz@line@left} and {\tkz@line@right},
        line cap          = round,
        #1}
        }
}% end setup  
%<--------------------------------------------------------------------------–>
%            Drawing a line                                                  
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% \pgfkeys{/tkzdrawl/.cd,
%    /tkzdrawl/.search also={/tikz}
% }
\def\tkzDrawLine{\pgfutil@ifnextchar[{\tkz@DrawLine}{\tkz@DrawLine[]}}
\def\tkz@DrawLine[#1](#2,#3){%    
\begingroup 
 % \pgfqkeys{/tkzdrawl}{#1}  
   \draw[line style,#1] (#2) to (#3);
\endgroup
}
%<-------------------------------------------------------------------------–
%         tkzDrawLines 
%<-------------------------------------------------------------------------–
\def\tkz@@multiLines#1 #2\@nil{% 
  \protected@edef\tkz@temp{
    \noexpand \tkzDrawLine[\tkz@optline](#1)}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------–>
\def\tkzDrawLines{\pgfutil@ifnextchar[{\tkz@DrawLines}{\tkz@DrawLines[]}}  
\def\tkz@DrawLines[#1](#2){%
\xdef\tkz@optline{#1} 
\begingroup
   \let\next\tkz@@multiLines
   \next#2 \@nil %    
\endgroup     
}%  
%<-------------------------------------------------------------------------–> 
%   Label
%<-------------------------------------------------------------------------–> 
\def\tkzLabelLine{\pgfutil@ifnextchar[{\tkz@AddLabelLine}{\tkz@AddLabelLine[]}} 
\def\tkz@AddLabelLine[#1](#2,#3)#4{\path  (#2) to node[#1]{#4}(#3);} 


%<--------------------------------------------------------------------------–>
%                             draw      segment  (s)
%<--------------------------------------------------------------------------–>  
\pgfkeys{/tkzdraws/.cd,
  /tkzdraws/.search also={/tikz},
}                              
\def\tkzDrawSegment{\pgfutil@ifnextchar[{\tkz@DrawSegment}{%
                                         \tkz@DrawSegment[]}} 
\def\tkz@DrawSegment[#1](#2,#3){%    
\scope
  \pgfqkeys{/tkzdraws}{#1}
  \draw[line style,add=0 and 0,#1] (#2) to (#3); 
\endscope  
}%    

\def\tkz@multiDrawSeg#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzDrawSegment[\tkz@optseg](#1)}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
} 
\def\tkzDrawSegments{\pgfutil@ifnextchar[{\tkz@DrawSegments}{%
                                         \tkz@DrawSegments[]}}
\def\tkz@DrawSegments[#1](#2){% 
\def\tkz@optseg{#1} 
\begingroup
  \let\next\tkz@multiDrawSeg
  \next#2 \@nil %
\endgroup
}
%<--------------------------------------------------------------------------–>
%                               Mark   Segment
%<--------------------------------------------------------------------------–>
\pgfkeys{
  /@tkzmarkoptions/.cd,
     pos/.store in       = \tkz@mkpos,
     color/.store in     = \tkz@mkcolor,
     mark/.store in      = \tkz@markseg,
     size/.store in      = \tkz@mksize,
     size                = 4pt,
     color               = \tkz@mk@color,
     pos                 = .5,
     mark                = |,
    /@tkzmarkoptions/.search also={/tikz},
}
\def\tkzMarkSegment{\pgfutil@ifnextchar[{\tkz@MarkSegment}{\tkz@MarkSegment[]}}
\def\tkz@MarkSegment[#1](#2,#3){%
\begingroup
 \pgfqkeys{/@tkzmarkoptions}{#1}
\def\tkz@mymark{\pgfsetplotmarksize{\tkz@mksize}\pgfuseplotmark{\tkz@markseg}}
\begin{scope} 
  [decoration={markings,mark=at position \tkz@mkpos with {\tkz@mymark}}] 
  \path [\tkz@mkcolor,/@tkzmarkoptions/.cd,#1,postaction={decorate}] (#2) -- (#3);
\end{scope}
\endgroup
}
%<--------------------------------------------------------------------------–>
% multiple
\def\tkz@multiMS#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzMarkSegment[\tkz@optsg](#1)}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------–>
\def\tkzMarkSegments{\pgfutil@ifnextchar[{\tkz@MarkSegments}{\tkz@MarkSegments[]}}
\def\tkz@MarkSegments[#1](#2){% 
\def\tkz@optsg{#1} 
  \begingroup
   \let\next\tkz@multiMS
   \next#2 \@nil %
\endgroup 
} 
%<-------------------------------------------------------------------------–> 
%             Label on segment  
%<-------------------------------------------------------------------------–> 
\def\tkzLabelSegment{\pgfutil@ifnextchar[{\tkz@LabelSegment}%
                     {\tkz@LabelSegment[]}}
\def\tkz@LabelSegment[#1](#2,#3)#4{%
\begingroup    
  \path  (#2) to node[label style,#1]{#4} (#3) ;  
\endgroup 
} 
%<--------------------------------------------------------------------------–>
% multiple
\def\tkz@multiLS#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzLabelSegment[\tkz@optls](#1){\tkz@labelseg}}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------–>
\def\tkzLabelSegments{\pgfutil@ifnextchar[{\tkz@LabelSegments}{\tkz@LabelSegments[]}}
\def\tkz@LabelSegments[#1](#2)#3{% 
\def\tkz@optls{#1}
\def\tkz@labelseg{#3}
  \begingroup
   \let\next\tkz@multiLS
   \next#2 \@nil %    
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%             PolySeg
%<--------------------------------------------------------------------------–>
\def\tkzDrawPolySeg{\pgfutil@ifnextchar[{\tkz@DrawPolySeg}{\tkz@DrawPolySeg[]}}
\def\tkz@DrawPolySeg[#1](#2,#3){% 
\begingroup
\draw[line style,#1] (#2)
     \foreach \pt in {#2,#3}{--(\pt)};%
\endgroup
}


%<--------------------------------------------------------------------------–>
%  add dim
    % \draw[dim={5,7pt,}]   (A) --  (B);
    % \draw[dim={7,10pt,transform shape}]  (B) --  (C);
    % \draw[dim={X,,}]  (A) --  (C);
%<--------------------------------------------------------------------------–>
% new code from muzimuzhi Z
%https://tex.stackexchange.com/questions/553430/change-color-and-style-of-dimension-lines-in-tkz-euclide/553441

\pgfkeys{/pgf/decoration/.cd, distance/.initial = 10pt}  

\pgfdeclaredecoration{add dim}{final}{
\state{final}{% 
\pgfmathsetmacro{\dist}{\pgfkeysvalueof{/pgf/decoration/distance}}
          \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
          \pgfpathlineto{\pgfpoint{0pt}{1.2*\dist}}   
          \pgfpathmoveto{\pgfpoint{\pgfdecoratedpathlength}{0pt}} 
          \pgfpathlineto{\pgfpoint{(\pgfdecoratedpathlength}{1.2*\dist}}
          % start of patch
          \pgfusepath{stroke}
          \pgfsetarrowsstart{latex}
          \pgfsetarrowsend{latex}
          \expandafter\pgfsetdash\tkz@dim@dashpattern
          \pgfsetstrokecolor{\tkz@dim@color}
          % end of patch
          \pgfpathmoveto{\pgfpoint{0pt}{\dist}}
          \pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{\dist}} 
          \pgfusepath{stroke} 
          \pgfpathmoveto{\pgfpoint{0pt}{0pt}}
          \pgfpathlineto{\pgfpoint{\pgfdecoratedpathlength}{0pt}}
}}


\tikzset{
  dim/.style args={#1,#2,#3}{%
    postaction={
      decoration={
        show path construction,
        lineto code={
          % dim fence
          \draw[dim fence style/.try]
            (\tikzinputsegmentfirst) --
              ($ (\tikzinputsegmentfirst)!1.2*(#2)!90:(\tikzinputsegmentlast) $)
            (\tikzinputsegmentlast) --
            ($ (\tikzinputsegmentlast)!1.2*(#2)!-90:(\tikzinputsegmentfirst) $);
          % dim
          \draw[dim style/.try]
            ($ (\tikzinputsegmentfirst)!#2!90:(\tikzinputsegmentlast) $) --
            node[inner sep=0pt, font=\footnotesize, fill=\tkz@fillcolor, pos=.5, #3] {#1}
            ($ (\tikzinputsegmentlast)!#2!-90:(\tikzinputsegmentfirst) $);
        }
      },
      decorate,
    }
  },
  dim/.default={,0pt,},
  dim style/.style={
    latex-latex,
  },
}

%<---------------------------  style line ---------------------------------> 
\tikzset{add/.style args={#1 and #2}{to path={%
 ($(\tikztostart)!-#1!(\tikztotarget)$)--($(\tikztotarget)!-#2!(\tikztostart)$)%
  \tikztonodes}}
} 
\makeatother
\endinput

==> tikz-euclide/drawings/tkz-draw-eu-points.tex <==
 % tkz-draw-points.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.01c}
\def\filedate{2023/01/24} 
\typeout{2023/01/24 5.01c  tkz-draw-points.tex} 
\makeatletter
%<--------------------------------------------------------------------------->
%                    tkzSetUpPoint  définit la forme d'un point
%<--------------------------------------------------------------------------->
\pgfkeys{/tkzsetuppt/.cd,
      size/.store in       =  \tkz@pt@size,
      color/.store in      =  \tkz@pt@color,
      fill/.store in       =  \tkz@pt@fill, 
      shape/.store in      =  \tkz@pt@shape,
      size                 =  \tkz@euc@pointsize,
      color                =  \tkz@euc@pointcolor,
      fill                 =  \tkz@euc@pointcolor,
      shape                =  \tkz@euc@pointshape,
   /tkzsetuppt/.search also  = {/tikz},
 } 
\def\tkzSetUpPoint{\pgfutil@ifnextchar[{\tkz@SetUpPoint}{%
                                        \tkz@SetUpPoint[]}}
\def\tkz@SetUpPoint[#1]{%
\pgfqkeys{/tkzsetuppt}{#1}
% redefine point style with new values
\tikzset{point style/.style={draw         = \tkz@pt@color,
                             inner sep    = 0pt,
                             shape        = \tkz@pt@shape,
                             minimum size = \tkz@pt@size,
                             fill         = \tkz@pt@fill}}
}% end setup
%<--------------------------------------------------------------------------->
%                       Draw Point   
%<--------------------------------------------------------------------------->
\pgfkeys{/tkzdrawpt/.cd, 
  size/.code   = {\tikzset{point style/.append style={minimum size = #1}}},
  size         = \tkz@euc@pointsize,
  /tkzdrawpt/.search also  = {/tikz},
}
%<--------------------------------------------------------------------------    
\def\tkzDrawPoint{\pgfutil@ifnextchar[{\tkz@DrawPoint}{\tkz@DrawPoint[]}} 
\def\tkz@DrawPoint[#1](#2){%
\begingroup 
    \pgfqkeys{/tkzdrawpt}{#1}    
    \node[point style,/tkzdrawpt/.cd,#1] at (#2) {};%2016
\endgroup
}
%<---------------------------------------------------------------------------> 
\def\tkzDrawPoints{\pgfutil@ifnextchar[{\tkz@drawpts}{\tkz@drawpts[]}} 
%<---------------------------------------------------------------------------> 
\def\tkz@drawpts[#1](#2){%
\begingroup
   \pgfqkeys{/tkzdrawpt}{#1}        
   \foreach \point in {#2}{\node[point style,/tkzdrawpt/.cd,#1] at (\point) {};} %2016
\endgroup 
}
%<-------------------------------------------------------------------------->
%                   tkzLabelPoint          Affichage des LABELS pour un point
%<-------------------------------------------------------------------------->  
\def\tkzLabelPoint{\pgfutil@ifnextchar[{\tkz@LabelPoint}{\tkz@LabelPoint[]}} 
\def\tkz@LabelPoint[#1](#2)#3{%
      \node[label style,#1] at (#2) {#3};}%
%<--------------------------------------------------------------------------->

\def\tkzLabelPoints{\pgfutil@ifnextchar[{\tkz@LabelPoints}{\tkz@LabelPoints[]}}% 
\def\tkz@LabelPoints[#1](#2){%
 \foreach \point in {#2}{
      \node[label style,#1] at (\point) {$\point$};}
}%
%<--------------------------------------------------------------------------->
%<--------------------------------------------------------------------------->
%
%<--------------------------------------------------------------------------->
\def\tkzSetUpLabel{\pgfutil@ifnextchar[{\tkz@SetUpLabel}{%
                                        \tkz@SetUpLabel[]}}
\def\tkz@SetUpLabel[#1]{%
\tikzset{label style/.style={#1}}
}% end setup
%<--------------------------------------------------------------------------->

\pgfkeys{/tkzautolab/.cd,
    center/.store in           = \tkz@center,
    dist/.store in             = \tkz@dist,
    dist                       = 0.15,
   /tkzautolab/.search also   = {/tikz},
}
\def\tkzAutoLabelPoints{\pgfutil@ifnextchar[{\tkz@AutoLabelPoints}{\tkz@AutoLabelPoints[]}}% 
\def\tkz@AutoLabelPoints[#1](#2){%
\begingroup 
\pgfqkeys{/tkzautolab}{#1} 
 \foreach \point in {#2}{
 \path (\tkz@center) -- ($ (\point) + \tkz@dist*($(\point)-(\tkz@center)$) $) node[/tkzautolab/.cd,label style,#1]{$\point$};}
\endgroup
}%
%<--------------------------------------------------------------------------->
%                                 PointShowCoord  
%<--------------------------------------------------------------------------->
\pgfkeys{/tkzprcoord/.cd,
          xlabel/.store in    = \tkz@xlabel,
          ylabel/.store in    = \tkz@ylabel, 
          xstyle/.code        = {\tikzset{xcoord style/.append style={#1}}},
          ystyle/.code        = {\tikzset{ycoord style/.append style={#1}}},
          noxdraw/.is if      = tkz@coord@noxdraw,
          noxdraw/.default    = true,
          noydraw/.is if      = tkz@coord@noydraw,
          noydraw/.default    = true,
          xlabel              = {},
          ylabel              = {},
          xstyle              = {},
          ystyle              = {},
          noxdraw             = false,
          noydraw             = false,    
  /tkzprcoord/.search also   = {/tikz},
}
\def\tkzPointShowCoord{\pgfutil@ifnextchar[{\tkz@PointShowCoord}{\tkz@PointShowCoord[]}}     
\def\tkz@PointShowCoord[#1](#2){%
\begingroup 
\pgfqkeys{/tkzprcoord}{#1} 
% 2019 for showcoord
 \iftkznodedefined{tkz@xline}{}{%
 \path (0,0) --(1,0) node(tkz@xline){};
 \path (0,0) --(0,1) node(tkz@yline){};
 }
\iftkz@coord@noxdraw\else\draw[arrow coord style,/tkzprcoord/.cd,#1] (#2)--(#2 |- tkz@xline);\fi 
\iftkz@coord@noydraw\else\draw[arrow coord style,/tkzprcoord/.cd,#1] (#2)--(#2 -| tkz@yline);\fi   
\ifx\tkzutil@empty\tkz@xlabel
\else
\path (#2)--(#2 |- tkz@xline)
  node[xcoord style] {\tkz@xlabel};
\fi
\ifx\tkzutil@empty\tkz@ylabel
\else
 \path (#2)--(#2 -| tkz@yline)
   node[ycoord style] {\tkz@ylabel};
\fi    
\endgroup
}
\let\tkzShowPointCoord\tkzPointShowCoord
\makeatother  
\endinput

==> tikz-euclide/drawings/tkz-draw-eu-polygons.tex <==
% tkz-obj-eu-polygons.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-polygons.tex} 
\makeatletter  
%<--------------------------------------------------------------------------–>
%                                 Polygon 
%<--------------------------------------------------------------------------–>
%<----------------------------   Draw       --------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkzDrawPolygon{\pgfutil@ifnextchar[{\tkz@DrawPolygon}{%
                                         \tkz@DrawPolygon[]}}
\def\tkz@DrawPolygon[#1](#2,#3){%
 \begingroup
 \draw[line style,line join=round,#1] (#2)
     \foreach \pt in {#2,#3}{--(\pt)}--cycle;%
 \endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkz@multipolygons#1 #2\@nil{% 
\protected@edef\tkz@temp{
\noexpand \tkzDrawPolygon[\tkz@optpolygon](#1)}\tkz@temp% 
\def\tkz@nextArg{#2}%
\ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
\fi
\next#2\@nil
}
%<--------------------------------------------------------------------------–>
\def\tkzDrawPolygons{\pgfutil@ifnextchar[{\tkz@DrawPolygons}{\tkz@DrawPolygons[]}} 
\def\tkz@DrawPolygons[#1](#2){%
\xdef\tkz@optpolygon{#1} 
\begingroup
   \let\next\tkz@multipolygons
   \next#2 \@nil %    
\endgroup     
}% 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–> 
%<----------------------------   FILL       --------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkzFillPolygon{\pgfutil@ifnextchar[{\tkz@FillPolygon}{%
                                         \tkz@FillPolygon[]}} 
\def\tkz@FillPolygon[#1](#2,#3){%
 \begingroup
     \fill[#1] (#2)
   \foreach \pt in {#2,#3}{--(\pt)}--cycle;%  
\endgroup
}
%<--------------------------------------------------------------------------–>
%<--------------   Labels for Regular Polygon      -------------------------–>
%
%<--------------------------------------------------------------------------–>
\pgfkeys{/deflabelregpoly/.cd,
      name/.store in      =   \tkz@regpolname,
      sep/.store in       =   \tkz@regpolsep,
      name        = P,
      sep         = 1.1
}   
 
\def\tkzLabelRegPolygon{\pgfutil@ifnextchar[{\tkz@labelPolygon}{%
                                             \tkz@labelPolygon[]}}  
\def\tkz@labelPolygon[#1](#2)#3{% 
\begingroup 
\pgfqkeys{/deflabelregpoly}{#1}  
 \foreach \v [count=\vi from 1]  in {#3}  {%
  \path (#2) to [pos=1.1] node {$\v$} (\tkz@regpolname\vi) ; 
  \pgfnodealias{\v}{\tkz@regpolname\vi} 
  } 
\endgroup
} 
%<----------------------------   CLIP       --------------------------------–>
%
%<--------------------------------------------------------------------------–>

\pgfkeys{tkzclippolygon/.cd,
       out code/.is if         = tkzClipOutPoly,
       out/.code               = \tkzClipOutPolyfalse}   

\def\tkzClipPolygon{\pgfutil@ifnextchar[{\tkz@ClipPolygon}{\tkz@ClipPolygon[]}}  
\def\tkz@ClipPolygon[#1](#2,#3){%
\tkzClipOutPolytrue
\pgfqkeys{/tkzclippolygon}{#1}%   
\iftkzClipOutPoly
\clip (#2)
   \foreach \pt in {#2,#3}{--(\pt)}--cycle;
\else
   \clip(#2)
    \foreach \pt in {#2,#3}{--(\pt)}--cycle[tkzreverseclip] ;
\fi 
}%
\makeatother
\endinput

==> tikz-euclide/drawings/tkz-draw-eu-protractor.tex <==
% tkz-obj-eu-protractor.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-protractor.tex}  
\makeatletter
%<--------------------------------------------------------------------------–>  
%                   !!! idea from Y. Combe  !!! 
%<--------------------------------------------------------------------------–> 
%                \tkzProtractor  Protractor
%
% Rapporteur ajustable et positionable
%
% Par défaut: 
%                  centre en (0,0)
%                  rayon de 5 cm
%                  ligne de base horizontale.
%                  épaisseur de ligne 0.4 pt
%
% Paramètres (optionnels, gérés par xkeyval)
%             shift : coordonées (n'importe quelle forme 
%                                            acceptée par tikz).
%             scale : facteur d'échelle
%             rotate : rotation
%             lw : line width (épaisseur des lignes)
%                   ce paramètre subit le facteur d'échelle.
%<--------------------------------------------------------------------------–> 
\def\FullProtractor{%
\draw[fill=black!50!yellow!20!,even odd rule,semitransparent]%
     (0,0) circle (4cm);
\draw (0,0) circle (3.3cm);
\draw (0,0) circle (4cm);
\draw[fill=black] (0,0) circle (.08mm);
\node[draw, circle, inner sep=.2mm] (a) at (0,0) {};
\foreach \x in {0, 90, ..., 360}{%
    \draw[very thin, gray!40] (a) -- (\x:4cm);}
\foreach \x in {0,...,359} {\draw (\x:3.8cm) -- (\x:4cm);}
\foreach \x in {0,5,...,355}  {\draw (\x:3.725cm) -- (\x:4cm);}
\foreach \x in {0,10,...,350}{%
     \node[rotate=(\x-90)] at (\x:3.6cm) {\tiny\x};
}
    \draw [>=stealth',->, thick,black] (0:2.5) arc(0:32:2.5);
    \draw [>=stealth',->, thick,black] (0:2) arc(0:32:2);
    \draw [>=stealth',->, thick,black] (0:1.5) arc(0:32:1.5);
}

\def\FullProtractorReturn{%
\draw[fill=black!50!yellow!20!,even odd rule,semitransparent] (0,0) circle (4cm);
\draw (0,0) circle (3.3cm);
\draw (0,0) circle (4cm);
\draw[fill=black] (0,0) circle (.08mm);
\node[draw, circle, inner sep=.2mm] (a) at (0,0) {};
\foreach \x in {0, 90, ..., 360}{%
    \draw[very thin, gray!40] (a) -- (\x:4cm);} 
\foreach \x in {0,...,359} {\draw (\x:3.8cm) -- (\x:4cm);}
\foreach \x in {0,5,...,355}  {\draw (\x:3.725cm) -- (\x:4cm);}   
\begin{scope}
   \foreach \x in {0,10,...,350}{%
      \node[rotate=(-\x-90)] at (-\x:3.6cm) {\tiny\x};
} 
  \end{scope}
  \draw [>=stealth',->, thick,black] (0:2.5) arc(0:-32:2.5);
  \draw [>=stealth',->, thick,black] (0:2) arc(0:-32:2); 
  \draw [>=stealth',->, thick,black] (0:1.5) arc(0:-32:1.5); 
} 

\pgfkeys{
  protractor/.cd,
  lw/.code        = {\def\cmdMO@Rap@lw{#1}},
  shift/.code     = {\def\cmdMO@Rap@shift{#1}},
  rotate/.code    = {\def\cmdMO@Rap@rotate{#1}},
  scale/.code     = {\def\cmdMO@Rap@scale{#1}},
  return/.is if   = tkz@RappReturn,
  return/.code     = \tkz@RappReturnfalse,
  /protractor/.search also={/tikz},
  lw = 0.4pt,
  scale=1,
  shift={(0,0)},
  rotate=0
  }  

\def\tkzProtractor{\pgfutil@ifnextchar[{\tkz@Protractor}{\tkz@Protractor[]}}
\def\tkz@Protractor[#1](#2,#3){%
\tkz@RappReturnfalse
\pgfqkeys{/protractor}{#1}
  \tkz@@extractxy{#2}
  \global\tkz@ax\pgf@x
  \global\tkz@ay\pgf@y
  \tkzFindSlopeAngle(#2,#3)
  \tkzGetAngle{cmdMO@Rap@rotate}%
  \global\let\tkz@@Protractor\FullProtractor%
  \iftkz@RappReturn
     \global\let\tkz@@Protractor\FullProtractorReturn
     \else
     \global\let\tkz@@Protractor\FullProtractor
 \fi
  \pgfmathsetlengthmacro{\MO@lw}{\cmdMO@Rap@lw * \cmdMO@Rap@scale}
  \begin{scope}[shift             = {(\tkz@ax,\tkz@ay)},%
                scale             = \cmdMO@Rap@scale,%
                rotate            = \cmdMO@Rap@rotate,%
                every node/.style = {scale =\cmdMO@Rap@scale,
                                     rotate =\cmdMO@Rap@rotate},%
                line width=\MO@lw]%
  \tkz@@Protractor 
\end{scope}
}
%<--------------------------------------------------------------------------–>
% fin de \tkzProtractor
%<--------------------------------------------------------------------------–>
\makeatother
\endinput

==> tikz-euclide/drawings/tkz-draw-eu-sectors.tex <==
% tkz-obj-eu-sectors.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-sectors.tex} 
\makeatletter  
%<-----------------------    Sectors         ------------------------------–>
\gdef\tkz@nums{0}
\pgfkeys{/drawsector/.cd,
  towards/.code               = {\def\tkz@nums{0}},
  rotate/.code                = {\def\tkz@nums{1}},
  R/.code                     = {\def\tkz@nums{2}},
  R with nodes/.code          = {\def\tkz@nums{3}},
  towards,
  /drawsector/.search also  = {/tikz},
} 

\def\tkzDrawSector{\pgfutil@ifnextchar[{\tkz@DrawSector}{\tkz@DrawSector[]}}
\def\tkz@DrawSector[#1](#2,#3)(#4){% 
\begingroup
\pgfqkeys{/drawsector}{#1}       
\ifcase\tkz@nums%
   \tkzDrawSectorN[#1](#2,#3)(#4)  
\or% 1
   \tkzDrawSectorRotate[#1](#2,#3)(#4)  
\or% 2
   \tkzDrawSectorRAngles[#1](#2,#3)(#4)
\or% 3
   \tkzDrawSectorR[#1](#2,#3)(#4)
\fi    
\endgroup
}
\def\tkzDrawSectorRAngles{\pgfutil@ifnextchar[{\tkz@DrawSectorRAngles}{%
                                               \tkz@DrawSectorRAngles[]}} 
\def\tkz@DrawSectorRAngles[#1](#2,#3)(#4,#5){%
\begingroup      
  \pgfmathparse{#4}\edef\tkz@FirstAngle{\pgfmathresult}% 
  \pgfmathparse{#5}\edef\tkz@SecondAngle{\pgfmathresult}%  
  \pgfmathgreaterthan{\tkz@FirstAngle}{0}   
  \ifdim\pgfmathresult pt=1 pt\relax%  
    \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
    \ifdim\pgfmathresult pt=1 pt\relax%
     \pgfmathsubtract{\tkz@FirstAngle}{360}
     \edef\tkz@FirstAngle{\pgfmathresult}%
 \fi 
 \else
     \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
    \ifdim\pgfmathresult pt=1 pt\relax%
     \pgfmathadd{\tkz@SecondAngle}{360}
     \edef\tkz@SecondAngle{\pgfmathresult}%
 \fi 
 \fi
 \draw[shift = {(#2)},/drawsector/.cd,#1]%
   (#2) --(\tkz@FirstAngle:#3) arc (\tkz@FirstAngle:\tkz@SecondAngle:#3)--cycle;
 \endgroup
  } %  revoir il y a plus simple que ce shift !!! 
%<--------------------------------------------------------------------------–>
% \tkzDrawSectorN(O,A)(B)
%<--------------------------------------------------------------------------–>
\def\tkzDrawSectorN{\pgfutil@ifnextchar[{\tkz@DrawSectorN}{%
                                         \tkz@DrawSectorN[]}}  
\def\tkz@DrawSectorN[#1](#2,#3)(#4){%
\begingroup
 \tkz@@CalcLengthcm(#2,#3){tkz@radius}
 \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstAngle}  
 \tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@SecondAngle} 
 \tkz@DrawSectorRAngles[#1](#2,\tkz@radius)(\tkz@FirstAngle,%
                                               \tkz@SecondAngle)      
\endgroup
}
%<--------------------------------------------------------------------------–>
% \tkzDrawSectorRotate(O,A)(angle de rotation) ??? pb avec angle negatif
%<--------------------------------------------------------------------------–>
\def\tkzDrawSectorRotate{\pgfutil@ifnextchar[{\tkz@DrawSectorRotate}{%
                                              \tkz@DrawSectorRotate[]}} 
\def\tkz@DrawSectorRotate[#1](#2,#3)(#4){%
\begingroup
    \tkz@@CalcLengthcm(#2,#3){tkz@radius} 
    \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstA} 
    \pgfmathadd{\tkz@FirstA}{#4}
    \edef\tkz@SecondA{\pgfmathresult} 
    \pgfmathgreaterthan{#4}{0}   
  \ifdim\pgfmathresult pt=1 pt\relax% 
   \tkz@DrawSectorRAngles[#1](#2,\tkz@radius)(\tkz@FirstA,\tkz@SecondA)    
  \else
  \tkz@DrawSectorRAngles[#1](#2,\tkz@radius)(\tkz@SecondA,\tkz@FirstA)      
  \fi        
\endgroup
}   
%<--------------------------------------------------------------------------–>
%  \tkzDrawSectorAngles(O,A)(ang1,ang2)
%<--------------------------------------------------------------------------–>
\def\tkzDrawSectorAngles{\pgfutil@ifnextchar[{\tkz@DrawSectorAngles}{%
                                              \tkz@DrawSectorAngles[]}}
\def\tkz@DrawSectorAngles[#1](#2,#3)(#4,#5){%
\begingroup
    \tkz@@CalcLengthcm(#2,#3){tkz@radius} 
    \tkz@DrawSectorRAngles[#1](#2,\tkz@radius pt)(#4,#5)      
\endgroup
}  
%<--------------------------------------------------------------------------–>
%    \tkzDrawSectorRwithNodesAngles(O,A,B)(ang1,ang2)
%<--------------------------------------------------------------------------–>
\def\tkzDrawSectorRwithNodesAngles{\pgfutil@ifnextchar[{%
                         \tkz@DrawSectorRwithNodesAngles}{%
                         \tkz@DrawSectorRwithNodesAngles[]}}   
\def\tkz@DrawSectorRwithNodesAngles[#1](#2,#3,#4)(#5,#6){%
\begingroup
    \tkz@@CalcLengthcm(#3,#4){tkz@radius}
    \tkz@DrawSectorRAngles[#1](#2,\tkz@radius pt)(#5,#6)
\endgroup
} 
% %<--------------------------------------------------------------------------–>
 
%<--------------------------------------------------------------------------–>
%  \tkzDrawSectorR(O, rad)(A,B)
%<--------------------------------------------------------------------------–>
\def\tkzDrawSectorR{\pgfutil@ifnextchar[{\tkz@DrawSectorR}{%
                                         \tkz@DrawSectorR[]}} 
\def\tkz@DrawSectorR[#1](#2,#3)(#4,#5){%
\begingroup 
  \tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@FirstAngle}  
  \tkzFindSlopeAngle(#2,#5)\tkzGetAngle{tkz@SecondAngle} 
  \tkz@DrawSectorRAngles[#1](#2,#3)(\tkz@FirstAngle,\tkz@SecondAngle)  
\endgroup   
}
%<--------------------------------------------------------------------------–>
%                                 Fill
%<--------------------------------------------------------------------------–>
\gdef\tkz@nums{0}
\pgfkeys{/@fillsector/.cd,
      towards/.code               = {\def\tkz@nums{0}},
      rotate/.code                = {\def\tkz@nums{1}},
      R/.code                     = {\def\tkz@nums{2}},
      R with nodes/.code          = {\def\tkz@nums{3}},
      towards,
      /@fillsector/.search also={/tikz},
} 

\def\tkzFillSector{\pgfutil@ifnextchar[{\tkz@FillSector}{\tkz@FillSector[]}}
\def\tkz@FillSector[#1](#2,#3)(#4){% 
\begingroup
\pgfqkeys{/@fillsector}{#1}     
\ifcase\tkz@nums%
   \tkzFillSectorN[#1](#2,#3)(#4)  
\or% 1
   \tkzFillSectorRotate[#1](#2,#3)(#4)  
\or% 2
   \tkzFillSectorRAngles[#1](#2,#3)(#4)
\or% 3
   \tkzFillSectorR[#1](#2,#3)(#4)
\fi    
\endgroup
}   


\def\tkzFillSectorRAngles{\pgfutil@ifnextchar[{\tkz@FillSectorRAngles}{%
                                               \tkz@FillSectorRAngles[]}} 
\def\tkz@FillSectorRAngles[#1](#2,#3)(#4,#5){%
\begingroup
  \pgfmathparse{#4}\edef\tkz@FirstAngle{\pgfmathresult}% 
  \pgfmathparse{#5}\edef\tkz@SecondAngle{\pgfmathresult}%  
   \pgfmathgreaterthan{\tkz@FirstAngle}{0}   
   \ifdim\pgfmathresult pt=1 pt\relax%  
     \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
     \ifdim\pgfmathresult pt=1 pt\relax%
      \pgfmathsubtract{\tkz@FirstAngle}{360}
      \edef\tkz@FirstAngle{\pgfmathresult}%
  \fi 
  \else
      \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
     \ifdim\pgfmathresult pt=1 pt\relax%
      \pgfmathadd{\tkz@SecondAngle}{360}
      \edef\tkz@SecondAngle{\pgfmathresult}%
  \fi\fi
  \pgfmathsubtract{\tkz@FirstAngle}{0}
  \edef\tkz@FirstAngle{\pgfmathresult}%
  \pgfmathadd{\tkz@SecondAngle}{0}
  \edef\tkz@SecondAngle{\pgfmathresult} 
  \path[shift  = {(#2)},/@fillsector/.cd,fill=\tkz@fillcolor,#1] (#2) -- %
      (\tkz@FirstAngle:#3) arc (\tkz@FirstAngle:\tkz@SecondAngle:#3)--cycle; 
\endgroup
}   
%<--------------------------------------------------------------------------–>
% \tkzFillSectorN(O,A)(B)
%<--------------------------------------------------------------------------–>
\def\tkzFillSectorN{\pgfutil@ifnextchar[{\tkz@FillSectorN}{\tkz@FillSectorN[]}} 
\def\tkz@FillSectorN[#1](#2,#3)(#4){%
\begingroup  
  \tkz@@CalcLength(#2,#3){tkz@radius}
  \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstAngle}  
  \tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@SecondAngle} 
  \tkz@FillSectorRAngles[#1](#2,\tkz@radius pt)(\tkz@FirstAngle,%
                                                \tkz@SecondAngle)    
\endgroup
}
%<--------------------------------------------------------------------------–>
% \tkzFillSectorRotate(O,A)(angle de rotation) ??? pb avec angle negatif
%<--------------------------------------------------------------------------–>
\def\tkzFillSectorRotate{\pgfutil@ifnextchar[{\tkz@FillSectorRotate}{%
                                              \tkz@FillSectorRotate[]}} 
\def\tkz@FillSectorRotate[#1](#2,#3)(#4){%
\begingroup
    \tkz@@CalcLength(#2,#3){tkz@radius} 
    \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@FirstA} 
    \pgfmathadd{\tkz@FirstA}{#4}
    \edef\tkz@SecondA{\pgfmathresult} 
    \pgfmathgreaterthan{#4}{0}   
  \ifdim\pgfmathresult pt=1 pt\relax% 
   \tkz@FillSectorRAngles[#1](#2,\tkz@radius pt)(\tkz@FirstA,\tkz@SecondA)    
  \else
  \tkz@FillSectorRAngles[#1](#2,\tkz@radius pt)(\tkz@SecondA,\tkz@FirstA)      
  \fi
   \endgroup
}   
%<--------------------------------------------------------------------------–>
%  \tkzFillSectorAngles(O,A)(ang1,ang2)
%<--------------------------------------------------------------------------–>
\def\tkzFillSectorAngles{\pgfutil@ifnextchar[{\tkz@FillSectorAngles}{%
                                              \tkz@FillSectorAngles[]}}
\def\tkz@FillSectorAngles[#1](#2,#3)(#4,#5){%
\begingroup
    \tkz@@CalcLength(#2,#3){tkz@radius} 
    \tkz@FillSectorRAngles[#1](#2,\tkz@radius pt)(#4,#5)      
\endgroup
}  
%<--------------------------------------------------------------------------–>
%  \tkzFillSectorR(O, rad)(A,B)
%<--------------------------------------------------------------------------–>
\def\tkzFillSectorR{\pgfutil@ifnextchar[{\tkz@FillSectorR}{%
                                         \tkz@FillSectorR[]}} 
\def\tkz@FillSectorR[#1](#2,#3)(#4,#5){%
\begingroup 
  \tkzFindSlopeAngle(#2,#4)\tkzGetAngle{tkz@FirstAngle}  
  \tkzFindSlopeAngle(#2,#5)\tkzGetAngle{tkz@SecondAngle} 
  \tkz@FillSectorRAngles[#1](#2,#3)(\tkz@FirstAngle,\tkz@SecondAngle)  
\endgroup   
}
%<--------------------------- Clip Sector ----------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkz@ClipSectorRAngles(#1,#2)(#3,#4){%
\begingroup      
  \pgfmathparse{#3}\edef\tkz@FirstAngle{\pgfmathresult}% 
  \pgfmathparse{#4}\edef\tkz@SecondAngle{\pgfmathresult}%  
  \pgfmathgreaterthan{\tkz@FirstAngle}{0}   
  \ifdim\pgfmathresult pt=1 pt\relax%  
    \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
    \ifdim\pgfmathresult pt=1 pt\relax%
     \pgfmathsubtract{\tkz@FirstAngle}{360}
     \edef\tkz@FirstAngle{\pgfmathresult}%
 \fi 
 \else
     \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
    \ifdim\pgfmathresult pt=1 pt\relax%
     \pgfmathadd{\tkz@SecondAngle}{360}
     \edef\tkz@SecondAngle{\pgfmathresult}%
 \fi 
 \fi
  \clip[shift = {(#1)}] (#1) --(\tkz@FirstAngle:#2)%
        arc(\tkz@FirstAngle:\tkz@SecondAngle:#2) -- cycle;
 \endgroup
  } %  revoir il y a plus simple que ce shift !!! 
%<--------------------------------------------------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkz@ClipSectorRotate(#1,#2)(#3){%
\begingroup
    \tkz@@CalcLength(#1,#2){tkz@radius} 
    \tkzFindSlopeAngle(#1,#2)\tkzGetAngle{tkz@FirstA} 
    \pgfmathadd{\tkz@FirstA}{#3}
    \edef\tkz@SecondA{\pgfmathresult} 
    \pgfmathgreaterthan{#3}{0}   
  \ifdim\pgfmathresult pt=1 pt\relax% 
   \tkz@ClipSectorRAngles(#1,\tkz@radius pt)(\tkz@FirstA,\tkz@SecondA)    
  \else
  \tkz@ClipSectorRAngles(#1,\tkz@radius pt)(\tkz@SecondA,\tkz@FirstA)      
  \fi
   \endgroup 
}
%<--------------------------------------------------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkz@ClipSectorN(#1,#2)(#3){%
\begingroup  
  \tkz@@CalcLength(#1,#2){tkz@radius}
  \tkzFindSlopeAngle(#1,#2)\tkzGetAngle{tkz@FirstAngle}  
  \tkzFindSlopeAngle(#1,#3)\tkzGetAngle{tkz@SecondAngle} 
  \tkz@ClipSectorRAngles(#1,\tkz@radius pt)(\tkz@FirstAngle,\tkz@SecondAngle)    
\endgroup  
} 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkz@numcs{0}
\pgfkeys{/clipsector/.cd,
      towards/.code               = {\def\tkz@numcs{0}},
      rotate/.code                = {\def\tkz@numcs{1}},
      R/.code                     = {\def\tkz@numcs{2}}, 
}
%<--------------------------------------------------------------------------–>
\def\tkzClipSector{\pgfutil@ifnextchar[{\tkz@ClipSector}{%
                                        \tkz@ClipSector[]}}

\def\tkz@ClipSector[#1](#2,#3)(#4){%
\pgfkeys{/clipsector/.cd}
\pgfqkeys{/clipsector}{#1}
\ifcase\tkz@numcs%
   \tkz@ClipSectorN(#2,#3)(#4)
  \or% 1
   \tkz@ClipSectorRotate(#2,#3)(#4)
  \or% 2 
   \tkz@ClipSectorRAngles(#2,#3)(#4)
  \fi 
} 
\makeatother
\endinput 

==> tikz-euclide/drawings/tkz-draw-eu-show.tex <==
%tkz-obj-eu-show.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-show.tex} 
\makeatletter  
%<--------------------------------------------------------------------------–>
% finding specific points in a triangle
%<--------------------------------------------------------------------------–>
%                            equi points
%<--------------------------------------------------------------------------–>
% draw  ? show ?   
\pgfkeys{/tkzEquiPt/.cd,
    from/.store in      = {\tkz@frompoint},
    dist/.store in      = {\tkz@equ@dist},
    show/.is if         = tkz@equi@show,
    dist                = 2,
    show                = false,
     /tkzEquiPt/.search also={/tikz}
}

\def\tkzDefEquiPoints{\pgfutil@ifnextchar[{\tkz@DefEquiPoints}{%
                                           \tkz@DefEquiPoints[]}}
\def\tkz@DefEquiPoints[#1](#2,#3){%
\pgfqkeys{/tkzEquiPt}{#1}
\begingroup
   \tkzUProjection(#2,#3)(\tkz@frompoint)
   \pgfnodealias{tkzEQpoint}{tkzPointResult}
   \tkzVecKNorm[\tkz@equ@dist](tkzEQpoint,#2)
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
   \tkzVecKNorm[-\tkz@equ@dist](tkzEQpoint,#2)
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
   \iftkz@equi@show
      \tkzCompass[compass style,#1](\tkz@frompoint,tkzFirstPointResult)
      \tkzCompass[compass style,#1](\tkz@frompoint,tkzSecondPointResult)
   \fi
\endgroup
}

%<---------------------------    The SHOW   --------------------------------–>
%<--------------------------------------------------------------------------–>
\global\def\tkz@numsh{0}
\pgfkeys{/show/.cd,
    mediator/.code             =          \def\tkz@numsh{0},
    perpendicular/.code args   =  {through #1} {\global\def\tkz@numsh{1}%
                                              \def\tkz@through{#1}}, 
    orthogonal/.code args      =  {through #1} {\global\def\tkz@numsh{1}%
                                                \global\def\tkz@through{#1}},
    parallel/.code args        = {through #1} {\global\def\tkz@numsh{2}%
                                            \global\def\tkz@through{#1}},    
    bisector/.code             =           \global\def\tkz@numsh{3},
    K/.code                    =   \def\tkz@koeff{#1}, 
    length/.code               =   \def\tkz@show@length{#1},
    ratio/.code                =   \def\tkz@show@ratio{#1},
    gap/.code                  =   \def\tkz@show@gap{#1},
    size/.code                 =   \def\tkz@show@size{#1},
    /show/.unknown/.code       =   {\let\searchname=\pgfkeyscurrentname
                                   \pgfkeysalso{\searchname/.try=#1,
                                   /tkzcompass/\searchname/.retry=#1,
                                   /tikz/\searchname/.retry=#1}%
                   }
         }    
\def\tkzShowLine{\pgfutil@ifnextchar[{\tkz@ShowLine}{\tkz@ShowLine[]}}
\def\tkz@ShowLine[#1](#2){% 
\begingroup
\pgfqkeys{/show}{ K   = 1,
          gap         = 2,
          ratio       = .5,
          length      = 1,
          size        = 1
          }  
\pgfqkeys{/show}{#1}  
\ifcase\tkz@numsh%
 % first case 0
  \tkzShowMediatorLine[#1](#2)  
 \or% 1
  \tkzShowOrthLine[#1](#2)(\tkz@through)  
 \or% 2
   \tkzShowLLLine[#1](#2)(\tkz@through)
 \or% 3
  \tkzShowBisectorLine[#1](#2)
\fi
\endgroup
}

\def\tkzShowMediatorLine{%
  \pgfutil@ifnextchar[{\tkz@ShowMediatorLine}{\tkz@ShowMediatorLine[]}}  
\def\tkz@ShowMediatorLine[#1](#2,#3){%
\begingroup
\pgfkeys{show/.cd,  gap    =  2,
          ratio            =  .5,
          length           =  1
    }
\pgfkeys{show/.cd,#1}  
  \path (#2) -- (#3) coordinate[pos=.5](tkzmidpoint);
  \tkzURotateAngle(#2,60)(#3)       
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult} 
  \tkzURotateAngle(#3,60)(#2)      
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult} 
  \tkz@VecKOrthNorm[1](tkzmidpoint,#2)     
   \pgfnodealias{MED@tmp1}{tkzPointResult} 
  \tkz@VecKOrthNorm[1](tkzmidpoint,#3)      
  \pgfnodealias{MED@tmp2}{tkzPointResult} 
  \tkz@VecKNorm[\tkz@show@gap](tkzmidpoint,MED@tmp1)  
  \pgfnodealias{MED@1}{tkzPointResult} 
  \tkz@VecKNorm[\tkz@show@gap](tkzmidpoint,MED@tmp2) 
   \pgfnodealias{MED@2}{tkzPointResult} 
  \tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](#2,MED@1)
  \tkzCompass[compass style,#1](#3,MED@1)
  \tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](#2,MED@2)
  \tkzCompass[compass style,#1](#3,MED@2)
\endgroup
}

\def\tkzShowLLLine{\pgfutil@ifnextchar[{\tkz@ShowLLLine}{\tkz@ShowLLLine[]}}  
\def\tkz@ShowLLLine[#1](#2,#3)(#4){%
\begingroup
\pgfkeys{show/.cd,gap=2,ratio=.75,length=1}
\pgfkeys{show/.cd,#1}   
    \tkz@VecKCoLinear[1](#2,#3,#4)
     \pgfnodealias{tkz@lltmp}{tkzPointResult}
    \tkzCompass[compass style,#1](#4,tkz@lltmp)
    \tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](#3,tkz@lltmp)
\endgroup
} 

%<--------------------------------------------------------------------------–>
%                        tkzLineOrth 
%<--------------------------------------------------------------------------–>
% pas de projection ortho car le point peut être sur la droite.
% manque les tests . Il faudrait voir si on peut projeter et choisir
\def\tkzShowOrthLine{\pgfutil@ifnextchar[{\tkz@ShowOrthLine}{\tkz@ShowOrthLine[]}} 
\def\tkz@ShowOrthLine[#1](#2,#3)(#4){% 
\begingroup
\pgfkeys{show/.cd,  
          ratio   = .75,
          length  = 1,
          gap     = -1,
          size    = 1} 
\pgfkeys{show/.cd,#1}
    \tkzDefPointWith(#2,#3)               
    \pgfnodealias{tkz@OLtmp}{tkzPointResult}
    \tkz@VecKCoLinear[1](#2,tkz@OLtmp,#4)      
    \pgfnodealias{tkzPointCo}{tkzPointResult}
    \tkzInterLL(#2,#3)(#4,tkzPointCo)
    \pgfnodealias{tkzPOpoint}{tkzPointResult}
    \tkz@@CalcLength(#4,tkzPOpoint){tkz@mathLen}
    \tkz@VecKNorm[1](#2,#3)
    \pgfnodealias{PO@tmp}{tkzPointResult}
    \tkz@VecKCoLinear[1](#2,PO@tmp,tkzPOpoint)  
    \pgfnodealias{PO@tmp2}{tkzPointResult}
    \tkz@VecKCoLinear[-1](#2,PO@tmp,tkzPOpoint)
    \pgfnodealias{PO@tmp1}{tkzPointResult}
    \tkz@VecKCoLinear[\tkz@show@size](tkzPOpoint,PO@tmp1,tkzPOpoint) 
    \pgfnodealias{PO@1}{tkzPointResult}
    \tkz@VecKCoLinear[\tkz@show@size](tkzPOpoint,PO@tmp2,tkzPOpoint)
    \pgfnodealias{PO@2}{tkzPointResult}
    \ifdim\tkz@mathLen pt>10 pt\relax
        \tkz@VecKNorm[1](#4,tkzPOpoint)
        \pgfnodealias{PO@tmp1}{tkzPointResult}
      \else
        \tkz@VecKOrthNorm[1](tkzPOpoint,PO@2)
        \pgfnodealias{PO@tmp1}{tkzPointResult}
     \fi
    \tkz@VecKCoLinear[-\tkz@show@gap](PO@tmp1,tkzPOpoint,tkzPOpoint)
    \pgfnodealias{PO@3}{tkzPointResult}
    \tkzCompass[compass style,#1,length=\tkz@show@ratio *\tkz@show@length](#4,PO@1)
    \tkzCompass[compass style,#1,length=\tkz@show@ratio *\tkz@show@length](#4,PO@2)
    \tkzCompass[compass style,#1,length=\tkz@show@ratio *\tkz@show@length](PO@1,PO@3)
    \tkzCompass[compass style,#1,length=\tkz@show@length](PO@2,PO@3) 
\endgroup
}    
%<-------------------------------------------------------------------------–> 
%    bisector Line
%<-------------------------------------------------------------------------–> 
\def\tkzShowBisectorLine{%
    \pgfutil@ifnextchar[{\tkz@ShowBisectorLine}{\tkz@ShowBisectorLine[]}}   
\def\tkz@ShowBisectorLine[#1](#2,#3,#4){% 
\begingroup
\pgfkeys{show/.cd,  gap   = 2,
          ratio           =.  5,
          length          = 1,
          size            = 1
          }
\pgfkeys{show/.cd,#1}    
  \tkzVecKNorm(#3,#2)           
    \pgfnodealias{tkz@pt1}{tkzPointResult}  
  \tkzVecKNorm(#3,#4)           
    \pgfnodealias{tkz@pt2}{tkzPointResult}
  \tkzDefMidPoint(tkz@pt1,tkz@pt2)    
    \pgfnodealias{tkz@pt3}{tkzPointResult}
  \tkzDefEquilateral(tkz@pt2,tkz@pt1)   
    \pgfnodealias{tkz@pt4}{tkzPointResult}
  \tkzDefMidPoint(tkz@pt3,tkz@pt4)    
    \pgfnodealias{tkz@ptm}{tkzPointResult}
  \tkzVecKNorm(#3,tkz@ptm)        
    \pgfnodealias{tkzBisPoint}{tkzPointResult}
  \tkzVecKNorm[\tkz@show@size](#3,#2)   
    \pgfnodealias{BI@1}{tkzPointResult}
  \tkzVecKNorm[\tkz@show@size](#3,#4)   
    \pgfnodealias{BI@2}{tkzPointResult}  
  \tkzVecK[\tkz@show@gap](#3,tkzBisPoint) 
    \pgfnodealias{tkzBisPoint}{tkzPointResult}
  \tkzCompass[compass style,#1,length=\tkz@show@ratio *\tkz@show@length](#3,BI@1)
  \tkzCompass[compass style,#1,length=\tkz@show@ratio *\tkz@show@length](#3,BI@2)
  \tkzCompass[compass style,#1,length=\tkz@show@length](BI@1,tkzBisPoint)
  \tkzCompass[compass style,#1,length=\tkz@show@ratio *\tkz@show@length](BI@2,tkzBisPoint)  
\endgroup    
}
%<--------------------------------------------------------------------------–>
%                        Transformations Géométriques
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                   The SHOW
%<--------------------------------------------------------------------------–>
\def\tkz@numst{0}
\pgfkeys{/showtsf/.cd,
 reflection/.code args={over #1--#2}{%
                  \def\tkzdeb{#1}
                  \def\tkzfin{#2}
                  \def\tkz@numst{0}},  
 symmetry/.code args={center #1}{%
                  \def\tkzcenter{#1} 
                  \def\tkz@numst{1}},
 projection/.code args={onto #1--#2}{%
                  \def\tkzdeb{#1}
                  \def\tkzfin{#2}  
                  \def\tkz@numst{2}},
translation/.code args={from #1 to #2}{%
                  \def\tkzfrom{#1}%
                  \def\tkzto{#2}%
                  \def\tkz@numst{3}},  
  K/.code                = \def\tkz@koeff{#1}, 
  length/.code           = \def\tkz@show@length{#1},
  ratio/.code            = \def\tkz@show@ratio{#1},
  gap/.code              = \def\tkz@show@gap{#1},
  size/.code             = \def\tkz@show@size{#1},
/showtsf/.unknown/.code  = {\let\searchname=\pgfkeyscurrentname
                            \pgfkeysalso{\searchname/.try=#1,
                                /tkzcompass/\searchname/.retry=#1,
                                /tikz/\searchname/.retry=#1}}
}  
%<--------------------------------------------------------------------------–>
\def\tkzShowTransformation{\pgfutil@ifnextchar[{\tkz@ShowTransformation}{%
                                                 \tkz@ShowTransformation[]}}
\def\tkz@ShowTransformation[#1](#2){% 
\begingroup
 \pgfqkeys{/showtsf}{K=1,gap=2,size=1,ratio=.5,length=1}  
 \pgfqkeys{/showtsf}{#1} 
 \pgfinterruptboundingbox  
\ifcase\tkz@numst%
 % first case 0
  \tkzShowSymOrth[#1](\tkzdeb,\tkzfin)(#2)   
  \or% 1
  \tkzShowCSym[#1](\tkzcenter)(#2)
  \or% 2
  \tkzShowProjection[#1](\tkzdeb,\tkzfin)(#2) 
  \or% 3
  \tkzShowTranslation[#1](\tkzfrom,\tkzto)(#2) 
  \fi  
  \endpgfinterruptboundingbox   
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzShowTranslation{\pgfutil@ifnextchar[{\tkz@ShowTranslation}{%
                                          \tkz@ShowTranslation[]}}  

\def\tkz@ShowTranslation[#1](#2,#3)(#4){%
\begingroup
\tkz@VecKCoLinear[1](#2,#3,#4) \pgfnodealias{tkz@lltmp}{tkzPointResult}
\tkzCompass[compass style,#1](#4,tkz@lltmp)
\tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](#3,tkz@lltmp)
\endgroup}
%<--------------------------------------------------------------------------–>
\def\tkzShowSymOrth{\pgfutil@ifnextchar[{\tkz@ShowSymOrth}{%
                                          \tkz@ShowSymOrth[]}}  
\def\tkz@ShowSymOrth[#1](#2,#3)(#4){%
\begingroup
  \pgfpointdiff{\pgfpointanchor{#2}{center}}%
               {\pgfpointanchor{#3}{center}}%
  \tkz@ax =\pgf@y%
  \tkz@ay =\pgf@x%
  \path[coordinate](#4)--++(-\tkz@ax,\tkz@ay) coordinate (tkz@point);
  \tkzInterLL(#2,#3)(#4,tkz@point)  
  \pgfnodealias{tkzPointofSym}{tkzPointResult}
  \tkz@VecK[2](#4,tkzPointofSym) 
  \pgfnodealias{tkz@pointtsf}{tkzPointResult}  
  \tkzCompass[compass style,#1](#2,#4)
  \tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](#3,#4)
  \tkzCompass[compass style,#1](#2,tkz@pointtsf)
  \tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](#3,tkz@pointtsf)   
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzShowCSym{\pgfutil@ifnextchar[{\tkz@ShowCSym}{\tkz@ShowCSym[]}}
 
\def\tkz@ShowCSym[#1](#2)(#3){%
\begingroup
 \pgfpointdiff{\pgfpointanchor{#2}{center}}%
              {\pgfpointanchor{#3}{center}}%
 \tkz@ax=\pgf@x%
 \tkz@ay=\pgf@y%
\path[coordinate](#2)--++(-\tkz@ax,-\tkz@ay) coordinate (tkz@pointtsf); 
       \tkzCompass[compass style,#1](#2,tkz@pointtsf)
       \tkzCompass[compass style,#1](#2,#3)
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzShowProjection{\pgfutil@ifnextchar[{\tkz@ShowProjection}{%
                                          \tkz@ShowProjection[]}}  
\def\tkz@ShowProjection[#1](#2,#3)(#4){%
\begingroup 
  \pgfpointdiff{\pgfpointanchor{#2}{center}}%
               {\pgfpointanchor{#3}{center}}%
  \tkz@ax =\pgf@y%
  \tkz@ay =\pgf@x%     
  \path[coordinate](#4)--++(-\tkz@ax,\tkz@ay) coordinate (tkz@point);
  \tkzInterLL(#2,#3)(#4,tkz@point)          
  \pgfnodealias{tkz@pointtsf}{tkzPointResult}
  \tkz@VecKCoLinear[1](#2,#3,tkz@pointtsf)        
  \pgfnodealias{SO@tmp1}{tkzPointResult}
  \tkz@VecKCoLinear[-1](#2,#3,tkz@pointtsf)
  \pgfnodealias{SO@tmp2}{tkzPointResult}
  \tkz@VecKNorm[\tkz@show@size](tkz@pointtsf,SO@tmp1)
  \pgfnodealias{SO@1}{tkzPointResult}
  \tkz@VecKNorm[\tkz@show@size](tkz@pointtsf,SO@tmp2)
  \pgfnodealias{SO@2}{tkzPointResult}
  \tkz@VecKNorm[-\tkz@show@gap](tkz@pointtsf,#4)
  \pgfnodealias{SO@3}{tkzPointResult}
  \tkzCompass[compass style,#1](#4,SO@1)
  \tkzCompass[compass style,#1](#4,SO@2)
  \tkzCompass[compass style,#1](SO@1,SO@3)
  \tkzCompass[compass style,#1,length=\tkz@show@ratio*\tkz@show@length](SO@2,SO@3)
\endgroup
}   
\makeatother  
\endinput

==> tikz-euclide/libs/tkz-lib-eu-marks.tex <==
% tkz-eu-lib-marks.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-lib-eu-marks.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%  Création des symboles
%<--------------------------------------------------------------------------–>
\def\tkz@undefined{none}    
% double bar
\pgfdeclareplotmark{||}
{%
  \pgfpathmoveto{\pgfqpoint{2\pgflinewidth}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{-\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-2\pgflinewidth}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{-2\pgflinewidth}{-\pgfplotmarksize}}
  \pgfusepathqstroke
}
%triple bar
\pgfdeclareplotmark{|||}
{%
  \pgfpathmoveto{\pgfqpoint{0 pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0 pt}{-\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-3\pgflinewidth}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{-3\pgflinewidth}{-\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{3\pgflinewidth}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{3\pgflinewidth}{-\pgfplotmarksize}}
  \pgfusepathqstroke
} 
% An bar slant

\pgfdeclareplotmark{s|}
{%
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}%
                           {-.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}%
                           {.70710678\pgfplotmarksize}}
  \pgfusepathqstroke
} 

% An double bar slant

\pgfdeclareplotmark{s||}
{%
 \pgfpathmoveto{\pgfqpoint{-0.75\pgfplotmarksize}{-\pgfplotmarksize}}
 \pgfpathlineto{\pgfqpoint{0.25\pgfplotmarksize}{\pgfplotmarksize}} 
 \pgfpathmoveto{\pgfqpoint{0\pgfplotmarksize}{-\pgfplotmarksize}}
 \pgfpathlineto{\pgfqpoint{1\pgfplotmarksize}{\pgfplotmarksize}} 
 \pgfusepathqstroke
}   
\pgfdeclareplotmark{s|||}
{%
 \pgfpathmoveto{\pgfqpoint{-0.75\pgfplotmarksize}{-\pgfplotmarksize}}
 \pgfpathlineto{\pgfqpoint{0.25\pgfplotmarksize}{\pgfplotmarksize}} 
 \pgfpathmoveto{\pgfqpoint{0\pgfplotmarksize}{-\pgfplotmarksize}}
 \pgfpathlineto{\pgfqpoint{1\pgfplotmarksize}{\pgfplotmarksize}}
 \pgfpathmoveto{\pgfqpoint{0.75\pgfplotmarksize}{-\pgfplotmarksize}}
 \pgfpathlineto{\pgfqpoint{1.75\pgfplotmarksize}{\pgfplotmarksize}} 
 \pgfusepathqstroke
} 
% z
\pgfdeclareplotmark{z}
{%
  \pgfpathmoveto{\pgfqpoint{0.75\pgfplotmarksize}{-\pgfplotmarksize}} 
  \pgfpathlineto{\pgfqpoint{-0.75\pgfplotmarksize}{-\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfplotmarksize}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{-0.75\pgfplotmarksize}{\pgfplotmarksize}}
  \pgfusepathqstroke
}
% s
\pgfdeclareplotmark{s}
{%
   \pgfpathmoveto{\pgfqpoint{0pt}{0pt}} 
   \pgfpathcurveto
       {\pgfpoint{0pt}{0pt}}
       {\pgfpoint{-\pgfplotmarksize}{\pgfplotmarksize}}
       {\pgfpoint{\pgfplotmarksize}{\pgfplotmarksize}}
   \pgfpathmoveto{\pgfqpoint{0pt}{0pt}} 
    \pgfpathcurveto
       {\pgfpoint{0pt}{0pt}}
       {\pgfpoint{\pgfplotmarksize}{-\pgfplotmarksize}}
       {\pgfpoint{-\pgfplotmarksize}{-\pgfplotmarksize}} 
    \pgfusepathqstroke
}  
% infinity
\pgfdeclareplotmark{oo}
{%
   \pgfpathmoveto{\pgfqpoint{0pt}{0pt}} 
   \pgfpathcurveto
       {\pgfpoint{0pt}{0pt}}
       {\pgfpoint{.5\pgfplotmarksize}{1\pgfplotmarksize}}
       {\pgfpoint{\pgfplotmarksize}{0pt}}
   \pgfpathmoveto{\pgfqpoint{0pt}{0pt}} 
    \pgfpathcurveto
       {\pgfpoint{0pt}{0pt}}
       {\pgfpoint{-.5\pgfplotmarksize}{1\pgfplotmarksize}}
       {\pgfpoint{-\pgfplotmarksize}{0pt}}  
   \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}  
      \pgfpathcurveto
       {\pgfpoint{0pt}{0pt}}
       {\pgfpoint{.5\pgfplotmarksize}{-1\pgfplotmarksize}}
       {\pgfpoint{\pgfplotmarksize}{0pt}}
   \pgfpathmoveto{\pgfqpoint{0pt}{0pt}} 
    \pgfpathcurveto
       {\pgfpoint{0pt}{0pt}}
       {\pgfpoint{-.5\pgfplotmarksize}{-1\pgfplotmarksize}}
       {\pgfpoint{-\pgfplotmarksize}{0pt}}      
    \pgfusepathqstroke
} 
\makeatother
\endinput

==> tikz-euclide/libs/tkz-lib-eu-shape.tex <==
 % tkz-lib-eu-shape.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-lib-eu-shape.tex}   
%<--------------------------------------------------------------------------–>
%  Création des symboles
%<--------------------------------------------------------------------------–>
\makeatletter
% define a new shape for the points
\pgfdeclareshape{cross}
{%
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \foregroundpath{
% store lower right in xa/ya and upper right in xb/yb
  \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
  \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
  \pgfpathmoveto{\pgfqpoint{0 pt}{\pgf@ya}}
  \pgfpathlineto{\pgfqpoint{0 pt}{\pgf@yb}}
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{0 pt}}
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{0 pt}}
 }
}
\makeatother
\endinput

==> tikz-euclide/obj-lua/tkz-obj-lua-circles.tex <==
% tkz-obj-lua-circles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-lua-circles.tex} 
\makeatletter
%<--------------------------------------------------------------------------–>
%            tkzCircle center and one point 
%<--------------------------------------------------------------------------–>
% attention radius circle is defined by center and a point on the circle
% R defined by center and the value of the radius
% no need to define a circle with R tikz uses this method.
% through instead of radius
\def\tkz@numc{0}
\pgfkeys{/tkzcircle/.cd,
      R/.code                                   = \def\tkz@numc{0},
      diameter/.code                            = \def\tkz@numc{1},
      circum/.code                              = \def\tkz@numc{2},
      in/.code                                  = \def\tkz@numc{3},
      ex/.code                                  = \def\tkz@numc{4},
      euler/.code                               = \def\tkz@numc{5},
      nine/.code                                = \def\tkz@numc{5},
      apollonius/.code                          = \def\tkz@numc{6},
      spieker/.code                             = \def\tkz@numc{7},
      orthogonal from/.code args                = {#1}{\gdef\tkz@numc{8}
                                                   \def\tkz@ptfrom{#1}}, 
      orthogonal through/.code args             = {#1 and #2}{\gdef\tkz@numc{9}
                                                   \def\tkz@ptone{#1}
                                                   \def\tkz@pttwo{#2}},
      K/.code                                   = \def\tkz@koeff{#1},
      K                                         =  1,
      circum
      } 
\def\tkzDefCircle{\pgfutil@ifnextchar[{\tkz@DefCircle}{\tkz@DefCircle[]}}
\def\tkz@DefCircle[#1](#2){% 
\begingroup  
\pgfqkeys{/tkzcircle}{#1}  
\ifcase\tkz@numc%
  \tkzDefCircleR(#2)
  \or% 1 
  \tkzDefCircleD(#2)  
  \or% 2
  \tkzDefCircumCircle(#2) 
  \or% 3
  \tkzDefInCircle(#2) 
  \or% 4
  \tkzDefExCircle(#2) 
  \or% 5
  \tkzDefEulerCircle(#2)
  \or% 6
  \tkzDefApolloniusCircle(#2) 
  \or% 7
  \tkzDefSpiekerCircle(#2)
   \or% 8
  \tkzDefOrthogonalCircle(#2,\tkz@ptfrom)
   \or% 9
  \tkzDefOrthoThroughCircle(#2,\tkz@ptone,\tkz@pttwo)
     \fi    
\endgroup
}
%for compatibility
%<--------------------------------------------------------------------------–>
%                     R
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleR(#1,#2){% 
\begingroup 
   \edef\tkzLengthResult{\fpeval{round(#2,5)}}
   \global\let\tkzLengthResult\tkzLengthResult
   \path (#1)--++(\tkzLengthResult,0) coordinate (tkzSecondPointResult);
   \tkzRenamePoint(tkzSecondPointResult){tkzPointResult}
\endgroup
} 

%<--------------------------------------------------------------------------–>
%              Diameter Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleD(#1,#2){% 
\begingroup
  \tkzDefMidPoint(#1,#2)
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \pgfnodealias{tkzSecondPointResult}{#2}
  \tkz@@CalcLengthcm(#1,tkzPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Circum Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefCircumCircle(#1,#2,#3){%
\begingroup
  \tkzCircumCenter(#1,#2,#3)
  \tkzRenamePoint(tkzPointResult){tkzFirstPointResult}
  \tkzRenamePoint(#1){tkzSecondPointResult}
  \tkz@@CalcLengthcm(#1,tkzPointResult){tkzLengthResult}%3.06 add [cm]
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              In(scribe) Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefInCircle(#1,#2,#3){%
\begingroup
  \tkzInCenter(#1,#2,#3) 
  \pgfnodealias{tkz@incenter}{tkzPointResult}
  \tkzUProjection(#1,#3)(tkz@incenter) 
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
  \tkz@@CalcLengthcm(tkzPointResult,tkz@incenter){tkzLengthResult}
  \pgfnodealias{tkzPointResult}{tkz@incenter}
  \pgfnodealias{tkzFirstPointResult}{tkz@incenter}
\endgroup
}  
%<--------------------------------------------------------------------------–>
%              Ex(scribe) Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefExCircle(#1,#2,#3){%
\begingroup
  \tkzExCenter(#1,#2,#3) 
  \pgfnodealias{tkz@excenter}{tkzPointResult}
  \tkzUProjection(#1,#3)(tkz@excenter)
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
  \tkz@@CalcLengthcm(tkzPointResult,tkz@excenter){tkzLengthResult}% for tkzGetLength
  \pgfnodealias{tkzPointResult}{tkz@excenter}
  \pgfnodealias{tkzFirstPointResult}{tkz@excenter}  
\endgroup
}
%<--------------------------------------------------------------------------–>
%              Radius Ex Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefExRadius(#1,#2,#3){%
\begingroup
   \tkzExCenter(#1,#2,#3)
   \tkzUProjection(#1,#3)(tkzPointResult)
\endgroup
}    
%<--------------------------------------------------------------------------–>
% The nine-point circle, also called Euler's circle or the Feuerbach circle  
% best way Ma,Mb,Mc circum center  2020
%<--------------------------------------------------------------------------–>
\def\tkzDefEulerCircle(#1,#2,#3){%
\begingroup
 \tkzDefMidPoint(#1,#2) \pgfnodealias{tkz@e1}{tkzPointResult}
 \tkzDefMidPoint(#2,#3) \pgfnodealias{tkz@e2}{tkzPointResult}
 \tkzDefMidPoint(#1,#3) \pgfnodealias{tkz@e3}{tkzPointResult}
 \tkzCircumCenter(tkz@e1,tkz@e2,tkz@e3) 
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}  
 \tkzRenamePoint(tkz@e1){tkzSecondPointResult}
 \tkz@@CalcLengthcm(tkzPointResult,tkz@e1){tkzLengthResult}
\endgroup
} 
\let\tkzDefNinePointsCircle\tkzEulerCircle%
\let\tkzFeuerBachCircle\tkzEulerCircle%  

\def\tkzDefEulerRadius(#1,#2,#3){%
\begingroup
   \tkzEulerCenter(#1,#2,#3)
   \pgfnodealias{eur@pta}{tkzPointResult}   
   \tkzDefMidPoint(#1,#2)  
   \tkz@@CalcLengthcm(eur@pta,tkzPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>
%                     Apollonius circle
%<--------------------------------------------------------------------------–>
\def\tkzDefApolloniusCircle(#1,#2){%
\begingroup
  \tkzDefBarycentricPointTwo(#1,1,#2,\tkz@koeff)   
  \pgfnodealias{apo@pta}{tkzPointResult} 
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}  
  \tkzDefBarycentricPointTwo(#1,1,#2,-\tkz@koeff)  
  \pgfnodealias{apo@ptb}{tkzPointResult} 
  \tkzDefMidPoint(apo@pta,apo@ptb)  
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult} 
  \tkz@@CalcLengthcm(tkzFirstPointResult,apo@pta){tkzLengthResult}  
  \pgfnodealias{tkzThirdPointResult}{apo@ptb} 
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefOrthogonalCircle(#1,#2,#3){%   
\begingroup
   \tkzTgtFromP(#1,#2)(#3)
   \tkz@@CalcLengthcm(#1,tkzFirstPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzDefOrthoThroughCircle(#1,#2,#3,#4){%  
\begingroup
  \tkz@@CalcLengthcm(#1,#3){tkz@lnb}%
  \edef\tkz@lnc{\fpeval{1/\tkz@lnb}}
  \tkzVecKNorm[\tkz@lnc](#1,#3) 
  \pgfnodealias{tkz@PointResult}{tkzPointResult}
  \tkzCircumCenter(tkz@PointResult,#3,#4)
  \tkz@@CalcLengthcm(tkzPointResult,#3){tkzLengthResult}
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \pgfnodealias{tkzSecondPointResult}{#3}
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Spieker Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefSpiekerCircle(#1,#2,#3){%
\begingroup
  \tkzSpiekerCenter(#1,#2,#3)
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \tkzUProjection(tkz@m1,tkz@m2)(tkzPointResult)
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
  \tkz@@CalcLength(tkzSecondPointResult,tkzFirstPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>

%<--------------------------------------------------------------------------–>
%              End Def Circle
%<--------------------------------------------------------------------------–>  
\makeatother 
\endinput

==> tikz-euclide/obj-lua/tkz-obj-lua-points-by.tex <==
% tkz-tools-lua-points-by.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-lua-points-by.tex}  
\makeatletter
%<--------------------------------------------------------------------------–>
%                        Transformations Géométriques
%<--------------------------------------------------------------------------–>
\def\tkz@numtrsf{0}
\pgfkeys{/tkzDefPointBy/.cd,
 translation/.code args={from #1 to #2}{               \def\tkzfrom{#1}%
                                                       \def\tkzto{#2}%
                                                       \def\tkz@numtrsf{0}},
 homothety/.code args={center #1 ratio #2}{            \def\tkzcenter{#1}%
                                                       \def\tkzratio{#2}%
                                                       \def\tkz@numtrsf{1}},
 reflection/.code args={over #1--#2}{                  \def\tkzdeb{#1}%
                                                       \def\tkzfin{#2}%
                                                       \def\tkz@numtrsf{2}},
 symmetry/.code args={center #1}{                      \def\tkzcenter{#1}%
                                                       \def\tkz@numtrsf{3}},
 projection/.code args={onto #1--#2}{                  \def\tkzdeb{#1}%
                                                       \def\tkzfin{#2}%  
                                                       \def\tkz@numtrsf{4}}, 
 rotation/.code args={center #1 angle #2}{             \def\tkzcenter{#1}%
                                                       \def\tkzangle{#2}%
                                                       \def\tkz@numtrsf{5}},
 rotation in rad/.code args={center #1 angle #2}{      \def\tkzcenter{#1}%
                                                       \def\tkzangle{#2}%
                                                       \def\tkz@numtrsf{6}},
 inversion/.code args={center #1 through #2}{          \def\tkzcenter{#1}%
                                                       \def\tkzpoint{#2}%
                                                       \def\tkz@numtrsf{7}},
 inversion negative/.code args={center #1 through #2}{ \def\tkzcenter{#1}%
                                                       \def\tkzpoint{#2}%
                                                       \def\tkz@numtrsf{8}},
 rotation with nodes/.code  args={center #1 from #2 to #3}{  \def\tkzcenter{#1}%
                                                            \def\tkzfrom{#2}%
                                                            \def\tkzto{#3}%
                                                            \def\tkz@numtrsf{9}}
}
%<--------------------------------------------------------------------------–>
\def\tkzDefPointBy{\pgfutil@ifnextchar[{\tkz@DefPointBy}{\tkz@DefPointBy[]}}
\def\tkz@DefPointBy[#1](#2){% 
\begingroup 
\pgfqkeys{/tkzDefPointBy}{#1}    
 \ifcase\tkz@numtrsf%
%  % first case 0   
   \tkzUTranslation(\tkzfrom,\tkzto)(#2) 
\or% 1
   \tkzUHomo(\tkzcenter,\tkzratio)(#2)
\or% 2
   \tkzUSymOrth(\tkzdeb,\tkzfin)(#2) 
\or% 3
   \tkzUCSym(\tkzcenter)(#2)
\or% 4
   \tkzUProjection(\tkzdeb,\tkzfin)(#2)  
\or% 5  
   \tkzURotateAngle(\tkzcenter,\tkzangle)(#2)
\or% 6 
   \tkzURotateInRad(\tkzcenter,\tkzangle)(#2)
\or% 7
   \tkzUInversePoint(\tkzcenter,\tkzpoint)(#2)     
\or% 8
   \tkzUInverseNegativePoint(\tkzcenter,\tkzpoint)(#2)   
\or% 9
   \tkzURotateWithNodes(\tkzcenter,\tkzfrom,\tkzto)(#2)
\fi   
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefPointsBy{\pgfutil@ifnextchar[{\tkz@DefPointsBy}{\tkz@DefPointsBy[]}}
\def\tkz@DefPointsBy[#1](#2)#3{% 
\begingroup
\pgfqkeys{/tkzDefPointBy}{#1}  
\ifcase\tkz@numtrsf%
 % first case 0
   \tkzTranslation(\tkzfrom,\tkzto)(#2){#3}  
 \or% 1
   \tkzHomo(\tkzcenter,\tkzratio)(#2){#3}
 \or% 2
   \tkzSymOrth(\tkzdeb,\tkzfin)(#2){#3} 
 \or% 3
   \tkzCSym(\tkzcenter)(#2){#3}
 \or% 4
   \tkzProjection(\tkzdeb,\tkzfin)(#2){#3}
 \or% 5
   \tkzRotateAngle(\tkzcenter,\tkzangle)(#2){#3}
 \or% 6
   \tkzRotateInRad(\tkzcenter,\tkzangle)(#2){#3}
 \or% 7
   \tkzInversePoint(\tkzcenter,\tkzpoint)(#2){#3}    
 \or% 8
   \tkzInverseNegativePoint(\tkzcenter,\tkzpoint)(#2){#3}
   \or% 9
 \tkzRotateWithNodes(\tkzcenter,\tkzfrom,\tkzto)(#2){#3}
\fi    
\endgroup
} 

%<--------------------------------------------------------------------------–>

\def\ExtractPoint#1,#2\@nil{% 
\xdef\tkz@LastList{#2}
\xdef\tkz@FirstPoint{#1}  
} 
\def\FirstPointInList#1{% 
\edef\tkz@templist{#1,}
\expandafter\ExtractPoint\tkz@templist\@nil
}
%<--------------------------------------------------------------------------–>
%  Translation par rapport à un point
%<--------------------------------------------------------------------------–>
\def\tkzTranslation(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
\foreach\PT in {#3}{%
   \FirstPointInList\tkz@LastList
    \ifx\tkz@FirstPoint\tkzutil@empty  
      \def\tkz@pointtsf{\PT '}
    \else
      \def\tkz@pointtsf{\tkz@FirstPoint}
    \fi 
   \tkz@VecCoLinear(#1,#2,\PT) 
    \pgfnodealias{\tkz@pointtsf}{tkzPointResult}       
   }  
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUTranslation(#1,#2)(#3){%
\begingroup 
  \tkz@VecCoLinear(#1,#2,#3)% 
\endgroup
}  

%<--------------------------------------------------------------------------–>
%  Symétrie par rapport à un point Homo with (-1) 
% #2 le centre #3 l'antécédent 
%<--------------------------------------------------------------------------–>
\def\tkzCSym(#1)(#2)#3{%
\begingroup
\gdef\tkz@LastList{#3}
 \foreach\PointCS in {#2}{%
   \FirstPointInList\tkz@LastList
   \ifx\tkz@FirstPoint\tkzutil@empty  
      \xdef\tkz@pointtsf{\PointCS '}
   \else
      \xdef\tkz@pointtsf{\tkz@FirstPoint}
   \fi 
     \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                  {\pgfpointanchor{\PointCS}{center}}%
     \tkz@ax=\pgf@x%
     \tkz@ay=\pgf@y%
 \pgfinterruptboundingbox
     \path(#1)--++(-\tkz@ax,-\tkz@ay)coordinate (\tkz@pointtsf); 
  \endpgfinterruptboundingbox
}       
\endgroup 
}
%<--------------------------------------------------------------------------–>
\def\tkzUCSym(#1)(#2){%
\begingroup
    \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                 {\pgfpointanchor{#2}{center}}%
    \tkz@ax=\pgf@x%
    \tkz@ay=\pgf@y%
   \path(#1)--++(-\tkz@ax,-\tkz@ay)coordinate (tkzPointResult); 
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%  Symétrie orthogonale par rapport à une droite
%<--------------------------------------------------------------------------–> 
\def\tkzSymOrth(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointSO in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \def\tkz@pointtsf{\PointSO '}
      \else
         \def\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
  \tkzUSymOrth(#1,#2)(\PointSO)    
  \pgfnodealias{\tkz@pointtsf}{tkzPointResult} 
  }    
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUSymOrth(#1,#2)(#3){%
\begingroup
   \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                {\pgfpointanchor{#2}{center}}%
   \tkz@ax =\pgf@y%
   \tkz@ay =\pgf@x%  
   \pgfinterruptboundingbox
   \path[coordinate] (#3)--++(-\tkz@ax,\tkz@ay) coordinate  (tkz@point);
     \endpgfinterruptboundingbox
   \tkzInterLL(#1,#2)(#3,tkz@point)
   \pgfnodealias{tkzPointofSym}{tkzPointResult}
   \tkz@VecK[2](#3,tkzPointofSym)
\endgroup
}

%<--------------------------------------------------------------------------–>
%  Projection orthogonale sur une droite
%<--------------------------------------------------------------------------–>
\def\tkzProjection(#1,#2)(#3)#4{%
\begingroup
\gdef\tkz@LastList{#4}
    \foreach\PointPJ in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty
         \def\tkz@pointtsf{\PointPJ '}
      \else
         \def\tkz@pointtsf{\tkz@FirstPoint}
      \fi
  \tkzUProjection(#1,#2)(\PointPJ)
  \pgfnodealias{\tkz@pointtsf}{tkzPointResult}
  }
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUProjection(#1,#2)(#3){%
\begingroup 
  \pgfpointdiff{\pgfpointanchor{#1}{center}}%
               {\pgfpointanchor{#2}{center}}%
  \tkz@ax =\pgf@y%
  \tkz@ay =\pgf@x%
  \pgfinterruptboundingbox
    \path[coordinate](#3)--++(-\tkz@ax,\tkz@ay) coordinate (tkz@point);
    \tkzInterLL(#1,#2)(#3,tkz@point)% définit tkzPointResult 
  \endpgfinterruptboundingbox
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkz@Projection(#1,#2)(#3)#4{%
\begingroup 
  \pgfpointdiff{\pgfpointanchor{#1}{center}}%
               {\pgfpointanchor{#2}{center}}%
  \tkz@ax =\pgf@y%
  \tkz@ay =\pgf@x%
   \pgfinterruptboundingbox
  \path[coordinate](#3)--++(-\tkz@ax,\tkz@ay) coordinate (tkz@point);
   \endpgfinterruptboundingbox
  \tkz@InterLL(#1,#2)(#3,tkz@point){#4}% définit tkzPointResult 
\endgroup
}
%<--------------------------------------------------------------------------–>
%  Homothétie par rapport à un point
%<--------------------------------------------------------------------------–>
\def\tkzHomo(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
\foreach\PointHO in {#3}{%
  \FirstPointInList\tkz@LastList
  \ifx\tkz@FirstPoint\tkzutil@empty  
     \xdef\tkz@pointtsf{\PointHO '}
  \else
     \xdef\tkz@pointtsf{\tkz@FirstPoint}
  \fi 
   \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                {\pgfpointanchor{\PointHO}{center}}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y% 
  \pgfmathparse{#2}
  \edef\tkz@coeff{\pgfmathresult}%
  \pgfinterruptboundingbox
  \path[coordinate](#1)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)%
        coordinate(\tkz@pointtsf);
 \endpgfinterruptboundingbox
  }  
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUHomo(#1,#2)(#3){%
\begingroup 
 \pgfpointdiff{\pgfpointanchor{#1}{center}}%
              {\pgfpointanchor{#3}{center}}%
 \pgf@xa=\pgf@x%
 \pgf@ya=\pgf@y% 
 \pgfmathparse{#2}
 \edef\tkz@coeff{\pgfmathresult}%
 \pgfinterruptboundingbox
 \path[coordinate](#1)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)%
      coordinate(tkzPointResult);
        \endpgfinterruptboundingbox
\endgroup
}
%<--------------------------------------------------------------------------–>
%                 rotation  en degré
%<--------------------------------------------------------------------------–>
\def\tkzRotateAngle(#1,#2)(#3)#4{%
\begingroup
\gdef\tkz@LastList{#4}
\foreach\PointRot in {#3}{%
  \FirstPointInList\tkz@LastList
  \ifx\tkz@FirstPoint\tkzutil@empty  
     \def\tkz@pointtsf{\PointRot '}
  \else
     \def\tkz@pointtsf{\tkz@FirstPoint}
  \fi 
    \tkz@@extractxy{\PointRot}
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \tkz@@extractxy{#1}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \tkzmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {#2}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \pgfinterruptboundingbox
    \path[coordinate](\tkz@bx,\tkz@by)coordinate(\tkz@pointtsf);% 
    \endpgfinterruptboundingbox
}   
  \endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzURotateAngle(#1,#2)(#3){%
\begingroup 
  \pgf@process{\pgfpointanchor{#3}{center}}%
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \pgf@process{\pgfpointanchor{#1}{center}}%
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \tkzmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {#2}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \pgfinterruptboundingbox
      \path (\tkz@bx,\tkz@by) coordinate (tkzPointResult);% 
    \endpgfinterruptboundingbox     
\endgroup
}   
%<--------------------------------------------------------------------------–>
% %                 rotation  en radian
% %<--------------------------------------------------------------------------–>
\def\tkzRotateInRad(#1,#2)(#3)#4{%
\begingroup
\gdef\tkz@LastList{#4}
    \foreach\PointRot in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointRot '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
   \pgfmathparse{#2 r}
   \let\tkz@Angle\pgfmathresult
    \tkz@@extractxy{\PointRot}
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \tkz@@extractxy{#1}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \tkzmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {\tkz@Angle}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
      \pgfinterruptboundingbox
    \path[coordinate](\tkz@bx,\tkz@by)coordinate(\tkz@pointtsf); 
      \endpgfinterruptboundingbox 
}  
\endgroup 
}
%<--------------------------------------------------------------------------–>
\def\tkzURotateInRad(#1,#2)(#3){%
\begingroup
   \pgfmathparse{#2 r}
   \let\tkz@Angle\pgfmathresult
    \tkz@@extractxy{#3}
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \tkz@@extractxy{#1}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \tkzmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {\tkz@Angle}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
      \pgfinterruptboundingbox
    \path[coordinate](\tkz@bx,\tkz@by)coordinate(tkzPointResult); 
      \endpgfinterruptboundingbox 
\endgroup 
}
%<--------------------------------------------------------------------------–>
%                   Inverse of a point 
%<--------------------------------------------------------------------------–>
\def\tkzInversePoint(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointIP in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointIP '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
    \tkz@@CalcLengthcm(#1,#2){tkz@lna}
    \tkz@@CalcLengthcm(#1,\PointIP){tkz@lnb}
    \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
    \tkzVecKNorm[\tkz@lnc](#1,\PointIP) 
    \pgfnodealias{\tkz@pointtsf}{tkzPointResult}
    }  
\endgroup
} 
\def\tkzUInversePoint(#1,#2)(#3){%  
\begingroup  
   \tkz@@CalcLengthcm(#1,#2){tkz@lna}% 
   \tkz@@CalcLengthcm(#1,#3){tkz@lnb}% 
   \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
   \tkzVecKNorm[\tkz@lnc](#1,#3) 
\endgroup
} 
% possible 
% \tkzDefLine[tangent from =#3](#1,#2) 
% \tkzTgtFromP(#1,#2)(#3) 
% \tkzInterLL(tkzFirstPointResult,tkzSecondPointResult)(#1,#2) 
%<--------------------------------------------------------------------------–>
%                   Inverse negative of a point 
%<--------------------------------------------------------------------------–>
\def\tkzInverseNegativePoint(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointIP in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointIP '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
   \tkz@@CalcLengthcm(#1,#2){tkz@lna}
   \tkz@@CalcLengthcm(#1,\PointIP){tkz@lnb}
   \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
   \tkzVecKNorm[\tkz@lnc](#1,\PointIP) 
   \tkzUCSym(#1)(tkzPointResult)
   \pgfnodealias{\tkz@pointtsf}{tkzPointResult}
   }  
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzUInverseNegativePoint(#1,#2)(#3){%  
\begingroup  
   \tkz@@CalcLengthcm(#1,#2){tkz@lna}% 
   \tkz@@CalcLengthcm(#1,#3){tkz@lnb}% 
   \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
   \tkzVecKNorm[\tkz@lnc](#1,#3) 
   \tkzUCSym(#1)(tkzPointResult)
\endgroup
}
%<--------------------------------------------------------------------------–>
%<--------------- rotate with nodes                 ------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzRotateWithNodes(#1,#2,#3)(#4)#5{%
\begingroup
\gdef\tkz@LastList{#5}
 \foreach\PointRotWN in {#4}{%
   \FirstPointInList\tkz@LastList
   \ifx\tkz@FirstPoint\tkzutil@empty  
      \def\tkz@pointtsf{\PointRotWN '}
   \else
      \def\tkz@pointtsf{\tkz@FirstPoint}
   \fi 
   \tkzFindAngle(#2,#1,#3)
   \tkz@@extractxy{\PointRotWN}
   \tkz@ax\pgf@x%
   \tkz@ay\pgf@y%
   \tkz@@extractxy{#1}
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \tkzmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                        {\pgfpoint{\tkz@bx}{\tkz@by}}%
                        {\tkzAngleResult}
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \pgfinterruptboundingbox
   \path[coordinate](\tkz@bx,\tkz@by) coordinate (\tkz@pointtsf);% 
   \endpgfinterruptboundingbox
}   
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzURotateWithNodes(#1,#2,#3)(#4){%
\begingroup 
  \tkzFindAngle(#2,#1,#3)
  \pgf@process{\pgfpointanchor{#4}{center}}%
  \tkz@ax\pgf@x%
  \tkz@ay\pgf@y%
  \pgf@process{\pgfpointanchor{#1}{center}}%
  \tkz@bx\pgf@x%
  \tkz@by\pgf@y%
  \tkzmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                           {\pgfpoint{\tkz@bx}{\tkz@by}}%
                           {\tkzAngleResult}
  \tkz@bx\pgf@x%
  \tkz@by\pgf@y%
  \pgfinterruptboundingbox
  \path (\tkz@bx,\tkz@by) coordinate (tkzPointResult);%
  \endpgfinterruptboundingbox  
\endgroup
}   
%<--------------------------------------------------------------------------–>
%                   Fin des transformations
%<--------------------------------------------------------------------------–>
\makeatother
\endinput

==> tikz-euclide/obj-lua/tkz-obj-lua-points-spc.tex <==
% tkz-obj-lua-points.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/01/23} 
\typeout{2023/01/23 5.02c tkz-obj-lua-points.tex} 
\makeatletter  
%add ExCenter
%<--------------------------------------------------------------------------–>
%                   Specific points
%<--------------------------------------------------------------------------–>
%                              barycentre
%<--------------------------------------------------------------------------–>
\def\tkzDefBarycentricPoint(#1){%
\begingroup
 \path[coordinate]  (barycentric cs:#1) coordinate (tkzPointResult); 
\endgroup
}
\let\tkzDefBCPoint\tkzDefBarycentricPoint

\def\tkzDefBarycentricPointTwo(#1,#2,#3,#4){%
\begingroup
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}
\tkz@ax\pgf@x %
\tkz@ay\pgf@y %
\edef\tkzcax{\strip@pt\tkz@ax}%
\edef\tkzcay{\strip@pt\tkz@ay}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#4}{center}}
\tkz@bx\pgf@x %
\tkz@by\pgf@y %
\edef\tkzcbx{\strip@pt\tkz@bx}%
\edef\tkzcby{\strip@pt\tkz@by}%
\edef\tkztpmx{\tkz@Dec{(\tkzcax*(#2) + \tkzcbx*(#4))/(#2 + #4 )}}
\edef\tkztpmy{\tkz@Dec{(\tkzcay*(#2) + \tkzcby*(#2))/(#2 + #4 )}}
\pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkztpmx pt}{\tkztpmy pt}}
\endgroup
}

%<--------------------------------------------------------------------------–>
%                      milieu  de deux points
%<--------------------------------------------------------------------------–>
% possible   \coordinate (#3) at ($(#1)!0.5!(#2)$);
%<--------------------------------------------------------------------------–>
% \def\tkzDefMidPoint(#1,#2){%
% \begingroup
%  \path (#1) -- (#2) coordinate[pos=.5](tkzPointResult);
% \endgroup
% }
\def\tkzDefMidPoint(#1,#2){%
\begingroup
   \pgf@process{\pgfpointanchor{#1}{center}}%
   \tkz@ax\pgf@x%
   \tkz@ay\pgf@y%
   \pgf@process{\pgfpointanchor{#2}{center}}%
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \advance\tkz@bx by\tkz@ax\relax%
   \advance\tkz@by by\tkz@ay\relax%
   \divide\tkz@bx by2\relax%
   \divide\tkz@by by2\relax
   \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkz@bx}{\tkz@by}}
\endgroup
}
\def\tkz@DefMidPoint(#1,#2,#3,#4){%
\begingroup
   \tkz@ax#1%
   \tkz@ay#2%
   \tkz@bx#3%
   \tkz@by#4%
   \advance\tkz@bx by\tkz@ax\relax%
   \advance\tkz@by by\tkz@ay\relax%
   \divide\tkz@bx by2\relax%
   \divide\tkz@by by2\relax
   \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkz@bx}{\tkz@by}}
\endgroup
}

%<--------------------------------------------------------------------------–>
\def\tkz@simicenter{0}
\pgfkeys{/tkzsimicenter/.cd,
      ext/.code       = \def\tkz@simicenter{0},
      int/.code       = \def\tkz@simicenter{1},
      ext
}%

\def\tkzDefSimilitudeCenter{\pgfutil@ifnextchar[{\tkz@DefSimilitudeCenter}%
                                                {\tkz@DefSimilitudeCenter[]}}     
\def\tkz@DefSimilitudeCenter[#1](#2,#3)(#4,#5){%
\pgfqkeys{/tkzsimicenter}{#1} 
\begingroup  
\ifcase\tkz@simicenter%
  \tkzDefExtSimilitudeCenter[#1](#2,#3)(#4,#5)
  \or% 1 
  \tkzDefIntSimilitudeCenter[#1](#2,#3)(#4,#5) 
\fi
\endgroup
}
%<--------------------------------------------------------------------------–>
%                    Internal Similitude center
%  Two circles have two similitude centers namely the internal center of
%   similitude Si and the external similitude center Se.
%<--------------------------------------------------------------------------–>
\def\tkz@numhomo{0}
\pgfkeys{
/tkzSimilitudeCenter/.cd,
 node/.code          = \def\tkz@numhomo{0},
 R/.code             = \def\tkz@numhomo{1},
 node,
 /tkzSimilitudeCenter/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
 \pgfkeysalso{\searchname/.try=#1, /tikz/\searchname/.retry=#1}}
}
\def\tkzDefIntSimilitudeCenter{\pgfutil@ifnextchar[{\tkz@DefIntSimilitudeCenter}{\tkz@DefIntSimilitudeCenter[]}}
\def\tkz@DefIntSimilitudeCenter[#1](#2,#3)(#4,#5){%
\begingroup
\pgfqkeys{/tkzSimilitudeCenter}{#1}
\ifcase\tkz@numhomo%
    \tkz@@CalcLengthcm(#2,#3){tkz@rt}%
    \tkz@@CalcLengthcm(#4,#5){tkz@rf}%
  \or% 1
   \def\tkz@rt{#3}%
   \def\tkz@rf{#5}%
\fi
\pgfinterruptboundingbox 
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}}
\tkz@ax\pgf@x %
\tkz@ay\pgf@y %
\edef\tkzcax{\strip@pt\tkz@ax}%
\edef\tkzcay{\strip@pt\tkz@ay}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#4}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#4}{center}}
\tkz@bx\pgf@x %
\tkz@by\pgf@y %
\edef\tkzcbx{\strip@pt\tkz@bx}%
\edef\tkzcby{\strip@pt\tkz@by}%
\edef\tkztpmx{\tkz@Dec{(\tkzcax*\tkz@rf + \tkzcbx*\tkz@rt)/(\tkz@rf + \tkz@rt )}}
\edef\tkztpmy{\tkz@Dec{(\tkzcay*\tkz@rf + \tkzcby*\tkz@rt)/(\tkz@rf + \tkz@rt )}}
  \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkztpmx pt}{\tkztpmy pt}}
\endpgfinterruptboundingbox 
\endgroup
}
\let\tkzDefIntHomotheticCenter\tkzDefIntSimilitudeCenter
%<--------------------------------------------------------------------------–>
%                    External Similitude center
%<--------------------------------------------------------------------------–>
\def\tkzDefExtSimilitudeCenter{\pgfutil@ifnextchar[{\tkz@DefExtSimilitudeCenter}{%
\tkz@DefExtSimilitudeCenter[]}}

\def\tkz@DefExtSimilitudeCenter[#1](#2,#3)(#4,#5){%
\begingroup
\pgfqkeys{/tkzSimilitudeCenter}{#1}
\ifcase\tkz@numhomo%
  \tkz@@CalcLengthcm(#2,#3){tkz@rt}%
  \tkz@@CalcLengthcm(#4,#5){tkz@rf}%
   \or% 1
  \def\tkz@rt{#3}%
  \def\tkz@rf{#5}%
\fi
\pgfinterruptboundingbox 
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}}
\tkz@ax\pgf@x %
\tkz@ay\pgf@y %
\edef\tkzcax{\strip@pt\tkz@ax}%
\edef\tkzcay{\strip@pt\tkz@ay}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#4}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#4}{center}}
\tkz@bx\pgf@x %
\tkz@by\pgf@y %
\edef\tkzcbx{\strip@pt\tkz@bx}%
\edef\tkzcby{\strip@pt\tkz@by}%
\edef\tkztpmx{\tkz@Dec{(\tkzcax*(-\tkz@rf) + \tkzcbx*\tkz@rt)/(\tkz@rt - (\tkz@rf))}}
\edef\tkztpmy{\tkz@Dec{(\tkzcay*(-\tkz@rf) + \tkzcby*\tkz@rt)/(\tkz@rt - (\tkz@rf))}}
  \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkztpmx pt}{\tkztpmy pt}}
   \endpgfinterruptboundingbox 
\endgroup
}

\let\tkzDefExtHomotheticCenter\tkzDefExtSimilitudeCenter
%<--------------------------------------------------------------------------–>
%        Harmonic Division
%<--------------------------------------------------------------------------–>
%  A , B , C ,D  CA/CB = DA/DB
%<--------------------------------------------------------------------------–>
\def\tkz@numdha{0}
\pgfkeys{/tkzharmonic/.cd,
      ext/.code       = \def\tkz@numdha{0},
      int/.code       = \def\tkz@numdha{1},
      both/.code      = \def\tkz@numdha{2},
      both,
}%

\def\tkzDivHarmonic{\pgfutil@ifnextchar[{\tkz@DivHarmonic}{\tkz@DivHarmonic[]}}     
\def\tkz@DivHarmonic[#1](#2){%
\begingroup 
\pgfqkeys{/tkzharmonic}{#1}  
  \ifcase\tkz@numdha%
   \tkzDefDivHarmonicExt(#2)
 \or%
    \tkzDefDivHarmonicInt(#2)
  \or%
    \tkzDefDivHarmonicBoth(#2)
 \fi
\endgroup
}

\def\tkzDefDivHarmonicExt(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
  \tkz@VecKOrth[](#1,#2)  \tkzGetPoint{tkz@px}
  \tkzDefMidPoint(tkz@px,#2)          \tkzGetPoint{tkz@py}
  \tkzInterLL(tkz@px,#3)(#1,tkz@py)   \tkzGetPoint{tkz@pz}
  \tkzInterLL(#2,tkz@pz)(#1,tkz@px)   \tkzGetPoint{tkz@px}
  \tkzInterLL(tkz@py,tkz@px)(#1,#2)   \tkzGetPoint{tkzPointResult}
\endpgfinterruptboundingbox 
\endgroup
}

\def\tkzDefDivHarmonicInt(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
  \tkz@VecKOrth[1](#1,#2)  \tkzGetPoint{tkz@px}
  \tkzDefMidPoint(tkz@px,#2)          \tkzGetPoint{tkz@py}
  \tkzInterLL(tkz@py,#3)(#1,tkz@px)   \tkzGetPoint{tkz@pz}
  \tkzInterLL(#2,tkz@pz)(#1,tkz@py)   \tkzGetPoint{tkz@py}
  \tkzInterLL(tkz@py,tkz@px)(#1,#2)   \tkzGetPoint{tkzPointResult}
\endpgfinterruptboundingbox 
\endgroup
}

\def\tkzDefDivHarmonicBoth(#1,#2,#3){%
\begingroup
\edef\tkz@k{\fpeval{#3}}
    \path[coordinate]  (barycentric cs:#1=1,#2={\tkz@k}) coordinate (tkzFirstPointResult);
    \path[coordinate]  (barycentric cs:#1=1,#2={-\tkz@k}) coordinate (tkzSecondPointResult);
\endgroup
}

\let\tkzDefHarmonic\tkzDivHarmonic
%<--------------------------------------------------------------------------–> 
%                   golden ratio
%<--------------------------------------------------------------------------–>
\def\tkzDefGoldenRatio(#1,#2){%
\begingroup
\tkzDefPointWith[linear,K=\tkzInvPhi](#1,#2)
\endgroup
}
%<--------------------------------------------------------------------------–> 
%                    triangle center
%<--------------------------------------------------------------------------–>

\def\tkz@numtc{0}
\pgfkeys{/tkzDefTriangleCenter/.cd,
   ortho/.code        = \def\tkz@numtc{0},
   orthic/.code       = \def\tkz@numtc{0},
   centroid/.code     = \def\tkz@numtc{1},
   median/.code       = \def\tkz@numtc{1},
   circum/.code       = \def\tkz@numtc{2},
   in/.code           = \def\tkz@numtc{3},
   ex/.code           = \def\tkz@numtc{4},
   euler/.code        = \def\tkz@numtc{5},
   symmedian/.code    = \def\tkz@numtc{6},
   lemoine/.code      = \def\tkz@numtc{6},
   grebe/.code        = \def\tkz@numtc{6},
   spieker/.code      = \def\tkz@numtc{7},
   gergonne/.code     = \def\tkz@numtc{8},
   nagel/.code        = \def\tkz@numtc{9}, 
   mittenpunkt/.code  = \def\tkz@numtc{10}, 
   feuerbach/.code    = \def\tkz@numtc{11},
   circum       
}     
\def\tkzDefTriangleCenter{\pgfutil@ifnextchar[{\tkz@DefTriangleCenter}{\tkz@DefTriangleCenter[]}}
\def\tkz@DefTriangleCenter[#1](#2){% 
\begingroup  
\pgfqkeys{/tkzDefTriangleCenter}{#1}  
\ifcase\tkz@numtc%
  \tkzOrthoCenter(#2)
  \or% 1 
  \tkzCentroid(#2)  
  \or% 2
  \tkzCircumCenter(#2) 
  \or% 3
  \tkzInCenter(#2) 
  \or% 4
  \tkzExCenter(#2) 
  \or% 5
  \tkzEulerCenter(#2)
  \or% 6
  \tkzSymmedianCenter(#2) 
  \or% 7
  \tkzSpiekerCenter(#2) 
  \or% 8
  \tkzGergonneCenter(#2) 
  \or%9
  \tkzNagelCenter(#2)
  \or%10
  \tkzMittenpunktCenter(#2) 
  \or%11
  \tkzFeuerbachCenter(#2) 
    \fi    
\endgroup
}
%<--------------------------------------------------------------------------–> 
%                    OrthoCenter
%<--------------------------------------------------------------------------–>
\def\tkzOrthoCenter(#1,#2,#3){%
\begingroup
  \pgfinterruptboundingbox 
   \tkzUProjection(#1,#2)(#3)
   \pgfnodealias{ort@pta}{tkzPointResult}
   \tkzUProjection(#1,#3)(#2)
   \pgfnodealias{ort@ptb}{tkzPointResult}
   \tkzInterLL(#2,ort@ptb)(#3,ort@pta)
   \endpgfinterruptboundingbox 
\endgroup
}
\let\tkzDefOrthoCenter\tkzOrthoCenter
%<--------------------------------------------------------------------------–>
%                      GravityCenter modif 3.03
%<--------------------------------------------------------------------------–>
\def\tkzCentroid(#1,#2,#3){%
\begingroup 
   \pgf@process{\pgfpointanchor{#1}{center}}%
   \tkz@ax\pgf@x%
   \tkz@ay\pgf@y%
   \pgf@process{\pgfpointanchor{#2}{center}}%
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \pgf@process{\pgfpointanchor{#3}{center}}%
   \tkz@cx\pgf@x%
   \tkz@cy\pgf@y%
   \edef\tkzcax{\strip@pt\tkz@ax}%
   \edef\tkzcay{\strip@pt\tkz@ay}%
   \edef\tkzcbx{\strip@pt\tkz@bx}%
   \edef\tkzcby{\strip@pt\tkz@by}%
   \edef\tkzccx{\strip@pt\tkz@cx}%
   \edef\tkzccy{\strip@pt\tkz@cy}%
   \edef\tkztpmx{\tkz@Dec{(\tkzcax + \tkzcbx + \tkzccx)/3}}
   \edef\tkztpmy{\tkz@Dec{(\tkzcay + \tkzcby + \tkzccy)/3}}
   \pgfinterruptboundingbox 
   \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkztpmx pt}{\tkztpmy pt}}
   \endpgfinterruptboundingbox   
\endgroup
}
\let\tkzBaryCenter\tkzCentroid

%<--------------------------------------------------------------------------–>
%                      CircumCenter
%<--------------------------------------------------------------------------–>
\def\tkzCircumCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
 \tkzDefMediatorLine(#1,#2)
 \pgf@process{\pgfpointanchor{tkzFirstPointResult}{center}}%
 \tkz@ax\pgf@x%
 \tkz@ay\pgf@y%
 \pgf@process{\pgfpointanchor{tkzSecondPointResult}{center}}%
 \tkz@bx\pgf@x%
 \tkz@by\pgf@y%
 \tkzDefMediatorLine(#1,#3)
 \pgf@process{\pgfpointanchor{tkzFirstPointResult}{center}}%
 \tkz@cx\pgf@x%
 \tkz@cy\pgf@y%
 \pgf@process{\pgfpointanchor{tkzSecondPointResult}{center}}%
 \tkz@dx\pgf@x%
 \tkz@dy\pgf@y%
\tkzInterLLxy(\tkz@ax,\tkz@ay,\tkz@bx,\tkz@by)(\tkz@cx,\tkz@cy,\tkz@dx,\tkz@dy)%
\endpgfinterruptboundingbox
\endgroup
} 
\let\tkzDefCircumCenter\tkzCircumCenter
%<--------------------------------------------------------------------------–>
%                     InCenter
%<--------------------------------------------------------------------------–>
\def\tkzInCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
\tkzDefBisectorLine(#3,#1,#2)
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\tkzDefBisectorLine(#3,#2,#1) 
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@dx\pgf@x%
\tkz@dy\pgf@y%
\pgf@process{\pgfpointanchor{#1}{center}}%
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgf@process{\pgfpointanchor{#2}{center}}%
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\tkzInterLLxy(\tkz@ax,\tkz@ay,\tkz@bx,\tkz@by)(\tkz@cx,\tkz@cy,\tkz@dx,\tkz@dy)%
\endpgfinterruptboundingbox
\endgroup
} 
\let\tkzDefInCenter\tkzInCenter
%<--------------------------------------------------------------------------–>
%                     ExCenter
%<--------------------------------------------------------------------------–>
\def\tkzExCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
\tkzDefBisectorOutLine(#2,#1,#3)
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\tkzDefBisectorOutLine(#2,#3,#1) 
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@dx\pgf@x%
\tkz@dy\pgf@y%
\pgf@process{\pgfpointanchor{#1}{center}}%
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgf@process{\pgfpointanchor{#3}{center}}%
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\tkzInterLLxy(\tkz@ax,\tkz@ay,\tkz@bx,\tkz@by)(\tkz@cx,\tkz@cy,\tkz@dx,\tkz@dy)%
\endpgfinterruptboundingbox
\endgroup
} 
\let\tkzDefExCenter\tkzExCenter
%<--------------------------------------------------------------------------–>
%                     EulerCenter neuf points
%<--------------------------------------------------------------------------–>
\def\tkzEulerCenter(#1,#2,#3){% 
% mileu de orthocentre et centre cercle circonscrit
% passe par les midpoints par les pieds des hauteurs
\begingroup
\pgfinterruptboundingbox 
\tkzDefMidPoint(#1,#2)
\pgfnodealias{eu@mic}{tkzPointResult}
\tkzDefMidPoint(#1,#3)
\pgfnodealias{eu@mib}{tkzPointResult}
\tkzDefMidPoint(#2,#3)
\pgfnodealias{eu@mia}{tkzPointResult}
\tkzCircumCenter(eu@mia,eu@mib,eu@mic)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzNinePointCenter\tkzEulerCenter
\let\tkzDefEulerCenter\tkzEulerCenter
%<--------------------------------------------------------------------------–>
%Symmedian center Lemoine point Grebe point K
%<--------------------------------------------------------------------------–>
\def\tkzSymmedianCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox    
\tkzDefMidPoint(#2,#3)
\pgfnodealias{eu@mic}{tkzPointResult}
\tkzDefMidPoint(#1,#3)
\pgfnodealias{eu@mib}{tkzPointResult}
\tkzUProjection(#2,#3)(#1)
\pgfnodealias{ort@pta}{tkzPointResult}
\tkzDefMidPoint(#1,ort@pta)
\pgfnodealias{eu@mid}{tkzPointResult}
\tkzUProjection(#1,#3)(#2)
\pgfnodealias{ort@ptb}{tkzPointResult}
\tkzDefMidPoint(#2,ort@ptb)
\pgfnodealias{eu@mie}{tkzPointResult}
\tkzInterLL(eu@mic,eu@mid)(eu@mib,eu@mie)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzLemoinePoint\tkzSymmedianCenter
\let\tkzGrebePoint\tkzSymmedianCenter
\let\tkzDefLemoinePoint\tkzLemoinePoint
%<--------------------------------------------------------------------------–> 
%                   Spieker center
%<--------------------------------------------------------------------------–>
\def\tkzSpiekerCenter(#1,#2,#3){%
\begingroup
% we need to get the midpoints
\pgfcoordinate{tkz@m3}{%
  \pgfpointscale{0.5}{%
  \pgfpointadd{\pgfpointanchor{#1}{center}}%
              {\pgfpointanchor{#2}{center}}}}%
\pgfcoordinate{tkz@m2}{%
  \pgfpointscale{0.5}{%
  \pgfpointadd{\pgfpointanchor{#1}{center}}%
              {\pgfpointanchor{#3}{center}}}}%
\pgfcoordinate{tkz@m1}{%
   \pgfpointscale{0.5}{%
   \pgfpointadd{\pgfpointanchor{#2}{center}}%
               {\pgfpointanchor{#3}{center}}}}%
\tkzInCenter(tkz@m1,tkz@m2,tkz@m3)
\endgroup
} 
\let\tkzDefSpiekerCenter\tkzSpiekerCenter 
%<--------------------------------------------------------------------------–> 
%                    Gergonne center Ge
%<--------------------------------------------------------------------------–>
\def\tkzGergonneCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzInCenter(#1,#2,#3)
\pgfnodealias{tkz@ptin}{tkzPointResult}
\tkzUProjection(#2,#3)(tkz@ptin)
\pgfnodealias{tkz@oca}{tkzPointResult}
\tkzUProjection(#1,#3)(tkz@ptin)
\pgfnodealias{tkz@ocb}{tkzPointResult}
\tkzInterLL(#1,tkz@oca)(#2,tkz@ocb)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzDefGergonneCenter\tkzGergonneCenter 
%<--------------------------------------------------------------------------–> 
%                    Nagel center Na
%<--------------------------------------------------------------------------–>
%  INa = 3 IG. Nagel point % correction 02/02/20
\def\tkzNagelCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzDefExcentralTriangle(#1,#2,#3){tkz@a,tkz@b,tkz@c}
\tkzUProjection(#2,#3)(tkz@a)
\pgfnodealias{tkz@tgta}{tkzPointResult}
\tkzUProjection(#1,#2)(tkz@c)
\pgfnodealias{tkz@tgtc}{tkzPointResult}
\tkzInterLL(#1,tkz@tgta)(#3,tkz@tgtc)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzDefNagelCenter\tkzNagelCenter 
%<--------------------------------------------------------------------------–>
%  Mittenpunkt
%<--------------------------------------------------------------------------–>
\def\tkzMittenpunktCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzExCenter(#2,#3,#1)
\pgfnodealias{tkz@a}{tkzPointResult}
\tkzExCenter(#3,#1,#2)
\pgfnodealias{tkz@b}{tkzPointResult}
\pgfcoordinate{tkz@ma}{%
\pgfpointscale{0.5}{%
\pgfpointadd{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}}}%
\pgfcoordinate{tkz@mb}{%
\pgfpointscale{0.5}{%
\pgfpointadd{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}}}%
\tkzInterLL(tkz@a,tkz@ma)(tkz@b,tkz@mb)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzDefMittenpunktCenter\tkzMittenpunktCenter 
\let\tkzDefMiddlespoint\tkzMittenpunktCenter     
%<--------------------------------------------------------------------------–> 
%                   Feuerbach point
%<--------------------------------------------------------------------------–>
\def\tkzFeuerbachCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzEulerCenter(#1,#2,#3)
\pgfnodealias{tkz@euler}{tkzPointResult}
\tkzInCenter(#1,#2,#3) 
\pgfnodealias{tkz@in}{tkzPointResult}
\tkzUProjection(#2,#3)(tkzPointResult)
\tkzInterLC(tkz@in,tkz@euler)(tkz@in,tkzPointResult)\tkzGetFirstPoint{tkz@fe}
\tkzRenamePoint(tkz@fe){tkzPointResult}
\endpgfinterruptboundingbox  
\endgroup
}
\let\tkzDefFeuerbachCenter\tkzFeuerbachCenter 
%<--------------------------------------------------------------------------–>
%                     Orthogonal center
%<--------------------------------------------------------------------------–>
\def\tkzOrthogonalCenter(#1,#2){%
\begingroup
\pgfinterruptboundingbox 
\tkz@VecK[\tkz@koeff/(1+\tkz@koeff)](#1,#2)
\pgfnodealias{tkzFirstPointResult}{tkzPointResult}
\tkz@VecK[\tkz@koeff/(\tkz@koeff-1)](#1,#2)
\pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\tkzDefMidPoint(tkzFirstPointResult,tkzSecondPointResult) 
\endpgfinterruptboundingbox 
\endgroup
}
%<--------------------------------------------------------------------------–>
%                  End Triangle center
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                  Projection  center of excircles
%<--------------------------------------------------------------------------–>
\def\tkzDefProjExcenter{\pgfutil@ifnextchar[{%
    \tkz@DefProjExcenter}{%
    \tkz@DefProjExcenter[]}
    }
\def\tkz@DefProjExcenter[#1](#2,#3,#4)(#5)#6{
\begingroup  
  \SetUpPTTR{#1}
   \foreach \name  [count=\i] in {#5} {%
      \global\expandafter\edef\csname tkz@pt\i\endcsname{\name}
        }
   \foreach \name  [count=\i] in {#6} {%
      \global\expandafter\edef\csname tkz@ppt\i\endcsname{\name}
        }
\tkzDefPointBy[projection=onto #3--#4 ](\tkz@pttr@name \csname tkz@pt1\endcsname) 
\pgfnodealias{\csname tkz@ppt1\endcsname\csname tkz@pt1\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#4 ](\tkz@pttr@name \csname tkz@pt2\endcsname) 
\pgfnodealias{\csname tkz@ppt1\endcsname\csname tkz@pt2\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#4 ](\tkz@pttr@name \csname tkz@pt3\endcsname) 
\pgfnodealias{\csname tkz@ppt1\endcsname\csname tkz@pt3\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #2--#4 ](\tkz@pttr@name \csname tkz@pt1\endcsname) 
\pgfnodealias{\csname tkz@ppt2\endcsname\csname tkz@pt1\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #2--#4 ](\tkz@pttr@name \csname tkz@pt2\endcsname) 
\pgfnodealias{\csname tkz@ppt2\endcsname\csname tkz@pt2\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #2--#4 ](\tkz@pttr@name \csname tkz@pt3\endcsname) 
\pgfnodealias{\csname tkz@ppt2\endcsname\csname tkz@pt3\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#2 ](\tkz@pttr@name \csname tkz@pt1\endcsname) 
\pgfnodealias{\csname tkz@ppt3\endcsname\csname tkz@pt1\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#2 ](\tkz@pttr@name \csname tkz@pt2\endcsname) 
\pgfnodealias{\csname tkz@ppt3\endcsname\csname tkz@pt2\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#2 ](\tkz@pttr@name \csname tkz@pt3\endcsname) 
\pgfnodealias{\csname tkz@ppt3\endcsname\csname tkz@pt3\endcsname}{tkzPointResult}
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%              Point on circle
%<--------------------------------------------------------------------------–>
\def\tkz@numptcirc{0}
\pgfkeys{/tkzptcircle/.cd,
through/.code  args = {center #1 angle #2 point #3}        { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@through{#3}%
                                                             \def\tkz@numptcirc{0}},
R/.code args = {center #1 angle #2 radius #3}              { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@radius{#3}%
                                                             \def\tkz@numptcirc{1}},
through in rad/.code  args = {center #1 angle #2 point #3} { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@through{#3}%
                                                             \def\tkz@numptcirc{2}},
R in rad/.code args = {center #1 angle #2 radius #3}       { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@radius{#3}%
                                                             \def\tkz@numptcirc{3}}                                                 
}
                                                  
\def\tkzDefPointOnCircle{\pgfutil@ifnextchar[{\tkz@DefPointOnCircle}{%
                                              \tkz@DefPointOnCircle[]}}     
\def\tkz@DefPointOnCircle[#1]{%
\begingroup 
\pgfqkeys{/tkzptcircle}{#1}
 \ifcase\tkz@numptcirc%
    \tkz@@CalcLengthcm(\tkz@center,\tkz@through){tkz@radius}
     \or% 1
    \relax%
    \or% 2
    \pgfmathparse{\tkz@angle\space r}
    \let\tkz@angle\pgfmathresult
    \tkz@@CalcLengthcm(\tkz@center,\tkz@through){tkz@radius}
    \or% 3
    \pgfmathparse{\tkz@angle\space r}
    \let\tkz@angle\pgfmathresult
\fi
\path (\tkz@center) --++(\tkz@angle:\tkz@radius) coordinate(tkzPointResult);
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Point on line
%<--------------------------------------------------------------------------–>
\def\tkzDefPointOnLine{\pgfutil@ifnextchar[{\tkz@DefPointOnLine}{\tkz@DefPointOnLine[]}}     
\def\tkz@DefPointOnLine[#1](#2,#3){%
\begingroup 
\path (#2) to [#1] coordinate (tkzPointResult)  (#3);
\endgroup
} 

\makeatother  
\endinput

==> tikz-euclide/obj-lua/tkz-obj-lua-points-with.tex <==
% tkz-obj-lua-points-with.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-lua-points-with.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%                          Vectors
%<--------------------------------------------------------------------------–>
% Objet :  outils mathématiques pour la géométrie euclideienne avec pgf/tikz
% utilisable de préférence avec un repère orthonormé et le cm comme unité 
% utile pour la compatibilité avec pgf 2
%<--------------------------------------------------------------------------–>
%             Duplicate Length      à revoir pas de pt pas de global
% ||v(CN)||= ||v(AB)|| et v(CN) colineaire à v(CD) 
% A-->#1 B-->#2 C-->#3 D-->#4 N-->#5   ?????
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                 Outils pour les vecteurs
%<--------------------------------------------------------------------------–>
%  ce sont des outils élémentaires qui à partir de deux points en définissent 
% un troisième 
% #1 si c'est une option alors c'est un nombre réel
% #2 et #3 sont deux points
% #4 est le nom du point qui résulte de la transformation
% exemple : \tkzVecKNorm (A,B){C} définit un point C tel que AC = 1 et C est %  %  un point de la droite (AC). #1 peut être négatif

\def\tkzDuplicateSegment(#1,#2)(#3,#4){%
\begingroup 
    \tkz@@CalcLength(#1,#2){tkz@firstlen}% 
    \tkz@@CalcLength(#3,#4){tkz@secondlen}%
   \edef\tkz@ratio{\tkz@Dec{\tkz@firstlen/\tkz@secondlen}}
    \tkz@VecKCoLinear[\tkz@ratio](#3,#4,#3)%
\endgroup 
}
\let\tkzDuplicateLength\tkzDuplicateSegment     
%<--------------------------------------------------------------------------–>
%                    Coordonnées d'un vecteur  (couple de points)  
% Deux points A et B donc un vecteur on récupère les coordonnées de v(AB)
% en cm 
% tkzGetVecCoord en cm ou en pt ???
%<--------------------------------------------------------------------------–>
%result in #3x et #3y #1 et #2 sont les points  
% passage en cm avec fp ? 
% 28.45274 =1 cm
\def\tkzGetVectxy(#1,#2)#3{%
\begingroup 
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\pgfmathparse{\pgf@sys@tonumber{\pgf@x}/1cm}%
\let\tkzresultx\pgfmathresult
\pgfmathparse{\pgf@sys@tonumber{\pgf@y}/1cm}%
\let\tkzresulty\pgfmathresult
\global\expandafter\edef\csname #3x\endcsname{\tkzresultx}% 
\global\expandafter\edef\csname #3y\endcsname{\tkzresulty}% 
\endgroup
}
%<--------------------------------------------------------------------------–>
% options #1 two points #2,#3 result in #4
%
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%          tkzDefPointWith  
%<--------------------------------------------------------------------------–>
\def\tkz@numv{0}
\pgfkeys{/@pointwith/.cd,
      colinear/.code     args     = {at #1}{\def\tkz@numv{0}\def\tkz@frompoint{#1}},
      orthogonal/.code            = {\def\tkz@numv{1}},
      linear/.code                = {\def\tkz@numv{2}},
      orthogonal normed/.code     = {\def\tkz@numv{3}},
      linear normed/.code         = {\def\tkz@numv{4}},
      colinear normed/.code  args = {at #1}{\def\tkz@numv{5}\def\tkz@frompoint{#1}},
      K/.code                     = {\edef\tkz@coeff{\fpeval{#1}}},
      K                           = 1,
      normed/.is if               =  tkz@line@normed,
      normed/.default             =  true,
      normed                      =  false,
      orthogonal  
} 
\def\tkzDefPointWith{\pgfutil@ifnextchar[{\tkz@DefPointWith}{\tkz@DefPointWith[]}}  

\def\tkz@DefPointWith[#1](#2,#3){%
\begingroup 
\pgfkeys{/@pointwith/.cd,K=1}  
\pgfqkeys{/@pointwith}{#1}
\ifcase\tkz@numv%
 % first case 0
   \tkz@DefVectorColinearat[\tkz@coeff](#2,#3)
  \or% 1
   \tkz@VecKOrth[\tkz@coeff](#2,#3)
  \or% 2
   \tkz@VecK[\tkz@coeff](#2,#3)
  \or% 3
   \tkz@VecKOrthNorm[\tkz@coeff](#2,#3)
  \or% 4
   \tkz@VecKNorm[\tkz@coeff](#2,#3)
  \or% 5
   \tkz@VecKColinearNorm[\tkz@coeff](#2,#3)
  \fi    
\endgroup
} 
%<--------------------------------------------------------------------------–>
%         tkzDefVectorfrom  
%<--------------------------------------------------------------------------–>
% tkz@numv 0
\def\tkz@DefVectorColinearat[#1](#2,#3){%
\iftkz@line@normed
   \tkz@VecKColinearNorm[#1](#2,#3)
\else
\begingroup
  \pgfpointdiff{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}%
  \pgf@xa=\pgf@x\relax%
  \pgf@ya=\pgf@y\relax%
  \pgfinterruptboundingbox
  \path (\tkz@frompoint)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya) coordinate (tkzPointResult);
  \endpgfinterruptboundingbox
\endgroup
\fi
} 
%<--------------------------------------------------------------------------–>
%     tkzVector K Orth   coeff dans #1
%     v(AN) perp v(AB)  (v(AB) , v(AN) ) sens direct cercle trigo 
%     ||v(AN)||=||v(AB)||
%<--------------------------------------------------------------------------–>
% tkz@numv 1
\def\tkzVecKOrth{\pgfutil@ifnextchar[{\tkz@VecKOrth}{\tkz@VecKOrth[1]}}  
\def\tkz@VecKOrth[#1](#2,#3){%
\iftkz@line@normed
   \tkz@VecKOrthNorm[#1](#2,#3)
\else
\begingroup
  \pgfpointdiff{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}%
  \pgf@xa=-\pgf@y%
  \pgf@ya=\pgf@x%
  \pgfinterruptboundingbox 
  \path (#2)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya) coordinate (tkzPointResult);
  \endpgfinterruptboundingbox
\endgroup
\fi
}%

%<--------------------------------------------------------------------------–>
%         v(AN)=#1 x v(AB)     
%   #1 le coeff; #2--> A #3--> B   #4-->N  tq    #4-#2 = #1*(#3-#2)                                 
%<--------------------------------------------------------------------------–>
% tkz@numv 2
\def\tkzVecK{\pgfutil@ifnextchar[{\tkz@VecK}{\tkz@VecK[1]}} 
\def\tkz@VecK[#1](#2,#3){% 
\iftkz@line@normed
   \tkz@VecKNorm[#1](#2,#3)
\else
\begingroup 
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x\relax%
   \pgf@ya=\pgf@y\relax%
   \pgfmathparse{#1}
   \let\tkz@coeff\pgfmathresult
      \pgfinterruptboundingbox 
   \path (#2)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya) coordinate (tkzPointResult);
    \endpgfinterruptboundingbox   
\endgroup
\fi
}% 
%<--------------------------------------------------------------------------–>
%              tkzVecKOrthNorm   coeff dans #1
%    v(AN) perp v(AB)  v(AB) v(AN) sens direct cercle trigo 
% ||v(AN||=1 si #1 est vide ou =1 sinon ||v(AN||=K
%<--------------------------------------------------------------------------–>
% tkz@numv 3
\def\tkzVecKOrthNorm{\pgfutil@ifnextchar[{\tkz@VecKOrthNorm}%
                                         {\tkz@VecKOrthNorm[1]}}
\def\tkz@VecKOrthNorm[#1](#2,#3){%    
\begingroup
 \tkzpointnormalised{\pgfpointdiff{\pgfpointanchor{#2}{center}}%
                                  {\pgfpointanchor{#3}{center}}} 
  \pgf@xa=-\pgf@y\relax%
  \pgf@ya=\pgf@x\relax%
  \pgfmathparse{#1}
  \let\tkz@tmp\pgfmathresult
  \edef\tkz@x{\tkz@Dec{28.45274*\tkz@tmp*\strip@pt\pgf@xa}}
  \edef\tkz@y{\tkz@Dec{28.45274*\tkz@tmp*\strip@pt\pgf@ya}}
  \pgfinterruptboundingbox 
  \path (#2)--++(\tkz@x pt,\tkz@y pt) coordinate (tkzPointResult);
  \endpgfinterruptboundingbox   
\endgroup
}%      
%<--------------------------------------------------------------------------–>
%              VectorNormalised ou K*VectorNormalised
% A-->#2 B-->#3 N-->#4      v(AB)  devient v(AN) tq ||v(AN)||=1 si #1=1  
%  sinon ||v(AN)||=#1 
%<--------------------------------------------------------------------------–>
% tkz@numv 4
\def\tkzVecKNorm{\pgfutil@ifnextchar[{\tkz@VecKNorm}{\tkz@VecKNorm[1]}} 
\def\tkz@VecKNorm[#1](#2,#3){%
\begingroup
    \tkzpointnormalised{%
    \pgfpointdiff{\pgfpointanchor{#2}{center}}
                 {\pgfpointanchor{#3}{center}}}
    \pgf@xa=\pgf@x\relax%
    \pgf@ya=\pgf@y\relax% 
   \pgfmathparse{#1}
   \let\tkz@tmp\pgfmathresult
  \edef\tkz@x{\tkz@Dec{28.45274*\tkz@tmp*\strip@pt\pgf@xa}}
  \edef\tkz@y{\tkz@Dec{28.45274*\tkz@tmp*\strip@pt\pgf@ya}}
    \pgfinterruptboundingbox 
    \path (#2)--++(\tkz@x pt,\tkz@y pt) coordinate (tkzPointResult);
    \endpgfinterruptboundingbox   
\endgroup
}%
%<--------------------------------------------------------------------------–>
%            \tkz@VecKColinearNorm
%<--------------------------------------------------------------------------–>
%% tkz@numv 5
\def\tkz@VecKColinearNorm[#1](#2,#3){%
\begingroup   
    \tkzpointnormalised{%
    \pgfpointdiff{\pgfpointanchor{#2}{center}}
                 {\pgfpointanchor{#3}{center}}}
    \pgf@xa=\pgf@x\relax%
    \pgf@ya=\pgf@y\relax% 
  \edef\tkz@x{\tkz@Dec{28.45274*(\tkz@coeff)*\strip@pt\pgf@xa}}
  \edef\tkz@y{\tkz@Dec{28.45274*(\tkz@coeff)*\strip@pt\pgf@ya}}
    \pgfinterruptboundingbox
    \path (\tkz@frompoint)--++(\tkz@x pt,\tkz@y pt) coordinate (tkzPointResult);
    \endpgfinterruptboundingbox
\endgroup
}%
%<--------------------------------------------------------------------------–>
%  VecKCoLinear  CN = K x AB  #1 pt #2 pt #3 pt #4 nb #5 pt result   
% il faut modifier cette macro : on supprime #3 pour la colinéarité
% Il suffit d'utiliser Replicate ou Duplicate     coeff dans #1
% v(CD)=#1 x v(AB) #1 le coeff; #2-->A #3-->B #4-->C 
%<--------------------------------------------------------------------------–>
\def\tkz@VecKCoLinear[#1](#2,#3,#4){% 
\begingroup
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x\relax%
   \pgf@ya=\pgf@y\relax% 
   \edef\tkz@coeff{\fpeval{#1}}
   \pgfinterruptboundingbox 
   \path (#4)--+(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)  coordinate (tkzPointResult);
   \endpgfinterruptboundingbox                     
\endgroup
}%  
\def\tkz@VecCoLinear(#1,#2,#3){% 
\begingroup
   \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                {\pgfpointanchor{#2}{center}}%
   \pgf@xa=\pgf@x\relax%
   \pgf@ya=\pgf@y\relax% 
   \pgfinterruptboundingbox 
   \path (#3)--+(\pgf@xa,\pgf@ya)  coordinate (tkzPointResult);
   \endpgfinterruptboundingbox                     
\endgroup
}% 
\makeatother
\endinput

==> tikz-euclide/obj-lua/tkz-obj-lua-points.tex <==
 % tkz-obj-lua-points.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c  tkz-obj-lua-points.tex} 
\makeatletter
%<--------------------------------------------------------------------------->
%                             init def point 
%<--------------------------------------------------------------------------->
%                            tkzDefPoint
%<--------------------------------------------------------------------------->
%                     macros complémentaires  pour def point
%<--------------------------------------------------------------------------->
\def\tkz@parsecoordinate#1{%
\tkz@getseparator#1,\@nil
\iftkz@polar 
   \tkz@getfrompolar#1\@nil
\else
   \tkz@getfromcart#1\@nil
\fi
}
\def\tkz@getseparator#1,#2\@nil{%
\ifx\tkzempty#2\tkzempty%
   \tkz@polartrue
\else
   \tkz@polarfalse
\fi
}      
\def\tkz@getfrompolar#1:#2\@nil{%
\edef\tkz@a{\fpeval{#1}}
\edef\tkz@r{\fpeval{#2}}
\xdef\tkz@polarrad{\tkz@r}
\xdef\tkz@polarangle{\tkz@a}
} 
\def\tkz@getfromcart#1,#2\@nil{%
\edef\tkz@x{\fpeval{#1}}
\edef\tkz@y{\fpeval{#2}}
\xdef\tkz@absc{\tkz@x}
\xdef\tkz@ord{\tkz@y}
}
%<--------------------------------------------------------------------------->
%           options pour point definition
%<--------------------------------------------------------------------------->
\pgfkeys{/tkzPt/.cd,  
         polar/.is if       = tkz@pt@polar,
         polar/.default     = true,
         polar              = false  
}
%<--------------------------------------------------------------------------->
%        tkz@ptStar  
%<--------------------------------------------------------------------------->
\def\tkz@ptStar[#1](#2,#3)#{%
\pgfkeys{/tkzPt/.cd, polar     = false} 
\pgfqkeys{/tkzPt}{#1}  
\iftkz@pt@polar%
  \edef\tkz@x{\fpeval{#3*cosd(#2)}}
  \edef\tkz@y{\fpeval{#3*sind(#2)}}
\else
  \edef\tkz@x{\fpeval{#2}}
  \edef\tkz@y{\fpeval{#3}}
\fi
\edef\tkzpt@xa{\tkz@Dec{(\tkz@x-(\tkz@init@xorigine))/\tkz@init@xstep}}
\edef\tkzpt@ya{\tkz@Dec{(\tkz@y-(\tkz@init@yorigine))/\tkz@init@ystep}}
\tkz@node
}
%<--------------------------------------------------------------------------->
% la macro defpoint les coordonnées cartésiennes ou polaires sont  traitées
% afin de pouvoir être adaptées avec les unités choisies
%<--------------------------------------------------------------------------->
\def\tkzDefPoint{\pgfutil@ifnextchar[{\tkz@DefPoint}{\tkz@DefPoint[]}}

\def\tkz@DefPoint[#1](#2)#{% 
\tkz@parsecoordinate{#2}
\iftkz@polar
   \tkz@ptStar[polar](\tkz@polarangle,\tkz@polarrad){tkz@coord@temp}
\else  
    \tkz@ptStar[](#2){tkz@coord@temp}
\fi
\tkz@DefPointEnd[#1]
}% 
\def\tkz@DefPointEnd[#1]#2{\coordinate[#1] (#2) at (tkz@coord@temp);}
%<--------------------------------------------------------------------------->
%                            tkzDefPoints
%<--------------------------------------------------------------------------->
\def\tkzDefPoints{\pgfutil@ifnextchar[{\tkz@DefPoints}{\tkz@DefPoints[]}}
\def\tkz@DefPoints[#1]#2{%
  \begingroup
  \def\tkz@parenthesis@for@err{(}%
  \def\tkz@maybe@parenthesis{#2}%
  \ifx\tkz@maybe@parenthesis\tkz@parenthesis@for@err
    \PackageError{tkz-base}{Syntax error  use {} instead of ()}{You need to use {} instead of ()}%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {\tkz@absorb@bad@arg}% 
  {\foreach \ptx/\pty/\name in {#2}{\tkzDefPoint[#1](\ptx,\pty){\name}}%
   \endgroup}%
}
\def\tkz@absorb@bad@arg#1){\endgroup}
%<--------------------------------------------------------------------------->
\def\tkz@node#1{ \pgfinterruptboundingbox
\path[coordinate](\tkzpt@xa,\tkzpt@ya) coordinate(#1);
 \endpgfinterruptboundingbox}  
%<--------------------------------------------------------------------------->
\def\tkzRenamePoint(#1)#2{\coordinate (#2) at (#1);}
\def\tkz@RenamePointEnd[#1]#2{\coordinate[#1] (#2) at (\tkz@ax,\tkz@ay);}
\def\tkzGetPoint#1{\coordinate  (#1) at (tkzPointResult);} 
\def\tkzGetPoints#1#2{\coordinate  (#1) at (tkzFirstPointResult);
                      \coordinate  (#2) at (tkzSecondPointResult);}
\def\tkzGetFirstPoint#1{\coordinate  (#1) at (tkzFirstPointResult);}
\def\tkzGetSecondPoint#1{\coordinate  (#1) at (tkzSecondPointResult);}
\def\tkzGetThirdPoint#1{\coordinate  (#1) at (tkzThirdPointResult);}
\def\tkzDefShiftPointCoord[#1](#2)#3{%
                \begin{scope}[shift={(#1)}]
                     \coordinate  (#3) at (#2);
                \end{scope}
                           }%
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
                            
%<--------------------------------------------------------------------------->
%            tkzDefShiftPoint
%<--------------------------------------------------------------------------->
\def\tkzDefShiftPoint[#1](#2)#3{%
   \tkz@@extractxy{#1}
   \tkz@ax\pgf@x %
   \tkz@ay\pgf@y %   
\begin{scope}[shift={(\tkz@ax,\tkz@ay)}]
   \coordinate  (#3) at (#2);
\end{scope}
}
%<--------------------------------------------------------------------------->
%                    Coordonnées d'un point 
%    result in #2x et #2y    #1 est le point et on récupère ses coordonnées
% usage soit A un point \tkzGetPointCoord(A){V} alors \Vx = xA et \Vy = yA
% en cm 
% tkzGetPointCoord avec [#1] cm ou bien pt ?? todo
%<--------------------------------------------------------------------------->
\def\tkzGetPointCoord(#1)#2{%
\begingroup
   \pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
   \pgfmathparse{\pgf@sys@tonumber{\pgf@x}/28.45274}
   \global\let\tkzresultx\pgfmathresult
   \global\expandafter\edef\csname #2x\endcsname{\tkzresultx}% 
   \pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}
   \pgfmathparse{\pgf@sys@tonumber{\pgf@y}/28.45274}
   \global\let\tkzresulty\pgfmathresult
   \global\expandafter\edef\csname #2y\endcsname{\tkzresulty}
\endgroup
}  
\def\tkz@@extractxy#1{%
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}} 
}
\let\tkzGetPointxy\tkzGetPointCoord
\makeatother  
\endinput

==> tikz-euclide/obj/tkz-obj-eu-axesmin.tex <==
% tkz-obj-eu-axesmin.tex    
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-axesmin}   

\makeatletter
\def\removedot#1.{#1}
\newcommand\tkzgetinteger[1]{\expandafter\tkz@getinteger#1.\@nil}
\def\tkz@getinteger#1.#2\@nil{%
  \ifx\empty#2\empty
    \tkz@integertrue
  \else
  \ifnum\removedot#2=0   
    \tkz@integertrue
   \else 
     \tkz@integerfalse
   \fi
  \fi
}

%<--------------------------------------------------------------------------–>
%              Setup   axe
%<--------------------------------------------------------------------------–>
\pgfkeys{tkzaxis/.cd,
      line width/.code      = \xdef\tkz@sua@lw{#1},
      color/.code           = \xdef\tkz@sua@color{#1},
      tickwd/.code          = \xdef\tkz@sua@tickwd{#1},
      ticka/.code           = \xdef\tkz@sua@ticka{#1},
      tickb/.code           = \xdef\tkz@sua@tickb{#1},
      line width            = \tkz@init@lw,
      color                 = \tkz@init@color,
      tickwd                = \tkz@init@tickwd,
      ticka                 = \tkz@init@ticka,
      tickb                 = \tkz@init@tickb
} 

\def\tkzSetUpAxis{\pgfutil@ifnextchar[{\tkz@SetUpAxis}{\tkz@SetUpAxis[]}} 
\def\tkz@SetUpAxis[#1]{%
\begingroup
\pgfqkeys{/tkzaxis}{#1}
\global\let\tkz@init@lw\tkz@sua@lw
\global\let\tkz@init@gradsize\tkz@sua@gradsize 
\global\let\tkz@init@color\tkz@sua@color 
\global\let\tkz@init@tickwd\tkz@sua@tickwd 
\global\let\tkz@init@ticka\tkz@sua@ticka 
\global\let\tkz@init@tickb\tkz@sua@tickb  
\endgroup
}
%<--------------------------------------------------------------------------–>
%                 tkzDrawX      todo améliorer les unités
% sans doute à revoir loop from 0 to i then calcul dans la boucle de la position
% et de l'affichage
%<--------------------------------------------------------------------------–>
\pgfkeys{%
  /tkzdrawX/.cd,
  color/.store in            = \tkz@X@color,
  label/.store in            = \tkz@X@label,
  right space/.store in      = \tkz@axe@rxspace,
  left space/.store in       = \tkz@axe@lxspace,
  step/.code                 = {\edef\tkz@posnext{\fpeval{#1}}},
  color                      = \tkz@init@color,
  label                      = \tkz@init@xlabel,
  step                       = \tkz@init@xstep,
  right space                = \tkz@init@rightspace, %???
  left space                 = \tkz@init@leftspace,
  noticks/.is if             = tkz@X@noticks,
  noticks/.default           = true,
  noticks                    = true,
  tickwd/.store in           = \tkz@X@tickwd,
  tickup/.store in           = \tkz@X@tickup,
  tickdn/.store in           = \tkz@X@tickdn,
  tickwd                     = \tkz@init@tickwd,
  tickup                     = \tkz@init@ticka,
  tickdn                     = \tkz@init@tickb,
   /tkzdrawX/.search also={/tikz}, 
  }

\def\tkzDrawX{\pgfutil@ifnextchar[{\tkz@DrawX}{\tkz@DrawX[]}}
\def\tkz@DrawX[#1]{
\begingroup%
\pgfqkeys{/tkzdrawX}{#1}
\edef\tkz@posmax{\fpeval{trunc(\tkz@xb,\tkz@init@xdec)}}
\edef\tkz@posmin{\fpeval{trunc(\tkz@xa,\tkz@init@xdec)}}
\edef\tkz@xbsup{\fpeval{\tkz@xb+\tkz@axe@rxspace}}
\edef\tkz@xainf{\fpeval{\tkz@xa-\tkz@axe@lxspace}}
\path (\tkz@xainf,0)--(\tkz@xbsup,0) node(tkz@xline){};
\draw[xaxe style,
      color = \tkz@X@color, 
      /tkzdrawX/.cd, #1] (\tkz@xainf,0)--(\tkz@xbsup,0)
                        node[ xlabel style, 
                           /tkzdrawX/.cd, 
                          #1]{\tkz@X@label};
 \iftkz@X@noticks
 \else
  \edef\tkz@posmax{\fpeval{trunc(\tkz@posmax,\tkz@init@xdec)}}   
  \edef\tkz@posnext{\fpeval{\tkz@posnext/\tkz@init@xstep+\tkz@posmin}}
     \foreach \pos in {\tkz@posmin,...,\tkz@posmax}{%
         \edef\tkz@pos{\fpeval{\pos*1}}% ???
         \draw[ color         = \tkz@X@color,
                line width    = \tkz@X@tickwd,
                shift         = {(\tkz@pos,0)}]%
                (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn);
           }
 \fi
\endgroup
}
%<--------------------------------------------------------------------------–>
%                 tkzDrawY      todo améliorer les unités
%<--------------------------------------------------------------------------–>
\pgfkeys{%
  /tkzdrawY/.cd,
  color/.store in            = \tkz@Y@color,
  label/.store in            = \tkz@Y@label, 
  up space/.store in         = \tkz@axe@uyspace, 
  down space/.store in       = \tkz@axe@dyspace,
  step/.code                 = {\edef\tkz@posnext{\fpeval{#1}}},  
  color                      = \tkz@init@color,
  label                      = \tkz@init@ylabel,
  step                       = \tkz@init@ystep,
  up space                   = \tkz@init@upspace,
  down space                 = \tkz@init@downspace,
  noticks/.is if             = tkz@Y@noticks,
  noticks/.default           = true,
  noticks                    = true,
  tickwd/.store in           = \tkz@Y@tickwd,
  ticklt/.store in           = \tkz@Y@ticklt,
  tickrt/.store in           = \tkz@Y@tickrt,
  tickwd                     = \tkz@init@tickwd,
  ticklt                     = \tkz@init@tickb,
  tickrt                     = \tkz@init@ticka,
   /tkzdrawY/.search also={/tikz},    
        }
                                     
\def\tkzDrawY{\pgfutil@ifnextchar[{\tkz@DrawY}{\tkz@DrawY[]}}
\def\tkz@DrawY[#1]{%
\begingroup
\pgfkeys{/tkzdrawY/.cd,step = \tkz@init@ystep}
\pgfqkeys{/tkzdrawY}{#1}
\edef\tkz@posmax{\fpeval{trunc(\tkz@yb,\tkz@init@ydec)}}
\edef\tkz@posmin{\fpeval{trunc(\tkz@ya,\tkz@init@ydec)}}
\edef\tkz@ybsup{\fpeval{\tkz@yb+\tkz@axe@uyspace}}
\edef\tkz@yainf{\fpeval{\tkz@ya-\tkz@axe@dyspace}}
\path (0,\tkz@yainf)--(0,\tkz@ybsup) node(tkz@yline){};
\draw[color = \tkz@Y@color,
      yaxe style,/tkzdrawY/.cd,#1] (0,\tkz@yainf)--(0,\tkz@ybsup)
      node[ylabel style,/tkzdrawY/.cd,#1]{\tkz@Y@label};
 \iftkz@Y@noticks
 \else 
    \edef\tkz@posmax{\fpeval{trunc(\tkz@posmax,\tkz@init@ydec)}}    
    \edef\tkz@posnext{\fpeval{\tkz@posnext/\tkz@init@ystep+\tkz@posmin}}
   \foreach \tkz@pos in {\tkz@posmin,\tkz@posnext,...,\tkz@posmax}{% 
     \draw[color = \tkz@Y@color,
           line width = \tkz@Y@tickwd,
           shift       = {(0,\tkz@pos)}]% 
            (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt);}
    
 \fi        
\endgroup}
\makeatother
\endinput

==> tikz-euclide/obj/tkz-obj-eu-circles-by.tex <==
% tkz-obj-eu-circles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-circles.tex} 
\makeatletter
%<--------------------------------------------------------------------------–>
%            tkzCircle center and one point 
%<--------------------------------------------------------------------------–>
% attention radius circle is defined by center and a point on the circle
% R defined by center and the value of the radius
% no need to define a circle with R tikz uses this method.
% through instead of radius
\def\tkz@numcby{0}
\pgfkeys{/tkzDefCircleBy/.cd,
  translation/.code args = {from #1 to #2} {             \def\tkz@numcby{0}
                                                         \def\tkzfrom{#1}
                                                         \def\tkzto{#2}},
  homothety/.code args = {center #1 ratio #2}{           \def\tkz@numcby{1}
                                                         \def\tkzcenter{#1}
                                                         \def\tkzratio{#2}},
  reflection/.code args = {over #1--#2}{                 \def\tkz@numcby{2}
                                                         \def\tkzdeb{#1}
                                                         \def\tkzfin{#2}},
  symmetry/.code args = {center #1}{                     \def\tkz@numcby{3}
                                                         \def\tkzcenter{#1}},
  rotation/.code args = {center #1 angle #2}{            \def\tkz@numcby{4}
                                                         \def\tkzcenter{#1}
                                                         \def\tkzangle{#2}},
  inversion/.code args={center #1 through #2}{           \def\tkz@numcby{5}
                                                         \def\tkzcenter{#1}
                                                         \def\tkzpoint{#2}},
  inversion negative/.code args = {center #1 through #2}{\def\tkz@numcby{6}
                                                         \def\tkzcenter{#1}
                                                         \def\tkzpoint{#2}}
      } 
\def\tkzDefCircleBy{\pgfutil@ifnextchar[{\tkz@DefCircleBy}{\tkz@DefCircleBy[]}}
\def\tkz@DefCircleBy[#1](#2){% 
\begingroup  
\pgfqkeys{/tkzDefCircleBy}{#1}  
\ifcase\tkz@numcby%
  \tkzDefCircleTranslation(#2)%
  \or% 1 
  \tkzDefCircleHomothety(#2)  
  \or% 2
  \tkzDefCircleReflection(#2) 
  \or% 3
  \tkzDefCircleSymmetry(#2) 
  \or% 4
  \tkzDefCircleRotation(#2) 
  \or% 5
  \tkzDefInversionCircle(#2,\tkzcenter,\tkzpoint) 
  \or% 6
  \tkzDefInversionNegativeCircle(#2,\tkzcenter,\tkzpoint) 
\fi    
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleTranslation(#1,#2){%
\begingroup 
   \tkzUTranslation(\tkzfrom,\tkzto)(#1)
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
   \tkzUTranslation(\tkzfrom,\tkzto)(#2)
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}  
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleHomothety(#1,#2){%
\begingroup 
   \tkzUHomo(\tkzcenter,\tkzratio)(#1)
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
   \tkzUHomo(\tkzcenter,\tkzratio)(#2)
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleReflection(#1,#2){%
\begingroup 
   \tkzUSymOrth(\tkzdeb,\tkzfin)(#1) 
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \tkzUSymOrth(\tkzdeb,\tkzfin)(#2) 
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleSymmetry(#1,#2){%
\begingroup 
   \tkzUCSym(\tkzcenter)(#1)
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
   \tkzUCSym(\tkzcenter)(#2)
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleRotation(#1,#2){%
\begingroup 
   \tkzURotateAngle(\tkzcenter,\tkzangle)(#1)
    \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
    \tkzURotateAngle(\tkzcenter,\tkzangle)(#2)
    \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
%<--------------------------------------------------------------------------–>
% #3,#4 cercle d'inversion centre #3. through #4
% Si le cercle passe par le pôle l'image est une droite
\def\tkzDefInversionCircle(#1,#2,#3,#4){%  
\begingroup
    \tkz@@CalcLengthcm(#1,#2){tkz@lna}% 
    \tkz@@CalcLengthcm(#1,#3){tkz@lnb}% 
    \gdef\tkzMathResult{\fpeval{round(abs(\tkz@lnb - \tkz@lna),6)}}
    \ifdim\tkzMathResult pt < 1 pt\relax%
    \tkzURotateAngle(#1,-90)(#2)
    \pgfnodealias{tkz@a}{tkzPointResult}
    \tkzUInversePoint(#3,#4)(tkz@a)
    \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
    \tkzUInversePoint(#3,#4)(#2)
    \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
     \else
    \tkzURotateAngle(#1,90)(#2)
    \pgfnodealias{tkz@a}{tkzPointResult}
    \tkzURotateAngle(#1,-90)(#2)
    \pgfnodealias{tkz@b}{tkzPointResult}
    \tkzUInversePoint(#3,#4)(tkz@a)
    \pgfnodealias{tkz@p1}{tkzPointResult}
    \tkzUInversePoint(#3,#4)(tkz@b)
    \pgfnodealias{tkz@p2}{tkzPointResult}
    \tkzUInversePoint(#3,#4)(#2)    
    \pgfnodealias{tkz@p3}{tkzPointResult}
    \tkzDefCircle[circum](tkz@p3,tkz@p1,tkz@p2)
    \fi
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzDefInversionNegativeCircle(#1,#2,#3,#4){%
\begingroup
   \tkzDefInversionCircle(#1,#2,#3,#4)
   \tkzUCSym(\tkzcenter)(tkzFirstPointResult)
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
   \tkzUCSym(\tkzcenter)(tkzSecondPointResult)
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
%<--------------------------------------------------------------------------–>
%              End Def Circle
%<--------------------------------------------------------------------------–>  
\makeatother 
\endinput

==> tikz-euclide/obj/tkz-obj-eu-circles.tex <==
% tkz-obj-eu-circles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-circles.tex} 
\makeatletter
%<--------------------------------------------------------------------------–>
%            tkzCircle center and one point 
%<--------------------------------------------------------------------------–>
% attention radius circle is defined by center and a point on the circle
% R defined by center and the value of the radius
% no need to define a circle with R tikz uses this method.
% through instead of radius
\def\tkz@numc{0}
\pgfkeys{/tkzcircle/.cd,
      R/.code                                   = \def\tkz@numc{0},
      diameter/.code                            = \def\tkz@numc{1},
      circum/.code                              = \def\tkz@numc{2},
      in/.code                                  = \def\tkz@numc{3},
      ex/.code                                  = \def\tkz@numc{4},
      euler/.code                               = \def\tkz@numc{5},
      nine/.code                                = \def\tkz@numc{5},
      apollonius/.code                          = \def\tkz@numc{6},
      spieker/.code                             = \def\tkz@numc{7},
      orthogonal from/.code args                = {#1}{\gdef\tkz@numc{8}
                                                   \def\tkz@ptfrom{#1}}, 
      orthogonal through/.code args             = {#1 and #2}{\gdef\tkz@numc{9}
                                                   \def\tkz@ptone{#1}
                                                   \def\tkz@pttwo{#2}},
      K/.code                                   = \def\tkz@koeff{#1},
      K                                         =  1,
      circum
      } 
\def\tkzDefCircle{\pgfutil@ifnextchar[{\tkz@DefCircle}{\tkz@DefCircle[]}}
\def\tkz@DefCircle[#1](#2){% 
\begingroup  
\pgfqkeys{/tkzcircle}{#1}  
\ifcase\tkz@numc%
  \tkzDefCircleR(#2)
  \or% 1 
  \tkzDefCircleD(#2)  
  \or% 2
  \tkzDefCircumCircle(#2) 
  \or% 3
  \tkzDefInCircle(#2) 
  \or% 4
  \tkzDefExCircle(#2) 
  \or% 5
  \tkzDefEulerCircle(#2)
  \or% 6
  \tkzDefApolloniusCircle(#2) 
  \or% 7
  \tkzDefSpiekerCircle(#2)
   \or% 8
  \tkzDefOrthogonalCircle(#2,\tkz@ptfrom)
   \or% 9
  \tkzDefOrthoThroughCircle(#2,\tkz@ptone,\tkz@pttwo)
     \fi    
\endgroup
}
%for compatibility
%<--------------------------------------------------------------------------–>
%                     R
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleR(#1,#2){% 
\begingroup 
   \edef\tkzLengthResult{\fpeval{round(#2,5)}}
   \global\let\tkzLengthResult\tkzLengthResult
   \path (#1)--++(\tkzLengthResult,0) coordinate (tkzSecondPointResult);
   \tkzRenamePoint(tkzSecondPointResult){tkzPointResult}
\endgroup
} 

%<--------------------------------------------------------------------------–>
%              Diameter Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefCircleD(#1,#2){% 
\begingroup
  \tkzDefMidPoint(#1,#2)
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \pgfnodealias{tkzSecondPointResult}{#2}
  \tkz@@CalcLengthcm(#1,tkzPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Circum Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefCircumCircle(#1,#2,#3){%
\begingroup
  \tkzCircumCenter(#1,#2,#3)
  \tkzRenamePoint(tkzPointResult){tkzFirstPointResult}
  \tkzRenamePoint(#1){tkzSecondPointResult}
  \tkz@@CalcLengthcm(#1,tkzPointResult){tkzLengthResult}%3.06 add [cm]
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              In(scribe) Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefInCircle(#1,#2,#3){%
\begingroup
  \tkzInCenter(#1,#2,#3) 
  \pgfnodealias{tkz@incenter}{tkzPointResult}
  \tkzUProjection(#1,#3)(tkz@incenter) 
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
  \tkz@@CalcLengthcm(tkzPointResult,tkz@incenter){tkzLengthResult}
  \pgfnodealias{tkzPointResult}{tkz@incenter}
  \pgfnodealias{tkzFirstPointResult}{tkz@incenter}
\endgroup
}  
%<--------------------------------------------------------------------------–>
%              Ex(scribe) Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefExCircle(#1,#2,#3){%
\begingroup
  \tkzExCenter(#1,#2,#3) 
  \pgfnodealias{tkz@excenter}{tkzPointResult}
  \tkzUProjection(#1,#3)(tkz@excenter)
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
  \tkz@@CalcLengthcm(tkzPointResult,tkz@excenter){tkzLengthResult}% for tkzGetLength
  \pgfnodealias{tkzPointResult}{tkz@excenter}
  \pgfnodealias{tkzFirstPointResult}{tkz@excenter}  
\endgroup
}
%<--------------------------------------------------------------------------–>
%              Radius Ex Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefExRadius(#1,#2,#3){%
\begingroup
   \tkzExCenter(#1,#2,#3)
   \tkzUProjection(#1,#3)(tkzPointResult)
\endgroup
}    
%<--------------------------------------------------------------------------–>
% The nine-point circle, also called Euler's circle or the Feuerbach circle  
% best way Ma,Mb,Mc circum center  2020
%<--------------------------------------------------------------------------–>
\def\tkzDefEulerCircle(#1,#2,#3){%
\begingroup
 \tkzDefMidPoint(#1,#2) \pgfnodealias{tkz@e1}{tkzPointResult}
 \tkzDefMidPoint(#2,#3) \pgfnodealias{tkz@e2}{tkzPointResult}
 \tkzDefMidPoint(#1,#3) \pgfnodealias{tkz@e3}{tkzPointResult}
 \tkzCircumCenter(tkz@e1,tkz@e2,tkz@e3) 
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}  
 \tkzRenamePoint(tkz@e1){tkzSecondPointResult}
 \tkz@@CalcLengthcm(tkzPointResult,tkz@e1){tkzLengthResult}
\endgroup
} 
\let\tkzDefNinePointsCircle\tkzEulerCircle%
\let\tkzFeuerBachCircle\tkzEulerCircle%  

\def\tkzDefEulerRadius(#1,#2,#3){%
\begingroup
   \tkzEulerCenter(#1,#2,#3)
   \pgfnodealias{eur@pta}{tkzPointResult}   
   \tkzDefMidPoint(#1,#2)  
  \tkz@@CalcLengthcm(eur@pta,tkzPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>
%                     Apollonius circle
%<--------------------------------------------------------------------------–>
\def\tkzDefApolloniusCircle(#1,#2){%
\begingroup
  \tkzDefBarycentricPoint(#1=1,#2=\tkz@koeff)
  \pgfnodealias{apo@pta}{tkzPointResult} 
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}  
  \tkzDefBarycentricPoint(#1=1,#2=-\tkz@koeff)  
  \pgfnodealias{apo@ptb}{tkzPointResult} 
  \tkzDefMidPoint(apo@pta,apo@ptb)  
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult} 
  \tkz@@CalcLengthcm(tkzFirstPointResult,apo@pta){tkzLengthResult}  
  \pgfnodealias{tkzThirdPointResult}{apo@ptb} 
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefOrthogonalCircle(#1,#2,#3){%   
\begingroup
   \tkzTgtFromP(#1,#2)(#3)
   \tkz@@CalcLengthcm(#1,tkzFirstPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzDefOrthoThroughCircle(#1,#2,#3,#4){%  
\begingroup
  \tkz@@CalcLengthcm(#1,#3){tkz@lnb}%
  \edef\tkz@lnc{\fpeval{1/\tkz@lnb}}
  \tkzVecKNorm[\tkz@lnc](#1,#3) 
  \pgfnodealias{tkz@PointResult}{tkzPointResult}
  \tkzCircumCenter(tkz@PointResult,#3,#4)
  \tkz@@CalcLengthcm(tkzPointResult,#3){tkzLengthResult}
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \pgfnodealias{tkzSecondPointResult}{#3}
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Spieker Circle
%<--------------------------------------------------------------------------–>
\def\tkzDefSpiekerCircle(#1,#2,#3){%
\begingroup
  \tkzSpiekerCenter(#1,#2,#3)
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \tkzUProjection(tkz@m1,tkz@m2)(tkzPointResult)
    \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
  \tkz@@CalcLength(tkzSecondPointResult,tkzFirstPointResult){tkzLengthResult}
\endgroup
} 
%<--------------------------------------------------------------------------–>

%<--------------------------------------------------------------------------–>
%              End Def Circle
%<--------------------------------------------------------------------------–>  
\makeatother 
\endinput

==> tikz-euclide/obj/tkz-obj-eu-grids.tex <==
% tkz-obj-eu-grids.tex    
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-grids.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%              Setup   Grid
%<--------------------------------------------------------------------------–>
\pgfkeys{/tkzsugrid/.cd,
    line width/.store in      = \tkz@sug@lw,
    color/.store in           = \tkz@sug@color,
    line width                = \tkz@grid@lw,
    color                     = \tkz@grid@color
        } 

\def\tkzSetUpGrid{\pgfutil@ifnextchar[{\tkz@SetUpGrid}{\tkz@SetUpGrid[]}} 
\def\tkz@SetUpGrid[#1]{%
\begingroup
\pgfqkeys{/tkzsugrid}{#1}
\global\let\tkz@grid@lw\tkz@sug@lw
\global\let\tkz@grid@color\tkz@sug@color 
\endgroup
}
%<--------------------------------------------------------------------------–>
%         tkzGrid  
%<--------------------------------------------------------------------------–>
\pgfkeys{/tkzGrid/.cd,
  color/.code           = {\def\tkz@gd@color{#1}%
                            \edef\tkz@gd@subcolor{%
                            \tkz@gd@color!\tkzCoeffSubColor}},
  subxstep/.store in    = {\tkz@gd@subxstep},
  subystep/.store in    = {\tkz@gd@subystep},
  ratio/.store in       = {\tkz@gd@ratio},
  line width/.code      = {\edef\tkz@gd@lw{#1}
                            \edef\tkz@gd@sublw{\tkz@gd@ratio\tkz@gd@lw}},
  sub/.is if            = tkz@gd@sub,
  sub/.default          = true ,
  sub                   = false,
  color                 = \tkz@grid@color,
  ratio                 = 0.75, 
  subxstep              = \tkz@grid@xstep,
  subystep              = \tkz@grid@ystep,
  line width            = \tkz@grid@lw,
  /tkzGrid/.search also= {/tikz},
} 
%<--------------------------------------------------------------------------–>
\def\tkzGrid{\pgfutil@ifnextchar[{\tkz@Grid}{\tkz@Grid[]}}
\def\tkz@Grid[#1]{\@ifnextchar({\tkz@@Grid[#1]}%
                               {\tkz@@Grid[#1](\tkz@tmp@xa,\tkz@tmp@ya)(\tkz@tmp@xb,\tkz@tmp@yb)}}
\def\tkz@@Grid[#1](#2,#3)(#4,#5){%
  \pgfqkeys{/tkzGrid}{#1}   
    \begingroup
   \edef\tkz@gxa{\fpeval{(#2-\tkz@init@xorigine)/\tkz@init@xstep}}
   \edef\tkz@gxb{\fpeval{(#4-\tkz@init@xorigine)/\tkz@init@xstep}}
   \edef\tkz@gya{\fpeval{(#3-\tkz@init@yorigine)/\tkz@init@ystep}}
   \edef\tkz@gyb{\fpeval{(#5-\tkz@init@yorigine)/\tkz@init@ystep}}
    \iftkz@gd@sub% 
      \edef\@subxstep{\fpeval{\tkz@gd@subxstep/\tkz@init@xstep}}%
      \edef\@subystep{\fpeval{\tkz@gd@subystep/\tkz@init@ystep}}%
      \draw [xstep      = \@subxstep cm,%
             ystep      = \@subystep cm,%
             color      = \tkz@gd@subcolor,%
             line width = \tkzRatioLineGrid]%
             (\tkz@gxa,\tkz@gya) grid (\tkz@gxb,\tkz@gyb);%
    \fi
    \draw [color      = \tkz@gd@color,%
           line width = \tkz@gd@lw]%
           (\tkz@gxa,\tkz@gya) grid (\tkz@gxb,\tkz@gyb);%
    \endgroup
}%
\makeatother
\endinput

==> tikz-euclide/obj/tkz-obj-eu-lines.tex <==
% tkz-obj-eu-lines.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-lines.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%                          les lignes
%<--------------------------------------------------------------------------–>
\def\tkz@numline{0}
\pgfkeys{/tkzdefline/.cd,
  mediator/.code           =  \def\tkz@numline{0},
  perpendicular/.code args =  {through #1} {\def\tkz@numline{1}%
                                            \def\tkz@through{#1}},
  orthogonal/.code args    =  {through #1} {\def\tkz@numline{1}%
                                            \def\tkz@through{#1}}, 
  parallel/.code args      =  {through #1}{\def\tkz@numline{2}%
                                           \def\tkz@through{#1}},   
  bisector/.code           =  \def\tkz@numline{3},
  bisector out/.code       =  \def\tkz@numline{4},
  symmedian/.code          =  \def\tkz@numline{5},
  altitude/.code           =  \def\tkz@numline{6},
  euler/.code              =  \def\tkz@numline{7},
  tangent from/.code       =  \def\tkz@numline{8} \def\tkz@ptfrom{#1},
  tangent at/.code         =  \def\tkz@numline{9} \def\tkz@ptat{#1},
  K/.code                  =  \def\tkz@koeff{#1},
  K                        =  1,
  normed/.is if            =  tkz@line@normed,
  normed/.default          =  true,
  normed                   =  false,
  mediator
} 
\def\tkzDefLine{\pgfutil@ifnextchar[{\tkz@DefLine}{\tkz@DefLine[]}}
\def\tkz@DefLine[#1](#2){% 
\begingroup
%\pgfkeys{/tkzdefline/.cd,K=1}  
\pgfqkeys{/tkzdefline}{#1}  
\ifcase\tkz@numline%
 % first case 0
 \tkzDefMediatorLine(#2)  
  \or% 1
  \tkzDefOrthLine[\tkz@koeff](#2)
  \or% 2
   \tkzDefLineLL(#2)
  \or% 3
  \tkzDefBisectorLine(#2)
  \or% 4
  \tkzDefBisectorOutLine(#2)
  \or% 5
  \tkzDefSymmedianLine(#2)
    \or% 6
  \tkzDefAltitudeLine(#2)
  \or% 7
   \tkzDefEulerLine(#2)
   \or% 8
   \tkzTgtFromP(#2)(\tkz@ptfrom)
 \or% 9
   \tkzTgtAt(#2)(\tkz@ptat)
  \fi    
\endgroup
}
%<--------------------------------------------------------------------------–>
%                            tkzLineLL    revoir out !!
%<--------------------------------------------------------------------------–>
\def\tkzDefLineLL{\pgfutil@ifnextchar[{\tkz@DefLineLL}{%
                                         \tkz@DefLineLL[1]}} 
\def\tkz@DefLineLL[#1](#2,#3){% 
\begingroup
   \pgfpointdiff{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x\relax%%
   \pgf@ya=\pgf@y\relax%%
   \pgfinterruptboundingbox 
   \path[coordinate](\tkz@through)--++(\tkz@koeff\pgf@xa,\tkz@koeff\pgf@ya)%
         coordinate (tkzPointResult);
   \endpgfinterruptboundingbox
   \iftkz@line@normed
      \tkzVecKNorm(\tkz@through,tkzPointResult)
   \fi
\endgroup}% 
%<--------------------------------------------------------------------------–>
%                        tkzOrthLine 
%<--------------------------------------------------------------------------–>
\def\tkzDefOrthLine{\pgfutil@ifnextchar[{\tkz@DefOrthLine}{%
                                         \tkz@DefOrthLine[1]}} 
\def\tkz@DefOrthLine[#1](#2,#3){% 
\begingroup
 \tkzDefPointWith(#2,#3) 
  \pgfnodealias{tkz@OLtmp}{tkzPointResult}
  \tkz@VecKCoLinear[\tkz@koeff](#2,tkz@OLtmp,\tkz@through)
  \iftkz@line@normed
    \pgfinterruptboundingbox 
       \tkzVecKNorm(\tkz@through,tkzPointResult)
    \endpgfinterruptboundingbox 
  \fi
\endgroup}% 
%<--------------------------------------------------------------------------–>
%                            tkzMediatorLine
%<--------------------------------------------------------------------------–>
\def\tkzDefMediatorLine{\pgfutil@ifnextchar[{\tkz@DefMediatorLine}{%
                                             \tkz@DefMediatorLine[1]}} 

\def\tkz@DefMediatorLine[#1](#2,#3){% new 2020 
\begingroup
   \tkzDefEquilateral(#2,#3) 
   \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
   \tkzDefEquilateral(#3,#2)
   \pgfnodealias{tkzSecondPointResult}{tkzPointResult} 
   \ifx\tkz@koeff=1 %
   \else
     \tkzDefMidPoint(#2,#3)
     \pgfnodealias{tkz@mid}{tkzPointResult}
     \tkz@VecK[\tkz@koeff](tkz@mid,tkzFirstPointResult)
     \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
     \tkz@VecK[\tkz@koeff](tkz@mid,tkzSecondPointResult)
     \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
   \fi
   \iftkz@line@normed 
      \tkzDefMidPoint(#2,#3)
      \pgfnodealias{tkz@mid}{tkzPointResult}
     % \pgfinterruptboundingbox
         \tkzVecKNorm[\tkz@koeff](tkz@mid,tkzFirstPointResult)
         \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
         \tkzVecKNorm[\tkz@koeff](tkz@mid,tkzSecondPointResult)
         \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
    %  \endpgfinterruptboundingbox
   \fi
\endgroup}
% autre possibilité

%<--------------------------------------------------------------------------–>
%              BisectorLine  
%<--------------------------------------------------------------------------–>
\def\tkzDefBisectorLine(#1,#2,#3){% 
\begingroup
  \pgfinterruptboundingbox 
  \tkzDuplicateSegment(#2,#1)(#2,#3)
  \pgfnodealias{bi@tmp}{tkzPointResult}  
  \tkzDefMidPoint(bi@tmp,#1)
%  \tkzDefEquilateral(bi@tmp,#1)
  \ifx\tkz@koeff=1 %
  \else
    \tkzVecK[\tkz@koeff](#2,tkzPointResult)
  \fi
  \iftkz@line@normed
     \tkzVecKNorm[\tkz@koeff](#2,tkzPointResult)
    \fi
    \endpgfinterruptboundingbox 
\endgroup
}
%<--------------------------------------------------------------------------–>
%              Out BisectorLine
%<--------------------------------------------------------------------------–>
\def\tkzDefBisectorOutLine(#1,#2,#3){% 
\begingroup
\pgfinterruptboundingbox 
   \tkzDuplicateLength(#2,#1)(#2,#3)
   \pgfnodealias{out@tmp}{tkzPointResult}
   \tkzDefMidPoint(#1,out@tmp) 
   \pgfnodealias{out@pt1}{tkzPointResult}
   \tkzURotateAngle(#2,90)(out@pt1)
   \ifx\tkz@koeff=1 %
   \else
     \tkzVecK[\tkz@koeff](#2,tkzPointResult)
   \fi
   \iftkz@line@normed
     \tkzVecKNorm[\tkz@koeff](#2,tkzPointResult)
    \fi
\endpgfinterruptboundingbox 
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Symmedian line
%<--------------------------------------------------------------------------–>
\def\tkzDefSymmedianLine(#1,#2,#3){% 
\begingroup
  \tkzDefBisectorLine(#1,#2,#3)
  \pgfnodealias{sym@pt1}{tkzPointResult}
  \tkzDefMidPoint(#1,#3)
  \pgfnodealias{sym@pt2}{tkzPointResult}
  \tkzUSymOrth(#2,sym@pt1)(sym@pt2)
   \ifx\tkz@koeff=1 %
   \else
     \tkzVecK[\tkz@koeff](#2,tkzPointResult)
   \fi
  \iftkz@line@normed
    \tkzVecKNorm[\tkz@koeff](#2,tkzPointResult)
  \fi
\endgroup
}
%<--------------------------------------------------------------------------–>
%              Altitude Line
%<--------------------------------------------------------------------------–>
\def\tkzDefAltitudeLine(#1,#2,#3){%
\begingroup
   \pgfinterruptboundingbox
   \tkzUProjection(#1,#3)(#2)
   \pgfnodealias{ort@pta}{tkzPointResult}
   \endpgfinterruptboundingbox  
\endgroup
}
%<--------------------------------------------------------------------------–>
%              Euler Line
%<--------------------------------------------------------------------------–>
\def\tkzDefEulerLine(#1,#2,#3){%
\begingroup
  \pgfinterruptboundingbox
  \tkzOrthoCenter(#1,#2,#3)  
  \pgfnodealias{euler@pt1}{tkzPointResult}
   \tkzEulerCenter(#1,#2,#3)  
   \pgfnodealias{euler@pt2}{tkzPointResult}
   \pgfnodealias{tkzSecondPointResult}{euler@pt2}
   \pgfnodealias{tkzFirstPointResult}{euler@pt1}
   \endpgfinterruptboundingbox  
\endgroup
}
%<--------------------------------------------------------------------------–>
%    tangente à cercle passant par un point donné
%<--------------------------------------------------------------------------–>
   
\def\tkzTgtAt(#1)(#2){%
\begingroup
     \tkz@VecKOrthNorm[-1](#2,#1)  
 \endgroup
}
%<-------------------------------------------------------------------------–> 
\def\tkzTgtFromP(#1,#2)(#3){%
\begingroup
    \tkz@@CalcLengthcm(#1,#2){tkz@radone}
    \tkzDefMidPoint(#1,#3) 
    \tkz@@CalcLengthcm(tkzPointResult,#1){tkz@radtwo}
    \tkzInterCCR(#1,\tkz@radone)(tkzPointResult,\tkz@radtwo){%
    tkzFirstPointResult}{tkzSecondPointResult}%
    \tkzFindAngle(#3,tkzFirstPointResult,#1)   \tkzGetAngle{tkz@an}
    \ifdim\tkz@an pt<180 pt\relax%
    \else
    \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
    \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
    \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
    \fi
\endgroup
} 
%<-------------------------------------------------------------------------–>  
\def\tkzTgtFromPR(#1,#2)(#3){%
\begingroup
    \tkzDefMidPoint(#1,#3)
    \tkz@@CalcLengthcm(tkzPointResult,#1){tkzLengthResult}
    \tkzInterCCR(#1,#2)(tkzPointResult,\tkzLengthResult){%
    tkzFirstPointResult}{%
    tkzSecondPointResult}%
    \tkzFindAngle(#3,tkzFirstPointResult,#1)   \tkzGetAngle{tkz@an}
    \ifdim\tkz@an pt<180 pt\relax%
    \else
    \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
    \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
    \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
    \fi
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkz@numtang{0}
\pgfkeys{/tkz@tang/.cd,
  at/.code          = {\def\tkz@numtang{0}\def\tkz@ptat{#1}},
  from/.code        = {\def\tkz@numtang{1}\def\tkz@ptfrom{#1}},
  from with R/.code = {\def\tkz@numtang{2}\def\tkz@ptfrom{#1}}
  }
%<--------------------------------------------------------------------------–>
\def\tkzDefTangent{\pgfutil@ifnextchar[{\tkz@Tangent}{\tkz@Tangent[]}}

\def\tkz@Tangent[#1](#2){%
\begingroup
\pgfkeys{tkz@tang/.cd}
\pgfqkeys{/tkz@tang}{#1}
\ifcase\tkz@numtang
    \tkzTgtAt(#2)(\tkz@ptat)
\or
   \tkzTgtFromP(#2)(\tkz@ptfrom)
 \or
   \tkzTgtFromPR(#2)(\tkz@ptfrom)
\fi 
\endgroup
}   
\makeatother
\endinput

==> tikz-euclide/obj/tkz-obj-eu-points-by.tex <==
% tkz-tools-eu-points-by.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-points-by.tex}  
\makeatletter
%<--------------------------------------------------------------------------–>
%                        Transformations Géométriques
%<--------------------------------------------------------------------------–>
\def\tkz@numtrsf{0}
\pgfkeys{/tkzDefPointBy/.cd,
 translation/.code args={from #1 to #2}{               \def\tkzfrom{#1}%
                                                       \def\tkzto{#2}%
                                                       \def\tkz@numtrsf{0}},
 homothety/.code args={center #1 ratio #2}{            \def\tkzcenter{#1}%
                                                       \def\tkzratio{#2}%
                                                       \def\tkz@numtrsf{1}},
 reflection/.code args={over #1--#2}{                  \def\tkzdeb{#1}%
                                                       \def\tkzfin{#2}%
                                                       \def\tkz@numtrsf{2}},
 symmetry/.code args={center #1}{                      \def\tkzcenter{#1}%
                                                       \def\tkz@numtrsf{3}},
 projection/.code args={onto #1--#2}{                  \def\tkzdeb{#1}%
                                                       \def\tkzfin{#2}%  
                                                       \def\tkz@numtrsf{4}}, 
 rotation/.code args={center #1 angle #2}{             \def\tkzcenter{#1}%
                                                       \def\tkzangle{#2}%
                                                       \def\tkz@numtrsf{5}},
 rotation in rad/.code args={center #1 angle #2}{      \def\tkzcenter{#1}%
                                                       \def\tkzangle{#2}%
                                                       \def\tkz@numtrsf{6}},
 inversion/.code args={center #1 through #2}{          \def\tkzcenter{#1}%
                                                       \def\tkzpoint{#2}%
                                                       \def\tkz@numtrsf{7}},
 inversion negative/.code args={center #1 through #2}{ \def\tkzcenter{#1}%
                                                       \def\tkzpoint{#2}%
                                                       \def\tkz@numtrsf{8}},
 rotation with nodes/.code  args={center #1 from #2 to #3}{  \def\tkzcenter{#1}%
                                                            \def\tkzfrom{#2}%
                                                            \def\tkzto{#3}%
                                                            \def\tkz@numtrsf{9}}
}
%<--------------------------------------------------------------------------–>
\def\tkzDefPointBy{\pgfutil@ifnextchar[{\tkz@DefPointBy}{\tkz@DefPointBy[]}}
\def\tkz@DefPointBy[#1](#2){% 
\begingroup 
\pgfqkeys{/tkzDefPointBy}{#1}    
 \ifcase\tkz@numtrsf%
%  % first case 0   
   \tkzUTranslation(\tkzfrom,\tkzto)(#2) 
\or% 1
   \tkzUHomo(\tkzcenter,\tkzratio)(#2)
\or% 2
   \tkzUSymOrth(\tkzdeb,\tkzfin)(#2) 
\or% 3
   \tkzUCSym(\tkzcenter)(#2)
\or% 4
   \tkzUProjection(\tkzdeb,\tkzfin)(#2)  
\or% 5  
   \tkzURotateAngle(\tkzcenter,\tkzangle)(#2)
\or% 6 
   \tkzURotateInRad(\tkzcenter,\tkzangle)(#2)
\or% 7
   \tkzUInversePoint(\tkzcenter,\tkzpoint)(#2)     
\or% 8
   \tkzUInverseNegativePoint(\tkzcenter,\tkzpoint)(#2)   
\or% 9
   \tkzURotateWithNodes(\tkzcenter,\tkzfrom,\tkzto)(#2)
\fi   
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefPointsBy{\pgfutil@ifnextchar[{\tkz@DefPointsBy}{\tkz@DefPointsBy[]}}
\def\tkz@DefPointsBy[#1](#2)#3{% 
\begingroup
\pgfqkeys{/tkzDefPointBy}{#1}  
\ifcase\tkz@numtrsf%
 % first case 0
   \tkzTranslation(\tkzfrom,\tkzto)(#2){#3}  
 \or% 1
   \tkzHomo(\tkzcenter,\tkzratio)(#2){#3}
 \or% 2
   \tkzSymOrth(\tkzdeb,\tkzfin)(#2){#3} 
 \or% 3
   \tkzCSym(\tkzcenter)(#2){#3}
 \or% 4
   \tkzProjection(\tkzdeb,\tkzfin)(#2){#3}
 \or% 5
   \tkzRotateAngle(\tkzcenter,\tkzangle)(#2){#3}
 \or% 6
   \tkzRotateInRad(\tkzcenter,\tkzangle)(#2){#3}
 \or% 7
   \tkzInversePoint(\tkzcenter,\tkzpoint)(#2){#3}    
 \or% 8
   \tkzInverseNegativePoint(\tkzcenter,\tkzpoint)(#2){#3}
   \or% 9
 \tkzRotateWithNodes(\tkzcenter,\tkzfrom,\tkzto)(#2){#3}
\fi    
\endgroup
} 

%<--------------------------------------------------------------------------–>

\def\ExtractPoint#1,#2\@nil{% 
\xdef\tkz@LastList{#2}
\xdef\tkz@FirstPoint{#1}  
} 
\def\FirstPointInList#1{% 
\edef\tkz@templist{#1,}
\expandafter\ExtractPoint\tkz@templist\@nil
}
%<--------------------------------------------------------------------------–>
%  Translation par rapport à un point
%<--------------------------------------------------------------------------–>
\def\tkzTranslation(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
\foreach\PT in {#3}{%
   \FirstPointInList\tkz@LastList
    \ifx\tkz@FirstPoint\tkzutil@empty  
      \def\tkz@pointtsf{\PT '}
    \else
      \def\tkz@pointtsf{\tkz@FirstPoint}
    \fi 
   \tkz@VecCoLinear(#1,#2,\PT) 
    \pgfnodealias{\tkz@pointtsf}{tkzPointResult}       
   }  
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUTranslation(#1,#2)(#3){%
\begingroup 
  \tkz@VecCoLinear(#1,#2,#3)% 
\endgroup
}  

%<--------------------------------------------------------------------------–>
%  Symétrie par rapport à un point Homo with (-1) 
% #2 le centre #3 l'antécédent 
%<--------------------------------------------------------------------------–>
\def\tkzCSym(#1)(#2)#3{%
\begingroup
\gdef\tkz@LastList{#3}
 \foreach\PointCS in {#2}{%
   \FirstPointInList\tkz@LastList
   \ifx\tkz@FirstPoint\tkzutil@empty  
      \xdef\tkz@pointtsf{\PointCS '}
   \else
      \xdef\tkz@pointtsf{\tkz@FirstPoint}
   \fi 
     \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                  {\pgfpointanchor{\PointCS}{center}}%
     \tkz@ax=\pgf@x%
     \tkz@ay=\pgf@y%
      \pgfinterruptboundingbox
    \path(#1)--++(-\tkz@ax,-\tkz@ay)coordinate (\tkz@pointtsf); 
     \endpgfinterruptboundingbox
}       
\endgroup 
}
%<--------------------------------------------------------------------------–>
\def\tkzUCSym(#1)(#2){%
\begingroup
    \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                 {\pgfpointanchor{#2}{center}}%
    \tkz@ax=\pgf@x%
    \tkz@ay=\pgf@y%
   \path(#1)--++(-\tkz@ax,-\tkz@ay)coordinate (tkzPointResult); 
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%  Symétrie orthogonale par rapport à une droite
%<--------------------------------------------------------------------------–> 
\def\tkzSymOrth(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointSO in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \def\tkz@pointtsf{\PointSO '}
      \else
         \def\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
  \tkzUSymOrth(#1,#2)(\PointSO)    
  \pgfnodealias{\tkz@pointtsf}{tkzPointResult} 
  }    
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUSymOrth(#1,#2)(#3){%
\begingroup
   \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                {\pgfpointanchor{#2}{center}}%
   \tkz@ax =\pgf@y%
   \tkz@ay =\pgf@x%  
   \pgfinterruptboundingbox
   \path[coordinate] (#3)--++(-\tkz@ax,\tkz@ay) coordinate  (tkz@point);
     \endpgfinterruptboundingbox
   \tkzInterLL(#1,#2)(#3,tkz@point)
   \pgfnodealias{tkzPointofSym}{tkzPointResult}
   \tkz@VecK[2](#3,tkzPointofSym)
\endgroup
}

%<--------------------------------------------------------------------------–>
%  Projection orthogonale sur une droite
%<--------------------------------------------------------------------------–>
\def\tkzProjection(#1,#2)(#3)#4{%
\begingroup
\gdef\tkz@LastList{#4}
    \foreach\PointPJ in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty
         \def\tkz@pointtsf{\PointPJ '}
      \else
         \def\tkz@pointtsf{\tkz@FirstPoint}
      \fi
  \tkzUProjection(#1,#2)(\PointPJ)
  \pgfnodealias{\tkz@pointtsf}{tkzPointResult}
  }
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUProjection(#1,#2)(#3){%
\begingroup 
  \pgfpointdiff{\pgfpointanchor{#1}{center}}%
               {\pgfpointanchor{#2}{center}}%
  \tkz@ax =\pgf@y%
  \tkz@ay =\pgf@x%
  \pgfinterruptboundingbox
    \path[coordinate](#3)--++(-\tkz@ax,\tkz@ay) coordinate (tkz@point);
    \tkzInterLL(#1,#2)(#3,tkz@point)% définit tkzPointResult 
  \endpgfinterruptboundingbox
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkz@Projection(#1,#2)(#3)#4{%
\begingroup 
  \pgfpointdiff{\pgfpointanchor{#1}{center}}%
               {\pgfpointanchor{#2}{center}}%
  \tkz@ax =\pgf@y%
  \tkz@ay =\pgf@x%
   \pgfinterruptboundingbox
  \path[coordinate](#3)--++(-\tkz@ax,\tkz@ay) coordinate (tkz@point);
   \endpgfinterruptboundingbox
  \tkz@InterLL(#1,#2)(#3,tkz@point){#4}% définit tkzPointResult 
\endgroup
}
%<--------------------------------------------------------------------------–>
%  Homothétie par rapport à un point
%<--------------------------------------------------------------------------–>
\def\tkzHomo(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointHO in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointHO '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
       \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                    {\pgfpointanchor{\PointHO}{center}}%
       \pgf@xa=\pgf@x%
       \pgf@ya=\pgf@y% 
      \pgfmathparse{#2}\edef\tkz@coeff{\pgfmathresult}%
      \pgfinterruptboundingbox
      \path[coordinate](#1)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)%
            coordinate(\tkz@pointtsf);
     \endpgfinterruptboundingbox
  }  
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzUHomo(#1,#2)(#3){%
\begingroup 
       \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                    {\pgfpointanchor{#3}{center}}%
       \pgf@xa=\pgf@x%
       \pgf@ya=\pgf@y% 
      \pgfmathparse{#2}\edef\tkz@coeff{\pgfmathresult}%
        \pgfinterruptboundingbox
      \path[coordinate](#1)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)%
            coordinate(tkzPointResult);
              \endpgfinterruptboundingbox
\endgroup
}
%<--------------------------------------------------------------------------–>
%                 rotation  en degré
%<--------------------------------------------------------------------------–>
\def\tkzRotateAngle(#1,#2)(#3)#4{%
\begingroup
\gdef\tkz@LastList{#4}
    \foreach\PointRot in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \def\tkz@pointtsf{\PointRot '}
      \else
         \def\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
        \tkz@@extractxy{\PointRot}
        \tkz@ax\pgf@x%
        \tkz@ay\pgf@y%
        \tkz@@extractxy{#1}
        \tkz@bx\pgf@x%
        \tkz@by\pgf@y%
        \pgfmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                                 {\pgfpoint{\tkz@bx}{\tkz@by}}%
                                 {#2}
        \tkz@bx\pgf@x%
        \tkz@by\pgf@y%
          \pgfinterruptboundingbox
        \path[coordinate](\tkz@bx,\tkz@by)coordinate(\tkz@pointtsf);% 
          \endpgfinterruptboundingbox
        }   
  \endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzURotateAngle(#1,#2)(#3){%
\begingroup 
  \pgf@process{\pgfpointanchor{#3}{center}}%
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \pgf@process{\pgfpointanchor{#1}{center}}%
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \pgfmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {#2}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \pgfinterruptboundingbox
      \path (\tkz@bx,\tkz@by) coordinate (tkzPointResult);% 
    \endpgfinterruptboundingbox     
\endgroup
}   
%<--------------------------------------------------------------------------–>
% %                 rotation  en radian
% %<--------------------------------------------------------------------------–>
\def\tkzRotateInRad(#1,#2)(#3)#4{%
\begingroup
\gdef\tkz@LastList{#4}
    \foreach\PointRot in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointRot '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
   \pgfmathparse{#2 r}
   \let\tkz@Angle\pgfmathresult
    \tkz@@extractxy{\PointRot}
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \tkz@@extractxy{#1}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \pgfmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {\tkz@Angle}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
      \pgfinterruptboundingbox
    \path[coordinate](\tkz@bx,\tkz@by)coordinate(\tkz@pointtsf); 
      \endpgfinterruptboundingbox 
}  
\endgroup 
}
%<--------------------------------------------------------------------------–>
\def\tkzURotateInRad(#1,#2)(#3){%
\begingroup
   \pgfmathparse{#2 r}
   \let\tkz@Angle\pgfmathresult
    \tkz@@extractxy{#3}
    \tkz@ax\pgf@x%
    \tkz@ay\pgf@y%
    \tkz@@extractxy{#1}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
    \pgfmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                             {\pgfpoint{\tkz@bx}{\tkz@by}}%
                             {\tkz@Angle}
    \tkz@bx\pgf@x%
    \tkz@by\pgf@y%
      \pgfinterruptboundingbox
    \path[coordinate](\tkz@bx,\tkz@by)coordinate(tkzPointResult); 
      \endpgfinterruptboundingbox 
\endgroup 
}
%<--------------------------------------------------------------------------–>
%                   Inverse of a point 
%<--------------------------------------------------------------------------–>
\def\tkzInversePoint(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointIP in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointIP '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
    \tkz@@CalcLengthcm(#1,#2){tkz@lna}
    \tkz@@CalcLengthcm(#1,\PointIP){tkz@lnb}
    \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
    \tkzVecKNorm[\tkz@lnc](#1,\PointIP) 
    \pgfnodealias{\tkz@pointtsf}{tkzPointResult}
    }  
\endgroup
} 
\def\tkzUInversePoint(#1,#2)(#3){%  
\begingroup  
   \tkz@@CalcLengthcm(#1,#2){tkz@lna}% 
   \tkz@@CalcLengthcm(#1,#3){tkz@lnb}% 
   \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
   \tkzVecKNorm[\tkz@lnc](#1,#3) 
\endgroup
} 
% possible 
% \tkzDefLine[tangent from =#3](#1,#2) 
% \tkzTgtFromP(#1,#2)(#3) 
% \tkzInterLL(tkzFirstPointResult,tkzSecondPointResult)(#1,#2) 
%<--------------------------------------------------------------------------–>
%                   Inverse negative of a point 
%<--------------------------------------------------------------------------–>
\def\tkzInverseNegativePoint(#1,#2)(#3)#4{%
\begingroup 
\gdef\tkz@LastList{#4}
    \foreach\PointIP in {#3}{%
      \FirstPointInList\tkz@LastList
      \ifx\tkz@FirstPoint\tkzutil@empty  
         \xdef\tkz@pointtsf{\PointIP '}
      \else
         \xdef\tkz@pointtsf{\tkz@FirstPoint}
      \fi 
   \tkz@@CalcLengthcm(#1,#2){tkz@lna}
   \tkz@@CalcLengthcm(#1,\PointIP){tkz@lnb}
   \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
   \tkzVecKNorm[\tkz@lnc](#1,\PointIP) 
   \tkzUCSym(#1)(tkzPointResult)
   \pgfnodealias{\tkz@pointtsf}{tkzPointResult}
   }  
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzUInverseNegativePoint(#1,#2)(#3){%  
\begingroup  
   \tkz@@CalcLengthcm(#1,#2){tkz@lna}% 
   \tkz@@CalcLengthcm(#1,#3){tkz@lnb}% 
   \edef\tkz@lnc{\fpeval{\tkz@lna/\tkz@lnb*\tkz@lna}}
   \tkzVecKNorm[\tkz@lnc](#1,#3) 
   \tkzUCSym(#1)(tkzPointResult)
\endgroup
}
%<--------------------------------------------------------------------------–>
%<--------------- rotate with nodes                 ------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzRotateWithNodes(#1,#2,#3)(#4)#5{%
\begingroup
\gdef\tkz@LastList{#5}
 \foreach\PointRotWN in {#4}{%
   \FirstPointInList\tkz@LastList
   \ifx\tkz@FirstPoint\tkzutil@empty  
      \def\tkz@pointtsf{\PointRotWN '}
   \else
      \def\tkz@pointtsf{\tkz@FirstPoint}
   \fi 
   \tkzFindAngle(#2,#1,#3)
   \tkz@@extractxy{\PointRotWN}
   \tkz@ax\pgf@x%
   \tkz@ay\pgf@y%
   \tkz@@extractxy{#1}
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \pgfmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                        {\pgfpoint{\tkz@bx}{\tkz@by}}%
                        {\tkzAngleResult}
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \pgfinterruptboundingbox
   \path[coordinate](\tkz@bx,\tkz@by) coordinate (\tkz@pointtsf);% 
   \endpgfinterruptboundingbox
}   
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzURotateWithNodes(#1,#2,#3)(#4){%
\begingroup 
  \tkzFindAngle(#2,#1,#3)
  \pgf@process{\pgfpointanchor{#4}{center}}%
  \tkz@ax\pgf@x%
  \tkz@ay\pgf@y%
  \pgf@process{\pgfpointanchor{#1}{center}}%
  \tkz@bx\pgf@x%
  \tkz@by\pgf@y%
  \pgfmathrotatepointaround{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                           {\pgfpoint{\tkz@bx}{\tkz@by}}%
                           {\tkzAngleResult}
  \tkz@bx\pgf@x%
  \tkz@by\pgf@y%
  \pgfinterruptboundingbox
  \path (\tkz@bx,\tkz@by) coordinate (tkzPointResult);%
  \endpgfinterruptboundingbox  
\endgroup
}   
%<--------------------------------------------------------------------------–>
%                   Fin des transformations
%<--------------------------------------------------------------------------–>
\makeatother
\endinput

==> tikz-euclide/obj/tkz-obj-eu-points-rnd.tex <==
% tkz-obj-eu-points-rnd.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-points-rnd.tex} 
%<--------------------------------------------------------------------------–>
\makeatletter
%<-------------------------------------------------------------------------–>
%  Points aléatoires sur un segment, une droite, une demi-droite un cercle 
%<--------------------------------------------------------------------------–>
%                          les points aléatoires
%<--------------------------------------------------------------------------–>
\def\tkz@numrp{0}
\pgfkeys{/@tkzDefRandPoint/.cd,
      rectangle/.code args        = {#1 and #2}{\def\tkz@numrp{0}%
                                               \def\tkz@infl{#1}%
                                               \def\tkz@supr{#2}},
      segment/.code  args         = {#1--#2}{\def\tkz@numrp{1}%
                                             \def\tkz@start{#1}%
                                             \def\tkz@end{#2}}, 
      line/.code args             = {#1--#2}{\def\tkz@numrp{2}%
                                             \def\tkz@start{#1}%
                                             \def\tkz@end{#2}},  
      circle/.code args           = {center #1 radius #2}{\def\tkz@numrp{3}%
                                                          \def\tkz@center{#1}
                                                          \def\tkz@rad{#2}},
      circle through/.code args   = {center #1 through #2}{\def\tkz@numrp{4}%
                                                      \def\tkz@center{#1}
                                                      \def\tkz@point{#2}},
      disk through/.code args     = {center #1 through #2}{\def\tkz@numrp{5}%
                                                      \def\tkz@center{#1}
                                                      \def\tkz@point{#2}},
}
%<------------------------ version 2019 ---------------------------------->
\def\tkzDefRandPointOn{\pgfutil@ifnextchar[{\tkz@DefRandPointOn}{%
           \tkz@DefRandPointOn[]}}
\def\tkz@DefRandPointOn[#1]{%
\begingroup 
\pgfqkeys{/@tkzDefRandPoint}{#1}
\ifcase\tkz@numrp%
 % first case 0
   \tkzRandPointOnRect(\tkz@infl,\tkz@supr)
  \or% 1
   \tkzRandPointOnSegment(\tkz@start,\tkz@end)
  \or% 2
   \tkzRandPointOnLine(\tkz@start,\tkz@end)
  \or% 3
   \tkzRandPointOnCircle(\tkz@center,\tkz@rad)
  \or% 4
   \tkzRandPointOnCircleThrough(\tkz@center,\tkz@point)
   \or% 5
  \tkzRandPointOnDisk(\tkz@center,\tkz@point)
\fi
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzRandPointOnRect(#1,#2){% 
\tkz@@extractxy{#1}
 \pgf@xa=\pgf@x\relax%
 \pgf@ya=\pgf@y\relax%   
 \tkz@@extractxy{#2}
 \pgf@xb=\pgf@x\relax%
 \pgf@yb=\pgf@y\relax%  
 \edef\tkz@a{\fpeval{\pgf@xb-\pgf@xa}}
 \edef\tkz@b{\fpeval{\pgf@yb-\pgf@ya}}      
 \pgfmathparse{rnd}\global\let\tkzrndone\pgfmathresult 
 \pgfmathparse{rnd}\global\let\tkzrndtwo\pgfmathresult  
 \path[coordinate] ($(#1)+(\tkzrndone*\tkz@a pt,\tkzrndtwo*\tkz@b pt)$) coordinate (tkzPointResult);
   } 
%<--------------------------------------------------------------------------–>
\def\tkzRandPointOnSegment(#1,#2){% 
  \pgfmathparse{rnd}
  \let\myrnd\pgfmathresult 
\path[coordinate]  ($ (#1)!\myrnd!(#2) $) coordinate (tkzPointResult);
} 
%<--------------------------------------------------------------------------–>
\def\tkzRandPointOnLine(#1,#2){% 
  \pgfmathparse{rand}
  \let\myrnd\pgfmathresult 
\path[coordinate]  ($ (#1)!\myrnd!(#2) $) coordinate (tkzPointResult);
}
%<--------------------------------------------------------------------------–>
\def\tkzRandPointOnCircle(#1,#2){% 
\pgfmathrandominteger{\tkzrnd}{0}{360}
\tkz@ax#2cm %
  \edef\tkz@pxa{\fpeval{\tkz@ax*cosd(\tkzrnd)}}
  \edef\tkz@pxb{\fpeval{\tkz@ax*sind(\tkzrnd)}}      
  \path[coordinate]($(#1) + (\tkz@pxa pt,\tkz@pxb pt) $) coordinate (tkzPointResult);
}
\def\tkzRandPointOnCircleThrough(#1,#2){% 
\pgfmathrandominteger{\tkzrnd}{0}{360}
\tkz@@CalcLength(#1,#2){tkzLengthResult}
  \edef\tkz@pxa{\fpeval{\tkzLengthResult*cosd(\tkzrnd)}}
  \edef\tkz@pxb{\fpeval{\tkzLengthResult*sind(\tkzrnd)}} 
\path[coordinate]($(#1) + (\tkz@pxa pt ,\tkz@pxb pt) $) coordinate (tkzPointResult);
}
%<--------------------------------------------------------------------------–>
\def\tkzRandPointOnDisk(#1,#2){% 
  \pgfmathrandominteger{\tkzrnd}{0}{360}
  \tkz@@CalcLength(#1,#2){tkzLengthResult}
  \edef\tkz@pxa{\fpeval{\tkzLengthResult*cosd(\tkzrnd)}}
  \edef\tkz@pxb{\fpeval{\tkzLengthResult*sind(\tkzrnd)}}  
  \path[coordinate]($(#1) + (\tkz@pxa pt ,\tkz@pxb pt) $) coordinate (tkz@tmp);
  \pgfmathparse{rnd}
  \let\myrnd\pgfmathresult 
  \path[coordinate]  ($ (#1)!\myrnd!(tkz@tmp) $) coordinate (tkzPointResult);
}
\makeatother  
\endinput

==> tikz-euclide/obj/tkz-obj-eu-points-spc.tex <==
% tkz-obj-eu-points.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-el-points.tex} 
\makeatletter  
%add ExCenter
%<--------------------------------------------------------------------------–>
%                   Specific points
%<--------------------------------------------------------------------------–>
%                              barycentre
%<--------------------------------------------------------------------------–>
\def\tkzDefBarycentricPoint(#1){%
\begingroup
 \path[coordinate]  (barycentric cs:#1) coordinate (tkzPointResult); 
\endgroup
}
\let\tkzDefBCPoint\tkzDefBarycentricPoint

%<--------------------------------------------------------------------------–>
%                      milieu  de deux points
%<--------------------------------------------------------------------------–>
% possible   \coordinate (#3) at ($(#1)!0.5!(#2)$);
%<--------------------------------------------------------------------------–>
% \def\tkzDefMidPoint(#1,#2){%
% \begingroup
%  \path (#1) -- (#2) coordinate[pos=.5](tkzPointResult);
% \endgroup
% }
\def\tkzDefMidPoint(#1,#2){%
\begingroup
   \pgf@process{\pgfpointanchor{#1}{center}}%
   \tkz@ax\pgf@x%
   \tkz@ay\pgf@y%
   \pgf@process{\pgfpointanchor{#2}{center}}%
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \advance\tkz@bx by\tkz@ax\relax%
   \advance\tkz@by by\tkz@ay\relax%
   \divide\tkz@bx by2\relax%
   \divide\tkz@by by2\relax
   \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkz@bx}{\tkz@by}}
\endgroup
}
\def\tkz@DefMidPoint(#1,#2,#3,#4){%
\begingroup
   \tkz@ax#1%
   \tkz@ay#2%
   \tkz@bx#3%
   \tkz@by#4%
   \advance\tkz@bx by\tkz@ax\relax%
   \advance\tkz@by by\tkz@ay\relax%
   \divide\tkz@bx by2\relax%
   \divide\tkz@by by2\relax
   \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkz@bx}{\tkz@by}}
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkz@simicenter{0}
\pgfkeys{/tkzsimicenter/.cd,
      ext/.code       = \def\tkz@simicenter{0},
      int/.code       = \def\tkz@simicenter{1},
      ext
}%

\def\tkzDefSimilitudeCenter{\pgfutil@ifnextchar[{\tkz@DefSimilitudeCenter}%
                                              {\tkz@DefSimilitudeCenter[]}}     
\def\tkz@DefSimilitudeCenter[#1](#2,#3)(#4,#5){%
\pgfqkeys{/tkzsimicenter}{#1} 
\begingroup  
\ifcase\tkz@simicenter%
  \tkzDefExtSimilitudeCenter[#1](#2,#3)(#4,#5)
  \or% 1 
  \tkzDefIntSimilitudeCenter[#1](#2,#3)(#4,#5) 
\fi
\endgroup
}
%<--------------------------------------------------------------------------–>
%                    Internal Similitude center
%  Two circles have two similitude centers namely the internal center of
%   similitude Si and the external similitude center Se.
%<--------------------------------------------------------------------------–>
\def\tkz@numhomo{0}
\pgfkeys{
/tkzSimilitudeCenter/.cd,
 node/.code          = \def\tkz@numhomo{0},
 R/.code             = \def\tkz@numhomo{1},
 node,
 /tkzSimilitudeCenter/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
 \pgfkeysalso{\searchname/.try=#1, /tikz/\searchname/.retry=#1}}
}
\def\tkzDefIntSimilitudeCenter{\pgfutil@ifnextchar[{\tkz@DefIntSimilitudeCenter}{\tkz@DefIntSimilitudeCenter[]}}
\def\tkz@DefIntSimilitudeCenter[#1](#2,#3)(#4,#5){%
\begingroup
\pgfqkeys{/tkzSimilitudeCenter}{#1}
\ifcase\tkz@numhomo%
    \tkz@@CalcLengthcm(#2,#3){tkz@rt}%
    \tkz@@CalcLengthcm(#4,#5){tkz@rf}%
  \or% 1
   \def\tkz@rt{#3}%
   \def\tkz@rf{#5}%
\fi
\pgfinterruptboundingbox 
  \path[coordinate](barycentric cs:#2=\tkz@rf,#4=\tkz@rt)coordinate (tkzPointResult);
  \endpgfinterruptboundingbox 
\endgroup
}
\let\tkzDefIntHomotheticCenter\tkzDefIntSimilitudeCenter
%<--------------------------------------------------------------------------–>
%                    External Similitude center
%<--------------------------------------------------------------------------–>
\def\tkzDefExtSimilitudeCenter{\pgfutil@ifnextchar[{\tkz@DefExtSimilitudeCenter}{\tkz@DefExtSimilitudeCenter[]}}

\def\tkz@DefExtSimilitudeCenter[#1](#2,#3)(#4,#5){%
\begingroup
\pgfqkeys{/tkzSimilitudeCenter}{#1}
\ifcase\tkz@numhomo%
 \tkz@@CalcLengthcm(#2,#3){tkz@rt}%
 \tkz@@CalcLengthcm(#4,#5){tkz@rf}%
  \or% 1
 \def\tkz@rt{#3}%
 \def\tkz@rf{#5}%
\fi
 \pgfinterruptboundingbox 
   \path[coordinate](barycentric cs:#2=-\tkz@rf,#4=\tkz@rt) coordinate(tkzPointResult);
   \endpgfinterruptboundingbox 
\endgroup
}

\let\tkzDefExtHomotheticCenter\tkzDefExtSimilitudeCenter
%<--------------------------------------------------------------------------–>
%        Harmonic Division
%<--------------------------------------------------------------------------–>
%  A , B , C ,D  CA/CB = DA/DB
%<--------------------------------------------------------------------------–>
\def\tkz@numdha{0}
\pgfkeys{/tkzharmonic/.cd,
      ext/.code       = \def\tkz@numdha{0},
      int/.code       = \def\tkz@numdha{1},
      both/.code      = \def\tkz@numdha{2},
      both,
}%

\def\tkzDivHarmonic{\pgfutil@ifnextchar[{\tkz@DivHarmonic}{\tkz@DivHarmonic[]}}     
\def\tkz@DivHarmonic[#1](#2){%
\begingroup 
\pgfqkeys{/tkzharmonic}{#1}  
  \ifcase\tkz@numdha%
   \tkzDefDivHarmonicExt(#2)
 \or%
    \tkzDefDivHarmonicInt(#2)
  \or%
    \tkzDefDivHarmonicBoth(#2)
 \fi
\endgroup
}

\def\tkzDefDivHarmonicExt(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
  \tkz@VecKOrth[](#1,#2)  \tkzGetPoint{tkz@px}
  \tkzDefMidPoint(tkz@px,#2)          \tkzGetPoint{tkz@py}
  \tkzInterLL(tkz@px,#3)(#1,tkz@py)   \tkzGetPoint{tkz@pz}
  \tkzInterLL(#2,tkz@pz)(#1,tkz@px)   \tkzGetPoint{tkz@px}
  \tkzInterLL(tkz@py,tkz@px)(#1,#2)   \tkzGetPoint{tkzPointResult}
\endpgfinterruptboundingbox 
\endgroup
}

\def\tkzDefDivHarmonicInt(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
  \tkz@VecKOrth[1](#1,#2)  \tkzGetPoint{tkz@px}
  \tkzDefMidPoint(tkz@px,#2)          \tkzGetPoint{tkz@py}
  \tkzInterLL(tkz@py,#3)(#1,tkz@px)   \tkzGetPoint{tkz@pz}
  \tkzInterLL(#2,tkz@pz)(#1,tkz@py)   \tkzGetPoint{tkz@py}
  \tkzInterLL(tkz@py,tkz@px)(#1,#2)   \tkzGetPoint{tkzPointResult}
\endpgfinterruptboundingbox 
\endgroup
}

\def\tkzDefDivHarmonicBoth(#1,#2,#3){%
\begingroup
\edef\tkz@k{\fpeval{#3}}
    \path[coordinate]  (barycentric cs:#1=1,#2={\tkz@k}) coordinate (tkzFirstPointResult);
    \path[coordinate]  (barycentric cs:#1=1,#2={-\tkz@k}) coordinate (tkzSecondPointResult);
\endgroup
}

\let\tkzDefHarmonic\tkzDivHarmonic
%<--------------------------------------------------------------------------–> 
%                   golden ratio
%<--------------------------------------------------------------------------–>
\def\tkzDefGoldenRatio(#1,#2){%
\begingroup
\tkzDefPointWith[linear,K=\tkzInvPhi](#1,#2)
\endgroup
}
%<--------------------------------------------------------------------------–> 
%                    triangle center
%<--------------------------------------------------------------------------–>

\def\tkz@numtc{0}
\pgfkeys{/tkzDefTriangleCenter/.cd,
   ortho/.code        = \def\tkz@numtc{0},
   orthic/.code       = \def\tkz@numtc{0},
   centroid/.code     = \def\tkz@numtc{1},
   median/.code       = \def\tkz@numtc{1},
   circum/.code       = \def\tkz@numtc{2},
   in/.code           = \def\tkz@numtc{3},
   ex/.code           = \def\tkz@numtc{4},
   euler/.code        = \def\tkz@numtc{5},
   symmedian/.code    = \def\tkz@numtc{6},
   lemoine/.code      = \def\tkz@numtc{6},
   grebe/.code        = \def\tkz@numtc{6},
   spieker/.code      = \def\tkz@numtc{7},
   gergonne/.code     = \def\tkz@numtc{8},
   nagel/.code        = \def\tkz@numtc{9}, 
   mittenpunkt/.code  = \def\tkz@numtc{10}, 
   feuerbach/.code    = \def\tkz@numtc{11},
   circum       
}     
\def\tkzDefTriangleCenter{\pgfutil@ifnextchar[{\tkz@DefTriangleCenter}{\tkz@DefTriangleCenter[]}}
\def\tkz@DefTriangleCenter[#1](#2){% 
\begingroup  
\pgfqkeys{/tkzDefTriangleCenter}{#1}  
\ifcase\tkz@numtc%
  \tkzOrthoCenter(#2)
  \or% 1 
  \tkzCentroid(#2)  
  \or% 2
  \tkzCircumCenter(#2) 
  \or% 3
  \tkzInCenter(#2) 
  \or% 4
  \tkzExCenter(#2) 
  \or% 5
  \tkzEulerCenter(#2)
  \or% 6
  \tkzSymmedianCenter(#2) 
  \or% 7
  \tkzSpiekerCenter(#2) 
  \or% 8
  \tkzGergonneCenter(#2) 
  \or%9
  \tkzNagelCenter(#2)
  \or%10
  \tkzMittenpunktCenter(#2) 
  \or%11
  \tkzFeuerbachCenter(#2) 
    \fi    
\endgroup
}
%<--------------------------------------------------------------------------–> 
%                    OrthoCenter
%<--------------------------------------------------------------------------–>
\def\tkzOrthoCenter(#1,#2,#3){%
\begingroup
  \pgfinterruptboundingbox 
   \tkzUProjection(#1,#2)(#3)
   \pgfnodealias{ort@pta}{tkzPointResult}
   \tkzUProjection(#1,#3)(#2)
   \pgfnodealias{ort@ptb}{tkzPointResult}
   \tkzInterLL(#2,ort@ptb)(#3,ort@pta)
   \endpgfinterruptboundingbox 
\endgroup
}
\let\tkzDefOrthoCenter\tkzOrthoCenter
%<--------------------------------------------------------------------------–>
%                      GravityCenter modif 3.03
%<--------------------------------------------------------------------------–>
\def\tkzCentroid(#1,#2,#3){%
\begingroup 
   \pgf@process{\pgfpointanchor{#1}{center}}%
   \tkz@ax\pgf@x%
   \tkz@ay\pgf@y%
   \pgf@process{\pgfpointanchor{#2}{center}}%
   \tkz@bx\pgf@x%
   \tkz@by\pgf@y%
   \pgf@process{\pgfpointanchor{#3}{center}}%
   \tkz@cx\pgf@x%
   \tkz@cy\pgf@y%
   \advance\tkz@cx by\tkz@ax\relax%
   \advance\tkz@cy by\tkz@ay\relax%
   \advance\tkz@cx by\tkz@bx\relax%
   \advance\tkz@cy by\tkz@by\relax%
   \divide\tkz@cx by3\relax%
   \divide\tkz@cy by3\relax
   \pgfinterruptboundingbox 
   \pgfcoordinate{tkzPointResult}{\pgfqpoint{\tkz@cx}{\tkz@cy}}
   \endpgfinterruptboundingbox   
\endgroup
}
\let\tkzBaryCenter\tkzCentroid

%<--------------------------------------------------------------------------–>
%                      CircumCenter
%<--------------------------------------------------------------------------–>
\def\tkzCircumCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
 \tkzDefMediatorLine(#1,#2)
 \pgf@process{\pgfpointanchor{tkzFirstPointResult}{center}}%
 \tkz@ax\pgf@x%
 \tkz@ay\pgf@y%
 \pgf@process{\pgfpointanchor{tkzSecondPointResult}{center}}%
 \tkz@bx\pgf@x%
 \tkz@by\pgf@y%
 \tkzDefMediatorLine(#1,#3)
 \pgf@process{\pgfpointanchor{tkzFirstPointResult}{center}}%
 \tkz@cx\pgf@x%
 \tkz@cy\pgf@y%
 \pgf@process{\pgfpointanchor{tkzSecondPointResult}{center}}%
 \tkz@dx\pgf@x%
 \tkz@dy\pgf@y%
\tkzInterLLxy(\tkz@ax,\tkz@ay,\tkz@bx,\tkz@by)(\tkz@cx,\tkz@cy,\tkz@dx,\tkz@dy)%
\endpgfinterruptboundingbox
\endgroup
} 
\let\tkzDefCircumCenter\tkzCircumCenter
%<--------------------------------------------------------------------------–>
%                     InCenter
%<--------------------------------------------------------------------------–>
\def\tkzInCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
\tkzDefBisectorLine(#3,#1,#2)
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\tkzDefBisectorLine(#3,#2,#1) 
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@dx\pgf@x%
\tkz@dy\pgf@y%
\pgf@process{\pgfpointanchor{#1}{center}}%
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgf@process{\pgfpointanchor{#2}{center}}%
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\tkzInterLLxy(\tkz@ax,\tkz@ay,\tkz@bx,\tkz@by)(\tkz@cx,\tkz@cy,\tkz@dx,\tkz@dy)%
\endpgfinterruptboundingbox
\endgroup
} 
\let\tkzDefInCenter\tkzInCenter
%<--------------------------------------------------------------------------–>
%                     ExCenter
%<--------------------------------------------------------------------------–>
\def\tkzExCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox 
\tkzDefBisectorOutLine(#2,#1,#3)
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\tkzDefBisectorOutLine(#2,#3,#1) 
\pgf@process{\pgfpointanchor{tkzPointResult}{center}}%
\tkz@dx\pgf@x%
\tkz@dy\pgf@y%
\pgf@process{\pgfpointanchor{#1}{center}}%
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgf@process{\pgfpointanchor{#3}{center}}%
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\tkzInterLLxy(\tkz@ax,\tkz@ay,\tkz@bx,\tkz@by)(\tkz@cx,\tkz@cy,\tkz@dx,\tkz@dy)%
\endpgfinterruptboundingbox
\endgroup
} 
\let\tkzDefExCenter\tkzExCenter
%<--------------------------------------------------------------------------–>
%                     EulerCenter neuf points
%<--------------------------------------------------------------------------–>
\def\tkzEulerCenter(#1,#2,#3){% 
% mileu de orthocentre et centre cercle circonscrit
% passe par les midpoints par les pieds des hauteurs
\begingroup
\pgfinterruptboundingbox 
\tkzDefMidPoint(#1,#2)
\pgfnodealias{eu@mic}{tkzPointResult}
\tkzDefMidPoint(#1,#3)
\pgfnodealias{eu@mib}{tkzPointResult}
\tkzDefMidPoint(#2,#3)
\pgfnodealias{eu@mia}{tkzPointResult}
\tkzCircumCenter(eu@mia,eu@mib,eu@mic)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzNinePointCenter\tkzEulerCenter
\let\tkzDefEulerCenter\tkzEulerCenter
%<--------------------------------------------------------------------------–>
%Symmedian center Lemoine point Grebe point K
%<--------------------------------------------------------------------------–>
\def\tkzSymmedianCenter(#1,#2,#3){%
\begingroup
\pgfinterruptboundingbox    
\tkzDefMidPoint(#2,#3)
\pgfnodealias{eu@mic}{tkzPointResult}
\tkzDefMidPoint(#1,#3)
\pgfnodealias{eu@mib}{tkzPointResult}
\tkzUProjection(#2,#3)(#1)
\pgfnodealias{ort@pta}{tkzPointResult}
\tkzDefMidPoint(#1,ort@pta)
\pgfnodealias{eu@mid}{tkzPointResult}
\tkzUProjection(#1,#3)(#2)
\pgfnodealias{ort@ptb}{tkzPointResult}
\tkzDefMidPoint(#2,ort@ptb)
\pgfnodealias{eu@mie}{tkzPointResult}
\tkzInterLL(eu@mic,eu@mid)(eu@mib,eu@mie)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzLemoinePoint\tkzSymmedianCenter
\let\tkzGrebePoint\tkzSymmedianCenter
\let\tkzDefLemoinePoint\tkzLemoinePoint
%<--------------------------------------------------------------------------–> 
%                   Spieker center
%<--------------------------------------------------------------------------–>
\def\tkzSpiekerCenter(#1,#2,#3){%
\begingroup
% we need to get the midpoints
\pgfcoordinate{tkz@m3}{%
  \pgfpointscale{0.5}{%
  \pgfpointadd{\pgfpointanchor{#1}{center}}%
              {\pgfpointanchor{#2}{center}}}}%
\pgfcoordinate{tkz@m2}{%
  \pgfpointscale{0.5}{%
  \pgfpointadd{\pgfpointanchor{#1}{center}}%
              {\pgfpointanchor{#3}{center}}}}%
\pgfcoordinate{tkz@m1}{%
   \pgfpointscale{0.5}{%
   \pgfpointadd{\pgfpointanchor{#2}{center}}%
               {\pgfpointanchor{#3}{center}}}}%
\tkzInCenter(tkz@m1,tkz@m2,tkz@m3)
\endgroup
} 
\let\tkzDefSpiekerCenter\tkzSpiekerCenter 
%<--------------------------------------------------------------------------–> 
%                    Gergonne center Ge
%<--------------------------------------------------------------------------–>
\def\tkzGergonneCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzInCenter(#1,#2,#3)
\pgfnodealias{tkz@ptin}{tkzPointResult}
\tkzUProjection(#2,#3)(tkz@ptin)
\pgfnodealias{tkz@oca}{tkzPointResult}
\tkzUProjection(#1,#3)(tkz@ptin)
\pgfnodealias{tkz@ocb}{tkzPointResult}
\tkzInterLL(#1,tkz@oca)(#2,tkz@ocb)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzDefGergonneCenter\tkzGergonneCenter 
%<--------------------------------------------------------------------------–> 
%                    Nagel center Na
%<--------------------------------------------------------------------------–>
%  INa = 3 IG. Nagel point % correction 02/02/20
\def\tkzNagelCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzDefExcentralTriangle(#1,#2,#3){tkz@a,tkz@b,tkz@c}
\tkzUProjection(#2,#3)(tkz@a)
\pgfnodealias{tkz@tgta}{tkzPointResult}
\tkzUProjection(#1,#2)(tkz@c)
\pgfnodealias{tkz@tgtc}{tkzPointResult}
\tkzInterLL(#1,tkz@tgta)(#3,tkz@tgtc)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzDefNagelCenter\tkzNagelCenter 
%<--------------------------------------------------------------------------–>
%  Mittenpunkt
%<--------------------------------------------------------------------------–>
\def\tkzMittenpunktCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzExCenter(#2,#3,#1)
\pgfnodealias{tkz@a}{tkzPointResult}
\tkzExCenter(#3,#1,#2)
\pgfnodealias{tkz@b}{tkzPointResult}
\pgfcoordinate{tkz@ma}{%
\pgfpointscale{0.5}{%
\pgfpointadd{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}}}%
\pgfcoordinate{tkz@mb}{%
\pgfpointscale{0.5}{%
\pgfpointadd{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}}}%
\tkzInterLL(tkz@a,tkz@ma)(tkz@b,tkz@mb)
\endpgfinterruptboundingbox
\endgroup
}
\let\tkzDefMittenpunktCenter\tkzMittenpunktCenter 
\let\tkzDefMiddlespoint\tkzMittenpunktCenter     
%<--------------------------------------------------------------------------–> 
%                   Feuerbach point
%<--------------------------------------------------------------------------–>
\def\tkzFeuerbachCenter(#1,#2,#3){%  
\begingroup
\pgfinterruptboundingbox 
\tkzEulerCenter(#1,#2,#3)
\pgfnodealias{tkz@euler}{tkzPointResult}
\tkzInCenter(#1,#2,#3) 
\pgfnodealias{tkz@in}{tkzPointResult}
\tkzUProjection(#2,#3)(tkzPointResult)
\tkzInterLC(tkz@in,tkz@euler)(tkz@in,tkzPointResult)\tkzGetFirstPoint{tkz@fe}
\tkzRenamePoint(tkz@fe){tkzPointResult}
\endpgfinterruptboundingbox  
\endgroup
}
\let\tkzDefFeuerbachCenter\tkzFeuerbachCenter 
%<--------------------------------------------------------------------------–>
%                     Orthogonal center
%<--------------------------------------------------------------------------–>
\def\tkzOrthogonalCenter(#1,#2){%
\begingroup
\pgfinterruptboundingbox 
\tkz@VecK[\tkz@koeff/(1+\tkz@koeff)](#1,#2)
\pgfnodealias{tkzFirstPointResult}{tkzPointResult}
\tkz@VecK[\tkz@koeff/(\tkz@koeff-1)](#1,#2)
\pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\tkzDefMidPoint(tkzFirstPointResult,tkzSecondPointResult) 
\endpgfinterruptboundingbox 
\endgroup
}
%<--------------------------------------------------------------------------–>
%                  End Triangle center
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                  Projection  center of excircles
%<--------------------------------------------------------------------------–>
\def\tkzDefProjExcenter{\pgfutil@ifnextchar[{%
    \tkz@DefProjExcenter}{%
    \tkz@DefProjExcenter[]}
    }
\def\tkz@DefProjExcenter[#1](#2,#3,#4)(#5)#6{
\begingroup  
  \SetUpPTTR{#1}
   \foreach \name  [count=\i] in {#5} {%
      \global\expandafter\edef\csname tkz@pt\i\endcsname{\name}
        }
   \foreach \name  [count=\i] in {#6} {%
      \global\expandafter\edef\csname tkz@ppt\i\endcsname{\name}
        }
\tkzDefPointBy[projection=onto #3--#4 ](\tkz@pttr@name \csname tkz@pt1\endcsname) 
\pgfnodealias{\csname tkz@ppt1\endcsname\csname tkz@pt1\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#4 ](\tkz@pttr@name \csname tkz@pt2\endcsname) 
\pgfnodealias{\csname tkz@ppt1\endcsname\csname tkz@pt2\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#4 ](\tkz@pttr@name \csname tkz@pt3\endcsname) 
\pgfnodealias{\csname tkz@ppt1\endcsname\csname tkz@pt3\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #2--#4 ](\tkz@pttr@name \csname tkz@pt1\endcsname) 
\pgfnodealias{\csname tkz@ppt2\endcsname\csname tkz@pt1\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #2--#4 ](\tkz@pttr@name \csname tkz@pt2\endcsname) 
\pgfnodealias{\csname tkz@ppt2\endcsname\csname tkz@pt2\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #2--#4 ](\tkz@pttr@name \csname tkz@pt3\endcsname) 
\pgfnodealias{\csname tkz@ppt2\endcsname\csname tkz@pt3\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#2 ](\tkz@pttr@name \csname tkz@pt1\endcsname) 
\pgfnodealias{\csname tkz@ppt3\endcsname\csname tkz@pt1\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#2 ](\tkz@pttr@name \csname tkz@pt2\endcsname) 
\pgfnodealias{\csname tkz@ppt3\endcsname\csname tkz@pt2\endcsname}{tkzPointResult}
\tkzDefPointBy[projection=onto #3--#2 ](\tkz@pttr@name \csname tkz@pt3\endcsname) 
\pgfnodealias{\csname tkz@ppt3\endcsname\csname tkz@pt3\endcsname}{tkzPointResult}
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%              Point on circle
%<--------------------------------------------------------------------------–>
\def\tkz@numptcirc{0}
\pgfkeys{/tkzptcircle/.cd,
through/.code  args = {center #1 angle #2 point #3}        { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@through{#3}%
                                                             \def\tkz@numptcirc{0}},
R/.code args = {center #1 angle #2 radius #3}              { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@radius{#3}%
                                                             \def\tkz@numptcirc{1}},
through in rad/.code  args = {center #1 angle #2 point #3} { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@through{#3}%
                                                             \def\tkz@numptcirc{2}},
R in rad/.code args = {center #1 angle #2 radius #3}       { \def\tkz@center{#1}%
                                                             \def\tkz@angle{#2}%
                                                             \def\tkz@radius{#3}%
                                                             \def\tkz@numptcirc{3}}                                                 
}
                                                  
\def\tkzDefPointOnCircle{\pgfutil@ifnextchar[{\tkz@DefPointOnCircle}{%
                                              \tkz@DefPointOnCircle[]}}     
\def\tkz@DefPointOnCircle[#1]{%
\begingroup 
\pgfqkeys{/tkzptcircle}{#1}
 \ifcase\tkz@numptcirc%
    \tkz@@CalcLengthcm(\tkz@center,\tkz@through){tkz@radius}
     \or% 1
    \relax%
    \or% 2
    \pgfmathparse{\tkz@angle\space r}
    \let\tkz@angle\pgfmathresult
    \tkz@@CalcLengthcm(\tkz@center,\tkz@through){tkz@radius}
    \or% 3
    \pgfmathparse{\tkz@angle\space r}
    \let\tkz@angle\pgfmathresult
\fi
\path (\tkz@center) --++(\tkz@angle:\tkz@radius) coordinate(tkzPointResult);
\endgroup
} 
%<--------------------------------------------------------------------------–>
%              Point on line
%<--------------------------------------------------------------------------–>
\def\tkzDefPointOnLine{\pgfutil@ifnextchar[{\tkz@DefPointOnLine}{\tkz@DefPointOnLine[]}}     
\def\tkz@DefPointOnLine[#1](#2,#3){%
\begingroup 
\path (#2) to [#1] coordinate (tkzPointResult)  (#3);
\endgroup
} 

\makeatother  
\endinput

==> tikz-euclide/obj/tkz-obj-eu-points-with.tex <==
% tkz-obj-el-points-with.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-points-with.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%                          Vectors
%<--------------------------------------------------------------------------–>
% Objet :  outils mathématiques pour la géométrie euclideienne avec pgf/tikz
% utilisable de préférence avec un repère orthonormé et le cm comme unité 
% utile pour la compatibilité avec pgf 2
%<--------------------------------------------------------------------------–>
%             Duplicate Length      à revoir pas de pt pas de global
% ||v(CN)||= ||v(AB)|| et v(CN) colineaire à v(CD) 
% A-->#1 B-->#2 C-->#3 D-->#4 N-->#5   ?????
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                 Outils pour les vecteurs
%<--------------------------------------------------------------------------–>
%  ce sont des outils élémentaires qui à partir de deux points en définissent 
% un troisième 
% #1 si c'est une option alors c'est un nombre réel
% #2 et #3 sont deux points
% #4 est le nom du point qui résulte de la transformation
% exemple : \tkzVecKNorm (A,B){C} définit un point C tel que AC = 1 et C est %  %  un point de la droite (AC). #1 peut être négatif

\def\tkzDuplicateSegment(#1,#2)(#3,#4){%
\begingroup 
    \tkz@@CalcLength(#1,#2){tkz@firstlen}% 
    \tkz@@CalcLength(#3,#4){tkz@secondlen}%
   \edef\tkz@ratio{\fpeval{\tkz@firstlen/\tkz@secondlen}}
    \tkz@VecKCoLinear[\tkz@ratio](#3,#4,#3)%
\endgroup 
}
\let\tkzDuplicateLength\tkzDuplicateSegment     
%<--------------------------------------------------------------------------–>
%                    Coordonnées d'un vecteur  (couple de points)  
% Deux points A et B donc un vecteur on récupère les coordonnées de v(AB)
% en cm 
% tkzGetVecCoord en cm ou en pt ???
%<--------------------------------------------------------------------------–>
%result in #3x et #3y #1 et #2 sont les points  
% passage en cm avec fp ? 
% 28.45274 =1 cm
\def\tkzGetVectxy(#1,#2)#3{%
\begingroup 
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\pgfmathparse{\pgf@sys@tonumber{\pgf@x}/1cm}%
\let\tkzresultx\pgfmathresult
\pgfmathparse{\pgf@sys@tonumber{\pgf@y}/1cm}%
\let\tkzresulty\pgfmathresult
\global\expandafter\edef\csname #3x\endcsname{\tkzresultx}% 
\global\expandafter\edef\csname #3y\endcsname{\tkzresulty}% 
\endgroup
}
%<--------------------------------------------------------------------------–>
% options #1 two points #2,#3 result in #4
%
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%          tkzDefPointWith  
%<--------------------------------------------------------------------------–>
\def\tkz@numv{0}
\pgfkeys{/@pointwith/.cd,
      colinear/.code     args     = {at #1}{\def\tkz@numv{0}\def\tkz@frompoint{#1}},
      orthogonal/.code            = {\def\tkz@numv{1}},
      linear/.code                = {\def\tkz@numv{2}},
      orthogonal normed/.code     = {\def\tkz@numv{3}},
      linear normed/.code         = {\def\tkz@numv{4}},
      colinear normed/.code  args = {at #1}{\def\tkz@numv{5}\def\tkz@frompoint{#1}},
      K/.code                     = {\edef\tkz@coeff{\fpeval{#1}}},
      K                           = 1,
      normed/.is if               =  tkz@line@normed,
      normed/.default             =  true,
      normed                      =  false,
      orthogonal  
} 
\def\tkzDefPointWith{\pgfutil@ifnextchar[{\tkz@DefPointWith}{\tkz@DefPointWith[]}}  

\def\tkz@DefPointWith[#1](#2,#3){%
\begingroup 
\pgfkeys{/@pointwith/.cd,K=1}  
\pgfqkeys{/@pointwith}{#1}
\ifcase\tkz@numv%
 % first case 0
   \tkz@DefVectorColinearat[\tkz@coeff](#2,#3)
  \or% 1
   \tkz@VecKOrth[\tkz@coeff](#2,#3)
  \or% 2
   \tkz@VecK[\tkz@coeff](#2,#3)
  \or% 3
   \tkz@VecKOrthNorm[\tkz@coeff](#2,#3)
  \or% 4
   \tkz@VecKNorm[\tkz@coeff](#2,#3)
  \or% 5
   \tkz@VecKColinearNorm[\tkz@coeff](#2,#3)
  \fi    
\endgroup
} 
%<--------------------------------------------------------------------------–>
%         tkzDefVectorfrom  
%<--------------------------------------------------------------------------–>
% tkz@numv 0
\def\tkz@DefVectorColinearat[#1](#2,#3){%
\iftkz@line@normed
   \tkz@VecKColinearNorm[#1](#2,#3)
\else
\begingroup
  \pgfpointdiff{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}%
  \pgf@xa=\pgf@x\relax%
  \pgf@ya=\pgf@y\relax%
  \pgfinterruptboundingbox
  \path (\tkz@frompoint)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya) coordinate (tkzPointResult);
  \endpgfinterruptboundingbox
\endgroup
\fi
} 
%<--------------------------------------------------------------------------–>
%     tkzVector K Orth   coeff dans #1
%     v(AN) perp v(AB)  (v(AB) , v(AN) ) sens direct cercle trigo 
%     ||v(AN)||=||v(AB)||
%<--------------------------------------------------------------------------–>
% tkz@numv 1
\def\tkzVecKOrth{\pgfutil@ifnextchar[{\tkz@VecKOrth}{\tkz@VecKOrth[1]}}  
\def\tkz@VecKOrth[#1](#2,#3){%
\iftkz@line@normed
   \tkz@VecKOrthNorm[#1](#2,#3)
\else
\begingroup
  \pgfpointdiff{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}%
  \pgf@xa=-\pgf@y%
  \pgf@ya=\pgf@x%
  \pgfinterruptboundingbox 
  \path (#2)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya) coordinate (tkzPointResult);
  \endpgfinterruptboundingbox
\endgroup
\fi
}%

%<--------------------------------------------------------------------------–>
%         v(AN)=#1 x v(AB)     
%   #1 le coeff; #2--> A #3--> B   #4-->N  tq    #4-#2 = #1*(#3-#2)                                 
%<--------------------------------------------------------------------------–>
% tkz@numv 2
\def\tkzVecK{\pgfutil@ifnextchar[{\tkz@VecK}{\tkz@VecK[1]}} 
\def\tkz@VecK[#1](#2,#3){% 
\iftkz@line@normed
   \tkz@VecKNorm[#1](#2,#3)
\else
\begingroup 
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x\relax%
   \pgf@ya=\pgf@y\relax%
   \pgfmathparse{#1}
   \let\tkz@coeff\pgfmathresult
      \pgfinterruptboundingbox 
   \path (#2)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya) coordinate (tkzPointResult);
    \endpgfinterruptboundingbox   
\endgroup
\fi
}% 
%<--------------------------------------------------------------------------–>
%              tkzVecKOrthNorm   coeff dans #1
%    v(AN) perp v(AB)  v(AB) v(AN) sens direct cercle trigo 
% ||v(AN||=1 si #1 est vide ou =1 sinon ||v(AN||=K
%<--------------------------------------------------------------------------–>
% tkz@numv 3
\def\tkzVecKOrthNorm{\pgfutil@ifnextchar[{\tkz@VecKOrthNorm}%
                                         {\tkz@VecKOrthNorm[1]}}
\def\tkz@VecKOrthNorm[#1](#2,#3){%    
\begingroup
 \tkzpointnormalised{\pgfpointdiff{\pgfpointanchor{#2}{center}}%
                                  {\pgfpointanchor{#3}{center}}} 
  \pgf@xa=-\pgf@y\relax%
  \pgf@ya=\pgf@x\relax%
  \edef\tkz@x{\fpeval{28.45274*(#1)*\pgf@xa}}
  \edef\tkz@y{\fpeval{28.45274*(#1)*\pgf@ya}}
  \pgfinterruptboundingbox 
  \path (#2)--++(\tkz@x pt,\tkz@y pt) coordinate (tkzPointResult);
  \endpgfinterruptboundingbox   
\endgroup
}%      
%<--------------------------------------------------------------------------–>
%              VectorNormalised ou K*VectorNormalised
% A-->#2 B-->#3 N-->#4      v(AB)  devient v(AN) tq ||v(AN)||=1 si #1=1  
%  sinon ||v(AN)||=#1 
%<--------------------------------------------------------------------------–>
% tkz@numv 4
\def\tkzVecKNorm{\pgfutil@ifnextchar[{\tkz@VecKNorm}{\tkz@VecKNorm[1]}} 
\def\tkz@VecKNorm[#1](#2,#3){%
\begingroup
    \tkzpointnormalised{%
    \pgfpointdiff{\pgfpointanchor{#2}{center}}
                 {\pgfpointanchor{#3}{center}}}
    \pgf@xa=\pgf@x\relax%
    \pgf@ya=\pgf@y\relax% 
    \edef\tkz@x{\fpeval{28.45274*(#1)*\pgf@xa}}
    \edef\tkz@y{\fpeval{28.45274*(#1)*\pgf@ya}}
    \pgfinterruptboundingbox 
    \path (#2)--++(\tkz@x pt,\tkz@y pt) coordinate (tkzPointResult);
    \endpgfinterruptboundingbox   
\endgroup
}%
%<--------------------------------------------------------------------------–>
%            \tkz@VecKColinearNorm
%<--------------------------------------------------------------------------–>
%% tkz@numv 5
\def\tkz@VecKColinearNorm[#1](#2,#3){%
\begingroup   
    \tkzpointnormalised{%
    \pgfpointdiff{\pgfpointanchor{#2}{center}}
                 {\pgfpointanchor{#3}{center}}}
    \pgf@xa=\pgf@x\relax%
    \pgf@ya=\pgf@y\relax% 
    \edef\tkz@x{\fpeval{28.45274*(#1)*\pgf@xa}}
    \edef\tkz@y{\fpeval{28.45274*(#1)*\pgf@ya}}
    \pgfinterruptboundingbox
    \path (\tkz@frompoint)--++(\tkz@x pt,\tkz@y pt) coordinate (tkzPointResult);
    \endpgfinterruptboundingbox
\endgroup
}%
%<--------------------------------------------------------------------------–>
%  VecKCoLinear  CN = K x AB  #1 pt #2 pt #3 pt #4 nb #5 pt result   
% il faut modifier cette macro : on supprime #3 pour la colinéarité
% Il suffit d'utiliser Replicate ou Duplicate     coeff dans #1
% v(CD)=#1 x v(AB) #1 le coeff; #2-->A #3-->B #4-->C 
%<--------------------------------------------------------------------------–>
\def\tkz@VecKCoLinear[#1](#2,#3,#4){% 
\begingroup
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x\relax%
   \pgf@ya=\pgf@y\relax% 
   \edef\tkz@coeff{\fpeval{#1}}
   \pgfinterruptboundingbox 
   \path (#4)--+(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)  coordinate (tkzPointResult);
   \endpgfinterruptboundingbox                     
\endgroup
}%  
\def\tkz@VecCoLinear(#1,#2,#3){% 
\begingroup
   \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                {\pgfpointanchor{#2}{center}}%
   \pgf@xa=\pgf@x\relax%
   \pgf@ya=\pgf@y\relax% 
   \pgfinterruptboundingbox 
   \path (#3)--+(\pgf@xa,\pgf@ya)  coordinate (tkzPointResult);
   \endpgfinterruptboundingbox                     
\endgroup
}% 
\makeatother
\endinput

==> tikz-euclide/obj/tkz-obj-eu-points.tex <==
 % tkz-obj-eu-points.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c  tkz-obj-eu-points.tex} 
\makeatletter
%<--------------------------------------------------------------------------->
%                             init def point 
%<--------------------------------------------------------------------------->
%                            tkzDefPoint
%<--------------------------------------------------------------------------->
%                     macros complémentaires  pour def point
%<--------------------------------------------------------------------------->
\def\tkz@parsecoordinate#1{%
\tkz@getseparator#1,\@nil
\iftkz@polar 
   \tkz@getfrompolar#1\@nil
\else
   \tkz@getfromcart#1\@nil
\fi
}
\def\tkz@getseparator#1,#2\@nil{%
\ifx\tkzempty#2\tkzempty%
   \tkz@polartrue
\else
   \tkz@polarfalse
\fi
}      
\def\tkz@getfrompolar#1:#2\@nil{%
\edef\tkz@a{\fpeval{#1}}
\edef\tkz@r{\fpeval{#2}}
\xdef\tkz@polarrad{\tkz@r}
\xdef\tkz@polarangle{\tkz@a}
} 
\def\tkz@getfromcart#1,#2\@nil{%
\edef\tkz@x{\fpeval{#1}}
\edef\tkz@y{\fpeval{#2}}
\xdef\tkz@absc{\tkz@x}
\xdef\tkz@ord{\tkz@y}
}
%<--------------------------------------------------------------------------->
%           options pour point definition
%<--------------------------------------------------------------------------->
\pgfkeys{/tkzPt/.cd,  
         polar/.is if       = tkz@pt@polar,
         polar/.default     = true,
         polar              = false  
}
%<--------------------------------------------------------------------------->
%        tkz@ptStar  
%<--------------------------------------------------------------------------->
\def\tkz@ptStar[#1](#2,#3)#{%
\pgfkeys{/tkzPt/.cd, polar     = false} 
\pgfqkeys{/tkzPt}{#1}  
\iftkz@pt@polar%
  \edef\tkz@x{\fpeval{#3*cosd(#2)}}
  \edef\tkz@y{\fpeval{#3*sind(#2)}}
\else
  \edef\tkz@x{\fpeval{#2}}
  \edef\tkz@y{\fpeval{#3}}
\fi
\edef\tkzpt@xa{\fpeval{(\tkz@x-\tkz@init@xorigine)/\tkz@init@xstep}}
\edef\tkzpt@ya{\fpeval{(\tkz@y-\tkz@init@yorigine)/\tkz@init@ystep}}
\tkz@node
}
%<--------------------------------------------------------------------------->
% la macro defpoint les coordonnées cartésiennes ou polaires sont  traitées
% afin de pouvoir être adaptées avec les unités choisies
%<--------------------------------------------------------------------------->
\def\tkzDefPoint{\pgfutil@ifnextchar[{\tkz@DefPoint}{\tkz@DefPoint[]}}

\def\tkz@DefPoint[#1](#2)#{% 
\tkz@parsecoordinate{#2}
\iftkz@polar
   \tkz@ptStar[polar](\tkz@polarangle,\tkz@polarrad){tkz@coord@temp}
\else  
    \tkz@ptStar[](#2){tkz@coord@temp}
\fi
\tkz@DefPointEnd[#1]
}% 
\def\tkz@DefPointEnd[#1]#2{\coordinate[#1] (#2) at (tkz@coord@temp);}
%<--------------------------------------------------------------------------->
%                            tkzDefPoints
%<--------------------------------------------------------------------------->
\def\tkzDefPoints{\pgfutil@ifnextchar[{\tkz@DefPoints}{\tkz@DefPoints[]}}
\def\tkz@DefPoints[#1]#2{%
  \begingroup
  \def\tkz@parenthesis@for@err{(}%
  \def\tkz@maybe@parenthesis{#2}%
  \ifx\tkz@maybe@parenthesis\tkz@parenthesis@for@err
    \PackageError{tkz-base}{Syntax error  use {} instead of ()}{You need to use {} instead of ()}%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {\tkz@absorb@bad@arg}% 
  {\foreach \ptx/\pty/\name in {#2}{\tkzDefPoint[#1](\ptx,\pty){\name}}%
   \endgroup}%
}
\def\tkz@absorb@bad@arg#1){\endgroup}
%<--------------------------------------------------------------------------->
\def\tkz@node#1{ \pgfinterruptboundingbox
\path[coordinate](\tkzpt@xa,\tkzpt@ya) coordinate(#1);
 \endpgfinterruptboundingbox}  
% \def\tkz@drawnode#1{\path[coordinate](\tkzpt@xa,\tkzpt@ya) coordinate(#1);
%              \tkz@DrawPt{#1}
%              }
% 
%<--------------------------------------------------------------------------->
\def\tkzRenamePoint(#1)#2{\coordinate (#2) at (#1);}
\def\tkz@RenamePointEnd[#1]#2{\coordinate[#1] (#2) at (\tkz@ax,\tkz@ay);}
\def\tkzGetPoint#1{\coordinate  (#1) at (tkzPointResult);} 
\def\tkzGetPoints#1#2{\coordinate  (#1) at (tkzFirstPointResult);
                      \coordinate  (#2) at (tkzSecondPointResult);}
\def\tkzGetFirstPoint#1{\coordinate  (#1) at (tkzFirstPointResult);}
\def\tkzGetSecondPoint#1{\coordinate  (#1) at (tkzSecondPointResult);}
\def\tkzGetThirdPoint#1{\coordinate  (#1) at (tkzThirdPointResult);}
\def\tkzDefShiftPointCoord[#1](#2)#3{%
                \begin{scope}[shift={(#1)}]
                     \coordinate  (#3) at (#2);
                \end{scope}
                           }%
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
                            
%<--------------------------------------------------------------------------->
%            tkzDefShiftPoint
%<--------------------------------------------------------------------------->
\def\tkzDefShiftPoint[#1](#2)#3{%
   \tkz@@extractxy{#1}
   \tkz@ax\pgf@x %
   \tkz@ay\pgf@y %   
\begin{scope}[shift={(\tkz@ax,\tkz@ay)}]
   \coordinate  (#3) at (#2);
\end{scope}
}
%<--------------------------------------------------------------------------->
%                    Coordonnées d'un point 
%    result in #2x et #2y    #1 est le point et on récupère ses coordonnées
% usage soit A un point \tkzGetPointCoord(A){V} alors \Vx = xA et \Vy = yA
% en cm 
% tkzGetPointCoord avec [#1] cm ou bien pt ?? todo
%<--------------------------------------------------------------------------->
\def\tkzGetPointCoord(#1)#2{%
\begingroup
   \pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
   \pgfmathparse{\pgf@sys@tonumber{\pgf@x}/28.45274}
   \global\let\tkzresultx\pgfmathresult
   \global\expandafter\edef\csname #2x\endcsname{\tkzresultx}% 
   \pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}
   \pgfmathparse{\pgf@sys@tonumber{\pgf@y}/28.45274}
   \global\let\tkzresulty\pgfmathresult
   \global\expandafter\edef\csname #2y\endcsname{\tkzresulty}
\endgroup
}  
\def\tkz@@extractxy#1{%
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}} 
}
\let\tkzGetPointxy\tkzGetPointCoord
\makeatother  
\endinput

==> tikz-euclide/obj/tkz-obj-eu-polygons.tex <==
% tkz-obj-eu-polygons.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-obj-eu-polygons.tex} 
% bug in regular polygon side 2020/03/09
\makeatletter  
%<--------------------------------------------------------------------------–>
%                                 Polygon 
%<--------------------------------------------------------------------------–>
%<---------------------------   square  ------------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkzDefSquare(#1,#2){
\begingroup
  \tkzURotateAngle(#2,-90)(#1)
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \tkzURotateAngle(#1, 90)(#2)
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
%<---------------------   parallélogramme  ---------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkzDefParallelogram(#1,#2,#3){
\begingroup
\tkzDefPointWith[colinear= at #3](#2,#1)
\endgroup
}
%<---------------------   rectangle        ---------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkzDefRectangle{\pgfutil@ifnextchar[{\tkz@DefRectangle}%
                      {\tkz@DefRectangle[]}} 
\def\tkz@DefRectangle[#1](#2,#3){%
\begingroup
   \path[#1](#2) -| coordinate (tkzFirstPointResult) (#3) -| coordinate (tkzSecondPointResult) (#2);
\endgroup
}
%<-------------------------- gold rectangle -------------------------------–>
%
%<--------------------------------------------------------------------------–>
\def\tkzDefGoldRectangle(#1,#2){
\begingroup
  \tkzDefPointWith[K=-\tkzInvPhi](#2,#1)
  \pgfnodealias{tkzFirstPointResult}{tkzPointResult}
  \tkzDefPointWith[K=\tkzInvPhi](#1,#2)
  \pgfnodealias{tkzSecondPointResult}{tkzPointResult}
\endgroup
}
\let\tkzDefGoldenRectangle\tkzDefGoldRectangle
%<----------------------------   Regular Polygon   -------------------------–>
\def\tkz@numregpol{0}
\pgfkeys{/defregpoly/.cd,
      name/.store in      =  \tkz@regpolname,
      sides/.store in     =  \tkz@regpolsides,
      center/.code        =  \def\tkz@numregpol{0},
      side/.code          =  \def\tkz@numregpol{1},
      name/.default       =  P,
      sides/.default      =  5,
      center
} 
\def\tkzDefRegPolygon{\pgfutil@ifnextchar[{\tkz@DefRegPolygon}{\tkz@DefRegPolygon[]}}
\def\tkz@DefRegPolygon[#1](#2,#3){% 
\begingroup 
\pgfqkeys{/defregpoly}{#1}  
\ifcase\tkz@numregpol%
  \tkzRegPolygonCenter(#2,#3)
  \or%  
  \tkzRegPolygonSide(#2,#3)  
 \fi    
\endgroup
} 
\def\tkzRegPolygonCenter(#1,#2){
\begingroup 
   \foreach \v in {1,2,...,\tkz@regpolsides}
   {%
   \pgfmathsetmacro{\tkz@regangle}{360/\tkz@regpolsides*(\v-1)}  
   \tkzDefPointBy[rotation= center #1 angle \tkz@regangle](#2)   
   \pgfnodealias{\tkz@regpolname\v}{tkzPointResult}
   } 
\endgroup
}     
\def\tkzRegPolygonSide(#1,#2){
\begingroup  
% get the center 
\pgfmathsetmacro{\tkz@regangle}{360/\tkz@regpolsides*(\tkz@regpolsides-1)}
\pgfmathsetmacro{\tkz@regangleside}{(180-\tkz@regangle)/2}
\tkzDefMidPoint(#1,#2)
\pgfnodealias{tkz@tempPt}{tkzPointResult}
\tkz@@CalcLengthcm(tkz@tempPt,#1){tkz@len}
\pgfmathsetmacro{\tkz@inscriberadius}{%
  \tkz@len*tan(90*(\tkz@regpolsides-2)/\tkz@regpolsides)}
\tkzDefPointWith[orthogonal normed,K=\tkz@inscriberadius](tkz@tempPt,#2)
\pgfnodealias{tkz@RegPolCenter}{tkzPointResult}
\tkzRegPolygonCenter(tkz@RegPolCenter,#1)
\pgfnodealias{tkzPointResult}{tkz@RegPolCenter}
\endgroup
}
    

\makeatother
\endinput

==> tikz-euclide/obj/tkz-obj-eu-triangles.tex <==
% tkz-obj-eu-triangles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c  tkz-obj-eu-triangles.tex} 
\makeatletter  
%<--------------------------------------------------------------------------–>
%                       Triangle Equilateral
%<--------------------------------------------------------------------------–>
\def\tkzDefEquilateral(#1,#2){
\begingroup
 %\tkzDefMidPoint(#1,#2)
 \tkzURotateAngle(#1,60)(#2)
\endgroup
}
%<--------------------------------------------------------------------------–>
%                       Triangle Isosceles Right
%<--------------------------------------------------------------------------–>
\def\tkzDefIsoscelesRightTriangle(#1,#2){
\begingroup
 \tkzURotateAngle(#1,45)(#2)
 \pgfnodealias{tkz@a}{tkzPointResult}
  \tkzUHomo(#1,\tkzSqrTwobyTwo)(tkz@a)
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzDefIsoscelesRightTriangle(#1,#2){%
\begingroup
 \tkzURotateAngle(#1,45)(#2)
 \pgfnodealias{tkz@a}{tkzPointResult}
 \tkzUHomo(#1,\tkzSqrTwobyTwo)(tkz@a)
\endgroup
}
%<--------------------------------------------------------------------------–>
%                       Triangle OneTwo
%<--------------------------------------------------------------------------–>
\def\tkzDefTwoOne(#1,#2){
\begingroup
 \iftkz@swap@tr
     \tkzDefPointWith[K=-.5](#2,#1)
  \else
 \tkzDefPointWith[K=.5](#2,#1)
   \fi
 \endgroup
}
%<--------------------------------------------------------------------------– 
%         Pythagore
%<--------------------------------------------------------------------------– 
\def\tkzDefPythagore(#1,#2){
\begingroup
\iftkz@swap@tr
 \tkzDefPointWith[K=-.75](#2,#1)
 \else
  \tkzDefPointWith[K=.75](#2,#1)
  \fi
\endgroup
}
%<--------------------------------------------------------------------------– 
%     School
%<--------------------------------------------------------------------------– 
\def\tkzDefSchoolTriangle(#1,#2){
\begingroup
\iftkz@swap@tr
 \tkzDefPointWith(#2,#1) 
 \pgfnodealias{tkz@a}{tkzPointResult}
 \tkzURotateAngle(#1,-30)(#2)
 \tkzInterLL(#1,tkzPointResult)(#2,tkz@a)
\else
 \tkzDefPointWith(#2,#1) 
 \pgfnodealias{tkz@a}{tkzPointResult}
 \tkzURotateAngle(#1,30)(#2)
 \tkzInterLL(#1,tkzPointResult)(#2,tkz@a)
  \fi
\endgroup
}
%<--------------------------------------------------------------------------– 
%   Gold 
%<--------------------------------------------------------------------------– 
\def\tkzDefGoldTriangle(#1,#2){
\begingroup
 \iftkz@swap@tr
 \tkzDefPointWith[K=-\tkzInvPhi](#2,#1)
  \else
 \tkzDefPointWith[K=\tkzInvPhi](#2,#1)
   \fi
\endgroup
}
%<--------------------------------------------------------------------------– 
%
%<--------------------------------------------------------------------------– 
\def\tkzDefEuclideTriangle(#1,#2){
\begingroup
 \iftkz@swap@tr
 \tkzURotateAngle(#1,36)(#2)
  \else
 \tkzURotateAngle(#1,-36)(#2)
   \fi
\endgroup
}
%<--------------------------------------------------------------------------– 
%
%<--------------------------------------------------------------------------– 
\def\tkzDefGoldenTriangle(#1,#2){
\begingroup
 \tkzURotateAngle(#1,72)(#2)
 \tkzUHomo(#1,\tkzPhi)(tkzPointResult)
\endgroup
}
%<--------------------------------------------------------------------------– 
%
%<--------------------------------------------------------------------------– 
\def\tkzDefCheopsTriangle(#1,#2){
\begingroup
  \tkzDefMidPoint(#1,#2)
  \tkzDefPointWith[K=-\tkzSqrtPhi](tkzPointResult,#1)
\endgroup
}
%<--------------------------------------------------------------------------– 
%
%<--------------------------------------------------------------------------– 
\def\tkzDefTwoAnglesTriangle(#1,#2){
\begingroup
 \tkzURotateAngle(#1,\tkz@alpha)(#2)
 \pgfnodealias{tkz@a}{tkzPointResult}
 \tkzURotateAngle(#2,-\tkz@beta)(#1)
 \pgfnodealias{tkz@b}{tkzPointResult}
 \tkzInterLL(#1,tkz@a)(#2,tkz@b)
\endgroup
}
%<--------------------------------------------------------------------------–>
%                       Triangles
%<--------------------------------------------------------------------------–>

\def\tkz@numtr{0}
\pgfkeys{/deftriangle/.cd,
      equilateral/.code       = \def\tkz@numtr{0},
      half/.code              = \def\tkz@numtr{1},
      two one/.code           = \def\tkz@numtr{1},
      pythagore/.code         = \def\tkz@numtr{2},
      pythagoras/.code        = \def\tkz@numtr{2},
      right/.code             = \def\tkz@numtr{2},
      egyptian/.code          = \def\tkz@numtr{2},
      school/.code            = \def\tkz@numtr{3},
      golden/.code            = \def\tkz@numtr{4},
      sublime/.code           = \def\tkz@numtr{4},
      euclid/.code            = \def\tkz@numtr{5},
      euclide/.code           = \def\tkz@numtr{5},
      gold/.code              = \def\tkz@numtr{6},
      cheops/.code            = \def\tkz@numtr{7},
      two angles/.code  args  = {#1 and #2} { \def\tkz@numtr{8}%
                                              \def\tkz@alpha{#1}%
                                              \def\tkz@beta{#2}},
      isosceles right/.code    = \def\tkz@numtr{9},
      swap/.is if              =  tkz@swap@tr,
      swap/.default            =  true,
      swap                     =  false,
      equilateral
} 

\def\tkzDefTriangle{\pgfutil@ifnextchar[{\tkz@DefTriangle}{\tkz@DefTriangle[]}}
\def\tkz@DefTriangle[#1](#2,#3){% 
\begingroup  
\pgfqkeys{/deftriangle}{#1}  
\ifcase\tkz@numtr%
  \tkzDefEquilateral(#2,#3)
  \or% 1 
  \tkzDefTwoOne(#2,#3)  
  \or% 2
  \tkzDefPythagore(#2,#3)
  \or% 3
  \tkzDefSchoolTriangle(#2,#3)
  \or% 4
  \tkzDefGoldenTriangle(#2,#3)
  \or% 5
  \tkzDefEuclideTriangle(#2,#3)
  \or% 6
  \tkzDefGoldTriangle(#2,#3) 
  \or% 7
  \tkzDefCheopsTriangle(#2,#3)  
  \or% 8
  \tkzDefTwoAnglesTriangle(#2,#3)  
  \or% 9
  \tkzDefIsoscelesRightTriangle(#2,#3)  
  \fi    
\endgroup
}
%<--------------------------------------------------------------------------–>
%              les triangles sspécifiques
%<--------------------------------------------------------------------------–>

%<--------------------------------------------------------------------------– 
\def\tkz@numtspc{0}
\pgfkeys{/tkzDefSpcTriangle/.cd,
      in/.code                       = \def\tkz@numtspc{0},
      incentral/.code                = \def\tkz@numtspc{0},
      ex/.code                       = \def\tkz@numtspc{1},
      excentral/.code                = \def\tkz@numtspc{1},
      extouch/.code                  = \def\tkz@numtspc{2},
      intouch/.code                  = \def\tkz@numtspc{3},
      contact/.code                  = \def\tkz@numtspc{3},
      centroid/.code                 = \def\tkz@numtspc{4},
      medial/.code                   = \def\tkz@numtspc{4},
      orthic/.code                   = \def\tkz@numtspc{5},
      ortho/.code                    = \def\tkz@numtspc{5},
      feuerbach/.code                = \def\tkz@numtspc{6},
      euler/.code                    = \def\tkz@numtspc{7},
      tangential/.code               = \def\tkz@numtspc{8},
      symmedial/.code                = \def\tkz@numtspc{9},
      name/.store in                 = \tkz@pttr@name,
      name                           =  {},
      centroid,       
      }     
\def\tkzDefSpcTriangle{\pgfutil@ifnextchar[{\tkz@DefSpcTriangle}{%
                                 \tkz@DefSpcTriangle[]}}
\def\tkz@DefSpcTriangle[#1](#2)#3{% 
\begingroup  
\pgfqkeys{/tkzDefSpcTriangle}{#1}  
\ifcase\tkz@numtspc%
  \tkzDefIncentralTriangle(#2){#3}
  \or% 1 
  \tkzDefExcentralTriangle(#2){#3}  
  \or% 2
  \tkzDefExtouchTriangle(#2){#3}  
  \or% 3
  \tkzDefIntouchTriangle(#2){#3}  
  \or% 4
  \tkzDefCentroidTriangle(#2){#3} 
  \or% 5
  \tkzDefOrthicTriangle(#2){#3} 
  \or% 6
  \tkzDefFeuerbachTriangle(#2){#3} 
  \or% 7
  \tkzDefEulerTriangle(#2){#3}  
  \or% 8
  \tkzDefTangentialTriangle(#2){#3}  
  \or% 8
  \tkzDefSymmedialTriangle(#2){#3}  
    \fi    
\endgroup
}
 
\pgfkeys{/setuppttr/.is family}
\def\SetUpPTTR#1{\pgfqkeys{/setuppttr}{#1}}
\pgfkeys{/setuppttr/.cd,
   name/.store in   = \tkz@pttr@name,
   name             = {}
}
%<--------------------------------------------------------------------------– 
%     InCentral
%<--------------------------------------------------------------------------–
%<--------------------------------------------------------------------------–>
\def\@DefIncentralTriangle(#1,#2,#3)(#4,#5){%
\def\tkz@tmp{#5}%
    \tkz@recuplast(#3)
    \tkzDefBisectorLine(#2,#1,\tkz@last)
    \tkzInterLL(#2,\tkz@last)(#1,tkzPointResult)
    \pgfnodealias{\tkz@pttr@name#4}{tkzPointResult}
    \ifx\tkz@tmp\tkz@stop\else\@DefIncentralTriangle(#2,#3)(#5)\fi
}

\def\tkzDefIncentralTriangle{\pgfutil@ifnextchar[{%
                     \tkz@DefIncentralTriangle}{%
                     \tkz@DefIncentralTriangle[]}}
                     
\def\tkz@DefIncentralTriangle[#1](#2)#3{%
\begingroup
   \SetUpPTTR{#1}
   \pgfinterruptboundingbox 
   \@DefIncentralTriangle(#2,#2)(#3,\tkz@stop)
   \endpgfinterruptboundingbox
\endgroup
}
\let\tkzIncentralTriangle\tkzInExcentralTriangle
%<--------------------------------------------------------------------------– 
%     ExCentral
%<--------------------------------------------------------------------------–

%<--------------------------------------------------------------------------–>
\def\@DefExcentralTriangle(#1,#2,#3)(#4,#5){%
  \def\tkz@tmp{#5}%
  \tkz@recuplast(#3)
  \tkzDefExCircle(#2,#1,\tkz@last)  
  \pgfnodealias{\tkz@pttr@name#4}{tkzPointResult}
  \ifx\tkz@tmp\tkz@stop\else\@DefExcentralTriangle(#2,#3)(#5)\fi
}

\def\tkzDefExcentralTriangle{\pgfutil@ifnextchar[{%
         \tkz@DefExcentralTriangle}{%
         \tkz@DefExcentralTriangle[]}} 

\def\tkz@DefExcentralTriangle[#1](#2)#3{%
\begingroup
   \SetUpPTTR{#1}
   \@DefExcentralTriangle(#2,#2)(#3,\tkz@stop)
\endgroup
}
\let\tkzExcentralTriangle\tkzDefExcentralTriangle
%<--------------------------------------------------------------------------–>
% Intouch Triangle
%<--------------------------------------------------------------------------–>
\def\@DefIntouchTriangle(#1,#2,#3)(#4,#5){%
   \def\tkz@tmp{#5}%
    \tkz@recuplast(#3)
   \tkzUProjection(#2,\tkz@last)(tkz@pt)
   \pgfnodealias{\tkz@pttr@name#4}{tkzPointResult}
    \ifx\tkz@tmp\tkz@stop\else\@DefIntouchTriangle(#2,#3)(#5)\fi
}

\def\tkzDefIntouchTriangle{\pgfutil@ifnextchar[{%
                     \tkz@DefIntouchTriangle}{%
                     \tkz@DefIntouchTriangle[]}}
                      
\def\tkz@DefIntouchTriangle[#1](#2)#3{%
\begingroup
   \SetUpPTTR{#1}
   \tkzInCenter(#2) 
   \pgfnodealias{tkz@pt}{tkzPointResult}
   \@DefIntouchTriangle(#2,#2)(#3,\tkz@stop)
\endgroup
}
\let\tkzDefContactTriangle\tkzDefIntouchTriangle
%<--------------------------------------------------------------------------–>
% Extouch Triangle
%<--------------------------------------------------------------------------–>
\def\tkzDefExtouchTriangle{\pgfutil@ifnextchar[{%
                     \tkz@DefExtouchTriangle}{%
                     \tkz@DefExtouchTriangle[]}}
                      
\def\tkz@DefExtouchTriangle[#1](#2,#3,#4)#5{%
\begingroup
   \SetUpPTTR{#1}
    \foreach \name  [count=\i] in {#5} {%
         \global\expandafter\edef\csname tkz@point\i\endcsname{\name}
   }
   \begingroup
   \def\tkz@pttr@name{}
   \tkzDefExcentralTriangle(#2,#3,#4){tkz@a,tkz@b,tkz@c}
   \endgroup
   \tkzUProjection(#3,#4)(tkz@a)
   \pgfnodealias{\tkz@pttr@name\csname tkz@point1\endcsname}{tkzPointResult}
   \tkzUProjection(#2,#3)(tkz@c)
   \pgfnodealias{\tkz@pttr@name\csname tkz@point3\endcsname}{tkzPointResult}
   \tkzUProjection(#2,#4)(tkz@b)
   \pgfnodealias{\tkz@pttr@name\csname tkz@point2\endcsname}{tkzPointResult}
\endgroup
}
%<--------------------------------------------------------------------------–>
%  Feuerbach triangle 
%<--------------------------------------------------------------------------–>
\def\tkzDefFeuerbachTriangle{\pgfutil@ifnextchar[{%
   \tkz@DefFeuerbachTriangle}{\tkz@DefFeuerbachTriangle[]}}

\def\tkz@DefFeuerbachTriangle[#1](#2,#3,#4)#5{%
\begingroup
   \SetUpPTTR{#1}
   \foreach \name  [count=\i] in {#5} {%
         \global\expandafter\edef\csname tkz@point\i\endcsname{\name}
        }
   \tkzDefExCircle(#2,#3,#4) \tkzGetPoints{tkz@b}{tkz@hb}
   \tkzDefExCircle(#3,#4,#2) \tkzGetPoints{tkz@c}{tkz@hc}
   \tkzDefExCircle(#4,#2,#3) \tkzGetPoints{tkz@a}{tkz@ha}
   \tkzInterLC[near](#3,tkz@b)(tkz@b,tkz@hb)
   \tkzGetFirstPoint{\tkz@pttr@name\csname tkz@point2\endcsname}
   \tkzInterLC[near](#4,tkz@c)(tkz@c,tkz@hc)
   \tkzGetFirstPoint{\tkz@pttr@name\csname tkz@point3\endcsname}
   \tkzInterLC[near](#2,tkz@a)(tkz@a,tkz@ha)
   \tkzGetFirstPoint{\tkz@pttr@name\csname tkz@point1\endcsname}
\endgroup
}
%<--------------------------------------------------------------------------–>
%              Centroid
%<--------------------------------------------------------------------------–> 
% The medial triangle or midpoint triangle of a triangle ABC
\def\@DefCentroidTriangle(#1,#2,#3)(#4,#5){%
  \def\tkz@tmp{#5}%
  \tkz@recuplast(#3)
  \pgfcoordinate{\tkz@pttr@name#4}{%
  \pgfpointscale{0.5}{%
  \pgfpointadd{\pgfpointanchor{#2}{center}}%
               {\pgfpointanchor{\tkz@last}{center}}}
            }%
    \ifx\tkz@tmp\tkz@stop\else\@DefCentroidTriangle(#2,#3)(#5)\fi
     }
\def\tkzDefCentroidTriangle{\pgfutil@ifnextchar[{\tkz@DefCentroidTriangle}
                                    {\tkz@DefCentroidTriangle[]}} 
\def\tkz@DefCentroidTriangle[#1](#2)#3{%
\begingroup
   \SetUpPTTR{#1}
   \@DefCentroidTriangle(#2,#2)(#3,\tkz@stop)
\endgroup
}
\let\tkzDefMedialTriangle\tkzDefCentroidTriangle
\let\tkzDefMidpointTriangle\tkzDefCentroidTriangle
%<--------------------------------------------------------------------------–>
% Orthic Triangle H Ha Hb Hc modif 3.03
%<--------------------------------------------------------------------------–>
\def\@DefOrthicTriangle(#1,#2,#3)(#4,#5){%
    \def\tkz@tmp{#5}%
    \tkz@recuplast(#3)
    \tkzUProjection(#2,\tkz@last)(#1) 
    \pgfnodealias{\tkz@pttr@name#4}{tkzPointResult}
    \ifx\tkz@tmp\tkz@stop\else\@DefOrthicTriangle(#2,#3)(#5)\fi
}

\def\tkzDefOrthicTriangle{\pgfutil@ifnextchar[{\tkz@DefOrthicTriangle}
                                   {\tkz@DefOrthicTriangle[]}} 
\def\tkz@DefOrthicTriangle[#1](#2)#3{%
\begingroup
   \SetUpPTTR{#1}
   \@DefOrthicTriangle(#2,#2)(#3,\tkz@stop)
\endgroup
}
\let\tkzDefAltitudeTriangle\tkzDefOrthicTriangle

%<--------------------------------------------------------------------------–>
% The Euler triangle
%<--------------------------------------------------------------------------–>
\def\tkzDefEulerTriangle{\pgfutil@ifnextchar[{%
   \tkz@DefEulerTriangle}{\tkz@DefEulerTriangle[]}}   
\def\tkz@DefEulerTriangle[#1](#2,#3,#4)#5{%
\begingroup
   \SetUpPTTR{#1}
   \pgfinterruptboundingbox 
   \tkzOrthoCenter(#2,#3,#4) 
   \pgfnodealias{tkz@e}{tkzPointResult}
   \tkzDefMidPoint(#2,tkz@e)
   \pgfnodealias{tkz@m1}{tkzPointResult}
   \tkzDefMidPoint(#3,tkz@e)
   \pgfnodealias{tkz@m2}{tkzPointResult}
   \tkzDefMidPoint(#4,tkz@e)
   \pgfnodealias{tkz@m3}{tkzPointResult}
   \endpgfinterruptboundingbox
   \foreach \name  [count=\i] in {#5} {%
   \coordinate (\tkz@pttr@name\name) at (tkz@m\i);
   }
\endgroup
}
%<--------------------------------------------------------------------------–>
%  TangentialTriangle
%<--------------------------------------------------------------------------–>
\def\tkzDefTangentialTriangle{\pgfutil@ifnextchar[{%
   \tkz@DefTangentialTriangle}{\tkz@DefTangentialTriangle[]}}  
\def\tkz@DefTangentialTriangle[#1](#2,#3,#4)#5{%
\begingroup
   \SetUpPTTR{#1}
   \tkzCircumCenter(#2,#3,#4)       
   \pgfnodealias{tkz@circ}{tkzPointResult}
   \tkzDefLine[orthogonal=through #2](tkz@circ,#2) 
   \pgfnodealias{tkz@pta}{tkzPointResult}  
   \tkzDefLine[orthogonal=through #3](tkz@circ,#3) 
   \pgfnodealias{tkz@ptb}{tkzPointResult}  
   \tkzDefLine[orthogonal=through #4](tkz@circ,#4) 
   \pgfnodealias{tkz@ptc}{tkzPointResult}  
   \tkzInterLL(#2,tkz@pta)(#3,tkz@ptb) 
   \pgfnodealias{tkz@tg3}{tkzPointResult}
   \tkzInterLL(#3,tkz@ptb)(#4,tkz@ptc) 
   \pgfnodealias{tkz@tg1}{tkzPointResult}   
   \tkzInterLL(#4,tkz@ptc)(#2,tkz@pta) 
   \pgfnodealias{tkz@tg2}{tkzPointResult}   
   \foreach \name  [count=\i] in {#5} {%
   \coordinate (\tkz@pttr@name\name) at (tkz@tg\i);
   }
\endgroup
}
%<--------------------------------------------------------------------------– 
%     tkzDefSymmedianLine
%<--------------------------------------------------------------------------–
\def\@DefSymmedialTriangle(#1,#2,#3)(#4,#5){%
    \def\tkz@tmp{#5}%
     \tkz@recuplast(#3)
     \tkzDefSymmedianLine(#2,#1,\tkz@last)
     \tkzInterLL(#2,\tkz@last)(#1,tkzPointResult)
     \pgfnodealias{\tkz@pttr@name#4}{tkzPointResult}
     \ifx\tkz@tmp\tkz@stop\else\@DefSymmedialTriangle(#2,#3)(#5)\fi
}

\def\tkzDefSymmedialTriangle{\pgfutil@ifnextchar[{%
                     \tkz@DefSymmedialTriangle}{%
                     \tkz@DefSymmedialTriangle[]}}
                     
\def\tkz@DefSymmedialTriangle[#1](#2)#3{%
\begingroup
   \SetUpPTTR{#1}
   \pgfinterruptboundingbox 
   \@DefSymmedialTriangle(#2,#2)(#3,\tkz@stop)
   \endpgfinterruptboundingbox
\endgroup
}
\makeatother
\endinput

==> tikz-euclide/tools-lua/tkz-tools-lua-angles.tex <==
% tkz-tools-lua-angles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-lua-angles.tex}   
\makeatletter
\def\tkzmathrotatepointaround#1#2#3{%
  \pgf@process{%
    \pgf@process{#1}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@process{#2}%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    \pgf@x=\pgf@xc%
    \pgf@y=\pgf@yc%
    \advance\pgf@x-\pgf@xa%
    \advance\pgf@y-\pgf@ya%
    \pgfmathsetmacro\angle{#3}%
    \edef\sineangle{\tkz@Dec{\tkz@Sin{\tkz@Rad{\angle}}}}%
    \edef\cosineangle{\tkz@Dec{\tkz@Cos{\tkz@Rad{\angle}}}}%
    \pgf@xa\cosineangle\pgf@x%
    \advance\pgf@xa-\sineangle\pgf@y%
    \pgf@ya\sineangle\pgf@x%
    \advance\pgf@ya\cosineangle\pgf@y%
    \pgf@x\pgf@xb%
    \pgf@y\pgf@yb%
    \advance\pgf@x\pgf@xa%
    \advance\pgf@y\pgf@ya%
  }%
}

%<-------------------------------------------------------------------------->
%                           Angles
%<-------------------------------------------------------------------------->
\def\tkzmathanglebetweenpoints#1#2{
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}%
\edef\tkzax{\strip@pt\pgf@x}%
\edef\tkzay{\strip@pt\pgf@y}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}}%
\edef\tkzbx{\strip@pt\pgf@x}%
\edef\tkzby{\strip@pt\pgf@y}%
\edef\tkz@tmp{\tkz@Angle{\tkzax}{\tkzay}{\tkzbx}{\tkzby}}
\edef\pgfmathresult{\tkz@Dec{\tkz@Round{\tkz@tmp}{2}}}
}
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% thanks karu : http://tex.stackexchange.com/questions/151667/tkzgetangle-strange-behavior/196224#196224  
% \tkzGetAngle strange behavior
% defines \tkz@FirstAngle and \tkz@SecondAngle sens  trigo
%<--------------------------------------------------------------------------–>

\def\tkzNormalizeAngle(#1,#2){%
\directlua{angleA, angleB = normalize(#1,#2)
token.set_macro("tkz@FirstAngle", angleA)
token.set_macro("tkz@SecondAngle", angleB)
}}
%<--------------------------------------------------------------------------–>
%                          Angle 
% Recherche l'angle formé par #1 et #2 par rapport à l'horizontale
%<--------------------------------------------------------------------------–>
\def\tkzFindSlopeAngle(#1,#2){%
\begingroup
  \tkzmathanglebetweenpoints{#1}{#2}
 \global\let\tkzAngleResult\pgfmathresult  
\endgroup
}
%<--------------------------------------------------------------------------–>
%                          Angle  avec trois nodes
%<--------------------------------------------------------------------------–>
\def\tkzFindAngle(#1,#2,#3){% new code 2016
\begingroup
    \tkzFindSlopeAngle(#2,#1)\tkzGetAngle{tkz@FirstAngle}
    \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@SecondAngle}
    \tkzNormalizeAngle(\tkz@FirstAngle,\tkz@SecondAngle)
    \edef\tkz@Angle{\fpeval{\tkz@SecondAngle-\tkz@FirstAngle}}
    \global\let\tkzAngleResult\tkz@Angle
\endgroup
}

%<--------------------------------------------------------------------------–>
% Find angle
%<--------------------------------------------------------------------------–>
\def\tkzGetAngle#1{%
  \global\expandafter\edef\csname #1\endcsname{\tkzAngleResult}
}  
\makeatother
\endinput

==> tikz-euclide/tools-lua/tkz-tools-lua-base.tex <==
% tkz-tools-lua-base.tex    
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-lua-base.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
\global\let\tkz@tmp@xa\tkz@init@xmin% modif  2016
\global\let\tkz@tmp@xb\tkz@init@xmax% modif  2016
\global\let\tkz@tmp@ya\tkz@init@ymin% modif  2016
\global\let\tkz@tmp@yb\tkz@init@ymax% modif  2016 
%<--------------------------------------------------------------------------–>
\pgfkeys{
         /tkzInit/.cd,
         xmin/.store in     = \tkz@init@xmin,
         xmax/.store in     = \tkz@init@xmax,
         xstep/.store in    = \tkz@init@xstep,
         ymin/.store in     = \tkz@init@ymin,
         ymax/.store in     = \tkz@init@ymax,
         ystep/.store in    = \tkz@init@ystep, 
         NO/.is if          = tkz@init@NO,
         NO/.default        = true, 
         xmin               = 0,
         xmax               = 10,
         xstep              = 1,
         ymin               = 0,
         ymax               = 10,
         ystep              = 1,
         NO                 = false 
         } 
  
\def\tkzInit{\pgfutil@ifnextchar[{\tkz@Init}{\tkz@Init[]}} 
\def\tkz@Init[#1]{%
    \pgfqkeys{/tkzInit}{#1}
  \ifx\tkzfctloaded\undefined
    \else   
      \tkz@tkzf@fct=0 %  only if tkz-fct loaded
   \fi   
  \xdef\tkz@init@xorigine{0}
  \xdef\tkz@init@yorigine{0}
  \edef\@xsgmin{\fpeval{sign(\tkz@init@xmin)}}
  \edef\@xsgmax{\fpeval{sign(\tkz@init@xmax)}}
  \edef\@ysgmin{\fpeval{sign(\tkz@init@ymin)}}
  \edef\@ysgmax{\fpeval{sign(\tkz@init@ymax)}}
  \let\tkz@tmp@xa\tkz@init@xmin %modif 2016
  \let\tkz@tmp@xb\tkz@init@xmax %modif 2016
  \let\tkz@tmp@ya\tkz@init@ymin %modif 2016
  \let\tkz@tmp@yb\tkz@init@ymax %modif 2016
  \tkz@init@NOfalse                   
  \ifx\@xsgmin\@xsgmax \tkz@init@NOtrue \fi
  \ifx\@ysgmin\@ysgmax \tkz@init@NOtrue \fi
  \iftkz@init@NO%
  \ifx\@xsgmin\@xsgmax
      \edef\tkz@init@xmax{\tkz@Dec{\tkz@init@xmax-(\tkz@init@xmin)}}
      \edef\tkz@init@xorigine{\tkz@init@xmin}
      \edef\tkz@init@xmin{0}
  \fi
  \ifx\@ysgmin\@ysgmax
      \edef\tkz@init@ymax{\tkz@Dec{\tkz@init@ymax-(\tkz@init@ymin)}}
      \edef\tkz@init@yorigine{\tkz@init@ymin}
      \edef\tkz@init@ymin{0}
  \fi
  \fi
  \edef\tkz@xa{\tkz@Dec{\tkz@init@xmin/\tkz@init@xstep}}
  \edef\tkz@xb{\tkz@Dec{\tkz@init@xmax/\tkz@init@xstep}}
  \edef\tkz@ya{\tkz@Dec{\tkz@init@ymin/\tkz@init@ystep}}
  \edef\tkz@yb{\tkz@Dec{\tkz@init@ymax/\tkz@init@ystep}}
  \tkz@getdecimal{\tkz@init@xstep} % amélioration nb dec et integer
  \xdef\tkz@init@xdec{\number\c@pgfmath@countb}
  \tkz@getdecimal{\tkz@init@ystep}
  \xdef\tkz@init@ydec{\number\c@pgfmath@countb}
}%
\def\tkzAddName{\pgfutil@ifnextchar[{\tkz@AddName}{\tkz@AddName[]}} 
\def\tkz@AddName[#1]#2{%
\node[above left,#1] at (\pgf@path@lastx,\pgf@path@lasty){#2};  
}% 
%<--------------------------------------------------------------------------–>
\makeatother 
\endinput

==> tikz-euclide/tools-lua/tkz-tools-lua-intersections.tex <==
% tkz-tools-lua-intersections.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status “maintained”.
% 
% The Current Maintainer of this work is Alain Matthes.
%  utf8 encoding

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-lua-intersections.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%                 intersection  de deux lignes
%<--------------------------------------------------------------------------–>
\def\tkzInterLL(#1,#2)(#3,#4){% méthode avec xfp
\tkz@InterLL(#1,#2)(#3,#4){tkzPointResult}
}

\def\tkz@InterLL(#1,#2)(#3,#4)#5{%
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}%
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}}
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#3}{center}}%
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#4}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#4}{center}}%
\tkz@dx\pgf@x%
\tkz@dy\pgf@y%
\edef\tkzax{\strip@pt\tkz@ax}%
\edef\tkzay{\strip@pt\tkz@ay}%
\edef\tkzbx{\strip@pt\tkz@bx}%
\edef\tkzby{\strip@pt\tkz@by}%
\edef\tkzcx{\strip@pt\tkz@cx}%
\edef\tkzcy{\strip@pt\tkz@cy}%
\edef\tkzdx{\strip@pt\tkz@dx}%
\edef\tkzdy{\strip@pt\tkz@dy}%
\edef\tkz@deltax{\tkz@Dec{(\tkzax-(\tkzbx))/(28.45274)}}
\edef\tkz@deltaxx{\tkz@Dec{(\tkzcx-(\tkzdx))/(28.45274)}}
\edef\tkz@deltay{\tkz@Dec{(\tkzay-(\tkzby))/(28.45274)}}
\edef\tkz@deltayy{\tkz@Dec{(\tkzcy-(\tkzdy))/(28.45274)}}
\edef\tkz@deltaxy{\tkz@Dec{((\tkzax*\tkzby)-(\tkzay*\tkzbx))/(809.55841)}}
\edef\tkz@deltaxxyy{\tkz@Dec{((\tkzcx*\tkzdy)-(\tkzcy*\tkzdx))/(809.55841)}}
\edef\tkz@div{\tkz@Dec{(\tkz@deltax*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxx)}}
\edef\tkz@numx{\tkz@Dec{(\tkz@deltaxy*\tkz@deltaxx)-(\tkz@deltax*\tkz@deltaxxyy)}}
\edef\tkz@numy{\tkz@Dec{(\tkz@deltaxy*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxxyy)}}
\edef\tkz@xs{\tkz@Dec{\tkz@numx/\tkz@div}}
\edef\tkz@ys{\tkz@Dec{\tkz@numy/\tkz@div}}
\edef\tkz@xs{\tkz@Round{\tkz@xs}{5}}
\edef\tkz@ys{\tkz@Round{\tkz@ys}{5}}
\path[coordinate](\tkz@xs,\tkz@ys) coordinate (#5);
}


% méthode with coordinates
\def\tkzInterLLxy(#1,#2,#3,#4)(#5,#6,#7,#8){%
%\path (intersection of #1--#2 and #3--#4) coordinate(#5);%
\tkz@ax#1%
\tkz@ay#2%
\tkz@bx#3%
\tkz@by#4%
\tkz@cx#5%
\tkz@cy#6%
\tkz@dx#7%
\tkz@dy#8%
\edef\tkzax{\strip@pt\tkz@ax}%
\edef\tkzay{\strip@pt\tkz@ay}%
\edef\tkzbx{\strip@pt\tkz@bx}%
\edef\tkzby{\strip@pt\tkz@by}%
\edef\tkzcx{\strip@pt\tkz@cx}%
\edef\tkzcy{\strip@pt\tkz@cy}%
\edef\tkzdx{\strip@pt\tkz@dx}%
\edef\tkzdy{\strip@pt\tkz@dy}%
\edef\tkz@deltax{\tkz@Dec{(\tkzax-(\tkzbx))/(28.45274)}}
\edef\tkz@deltaxx{\tkz@Dec{(\tkzcx-(\tkzdx))/(28.45274)}}
\edef\tkz@deltay{\tkz@Dec{(\tkzay-(\tkzby))/(28.45274)}}
\edef\tkz@deltayy{\tkz@Dec{(\tkzcy-(\tkzdy))/(28.45274)}}
\edef\tkz@deltaxy{\tkz@Dec{((\tkzax*\tkzby)-(\tkzay*\tkzbx))/(809.55841)}}
\edef\tkz@deltaxxyy{\tkz@Dec{((\tkzcx*\tkzdy)-(\tkzcy*\tkzdx))/(809.55841)}}
\edef\tkz@div{\tkz@Dec{(\tkz@deltax*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxx)}}
\edef\tkz@numx{\tkz@Dec{(\tkz@deltaxy*\tkz@deltaxx)-(\tkz@deltax*\tkz@deltaxxyy)}}
\edef\tkz@numy{\tkz@Dec{(\tkz@deltaxy*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxxyy)}}
\edef\tkz@xs{\tkz@Dec{\tkz@numx/\tkz@div}}
\edef\tkz@ys{\tkz@Dec{\tkz@numy/\tkz@div}}
\edef\tkz@xs{\tkz@Round{\tkz@xs}{5}}
\edef\tkz@ys{\tkz@Round{\tkz@ys}{5}}
\path[coordinate](\tkz@xs,\tkz@ys) coordinate (tkzPointResult);
}

%<--------------------------------------------------------------------------–>
%                 intersection  de Ligne Cercle rayon connu
%<--------------------------------------------------------------------------–>
% /*
%    Calculate the intersection of a ray and a sphere
%    The line segment is defined from p1 to p2
%    The sphere is of radius r and centered at sc
%    There are potentially two points of intersection given by
%    p = p1 + mu1 (p2 - p1)
%    p = p1 + mu2 (p2 - p1)
%    Return FALSE if the ray doesn't intersect the sphere.
% */
% int RaySphere(XYZ p1,XYZ p2,XYZ sc,double r,double *mu1,double *mu2)
% {
%    double a,b,c;
%    double bb4ac;
%    XYZ dp;
% 
%    dp.x = p2.x - p1.x;
%    dp.y = p2.y - p1.y;
%    dp.z = p2.z - p1.z;
%    a = dp.x * dp.x + dp.y * dp.y + dp.z * dp.z;
%    b = 2 * (dp.x * (p1.x - sc.x) + dp.y * (p1.y - sc.y) + dp.z * (p1.z - sc.z));
%    c = sc.x * sc.x + sc.y * sc.y + sc.z * sc.z;
%    c += p1.x * p1.x + p1.y * p1.y + p1.z * p1.z;
%    c -= 2 * (sc.x * p1.x + sc.y * p1.y + sc.z * p1.z);
%    c -= r * r;
%    bb4ac = b * b - 4 * a * c;
%    if (ABS(a) < EPS || bb4ac < 0) {
%       *mu1 = 0;
%       *mu2 = 0;
%       return(FALSE);
%    }
% 
%    *mu1 = (-b + sqrt(bb4ac)) / (2 * a);
%    *mu2 = (-b - sqrt(bb4ac)) / (2 * a);
% 
%    return(TRUE);
% }
%<---------- test ------------------------------------------------------–>
\def\tkzTestInterLC(#1,#2)(#3,#4){%
\begingroup
\tkz@Projection(#1,#2)(#3){tkz@pth}% distance centre à la ligne
\tkz@@CalcLength(#3,tkz@pth){tkz@mathLen}%  
\tkz@@CalcLength(#3,#4){tkzLengthResult}%calcul du rayon
\ifdim\tkz@mathLen pt>\tkzLengthResult pt\relax%
\global\tkzFlagLCfalse
\else
\global\tkzFlagLCtrue
\fi
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkz@numlc{0}
\pgfkeys{/linecircle/.cd,
  node/.code               = \def\tkz@numlc{0},
  R/.code                  = \def\tkz@numlc{1}, 
  with nodes/.code         = \def\tkz@numlc{2},
  common/.store in         = \tkz@common,
  common                   = {},
  near/.is if              =  tkz@near,
  near/.default            =  true,
  near                     =  false,
  next to/.store in        = \tkz@nextto,
  next to/.initial         = {},
  next/.default            = {},
  next to                  = {},
  next to/.value required,
  node  
 }
%<--------------------------------------------------------------------------–>
\def\tkzInterLC{\pgfutil@ifnextchar[{\tkz@InterLC}{\tkz@InterLC[]}}
\def\tkz@InterLC[#1](#2,#3)(#4,#5){%
\begingroup      
\pgfqkeys{/linecircle}{#1}
 \pgfinterruptboundingbox 
\ifcase\tkz@numlc%
    % first case 0
  \tkz@@CalcLength(#4,#5){tkzLengthResult}
  \tkzInterLCR(#2,#3)(#4,\tkzLengthResult pt){tkzFirstPointResult}%
                         {tkzSecondPointResult}
\or% 1
    \tkzInterLCR(#2,#3)(#4,#5 cm){tkzFirstPointResult}
                   {tkzSecondPointResult}%
\or% 2
    \tkzInterLCWithNodes(#2,#3)(#4,#5){tkzFirstPointResult}%
                        {tkzSecondPointResult}%
\fi
\iftkz@near
  \tkz@@CalcLength(#2,tkzFirstPointResult){tkzLengthFirst}
  \tkz@@CalcLength(#2,tkzSecondPointResult){tkzLengthSecond}
      \ifdim \tkzLengthFirst pt < \tkzLengthSecond pt\relax%
      \else
       \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
       \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
       \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
      \fi
\else
    \ifx\tkz@common\tkzutil@empty 
      \ifx\tkz@nextto\tkzutil@empty 
         \tkzFindAngle(tkzSecondPointResult,tkzFirstPointResult,#4)   
         \tkzGetAngle{tkz@an}
          \ifdim\tkz@an pt<180 pt\relax%
          \else
           \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
           \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
           \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
          \fi
      \else
         \tkz@@CalcLength(\tkz@nextto,tkzFirstPointResult){tkzLengthFirst}
         \tkz@@CalcLength(\tkz@nextto,tkzSecondPointResult){tkzLengthSecond}
             \ifdim \tkzLengthFirst pt < \tkzLengthSecond pt\relax%
             \else
              \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
              \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
              \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
             \fi
       \fi
    \else 
         \tkz@@CalcLength(\tkz@common,tkzSecondPointResult){tkz@mathLen}
         \ifdim\tkz@mathLen pt<1pt\relax%
         \else
          \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
          \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
          \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
         \fi
     \fi
\fi%near
\endpgfinterruptboundingbox    
\endgroup
}
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzInterLCR(#1,#2)(#3,#4)#5#6{%
\begingroup
\tkz@radi=#4%
\tkz@@extractxy{#3}
\tkz@bx =\pgf@x\relax%
\tkz@by =\pgf@y\relax%
\tkz@Projection(#1,#2)(#3){tkz@pth}
\tkz@@CalcLength(#3,tkz@pth){tkz@mathLen}
 \ifdim\tkz@mathLen pt<0.05pt\relax%
        \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                     {\pgfpointanchor{#2}{center}}%
        \tkz@ax=\pgf@x%
        \tkz@ay=\pgf@y%
        \pgfpointborderellipse{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                              {\pgfpoint{\tkz@radi}{\tkz@radi}}
        \tkz@ax=\pgf@x\relax%
        \tkz@ay=\pgf@y\relax%
        \advance\tkz@bx by\tkz@ax\relax%
        \advance\tkz@by by\tkz@ay\relax%
        \pgfcoordinate{#6}{\pgfqpoint{\tkz@bx}{\tkz@by}}
        \tkzCSym(#3)(#6){#5}
  \else
       \edef\pgfmathresult{\fpeval{\tkz@mathLen/\tkz@radi}}
      % \edef\tkz@angle{\fpeval{acosd(\pgfmathresult)}}
        \pgfmathacos@{\pgfmathresult}%
        \let\tkz@angle\pgfmathresult%
        \pgfpointdiff{\pgfpointanchor{#3}{center}}%
                     {\pgfpointanchor{tkz@pth}{center}}%
        \tkz@ax=\pgf@x%
        \tkz@ay=\pgf@y%
        \pgfpointborderellipse{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                              {\pgfpoint{\tkz@radi}{\tkz@radi}}
        \tkz@ax =\pgf@x\relax%
        \tkz@ay =\pgf@y\relax%
        \advance\tkz@bx by\tkz@ax\relax%
        \advance\tkz@by by\tkz@ay\relax%
        \tkz@@extractxy{#3}
        \tkz@ax =\pgf@x\relax%
        \tkz@ay =\pgf@y\relax%
        \tkz@@extractxy{tkz@pth}
        \pgfmathrotatepointaround{\pgfpoint{\tkz@bx}{\tkz@by}}%
                                 {\pgfpoint{\tkz@ax}{\tkz@ay}}%
                                 {\tkz@angle}
         \pgfcoordinate{#5}{\pgfqpoint{\pgf@x}{\pgf@y}}
        \pgfmathrotatepointaround{\pgfpoint{\tkz@bx}{\tkz@by}}%
                                 {\pgfpoint{\tkz@ax}{\tkz@ay}}%
                                 {-\tkz@angle}
  \pgfcoordinate{#6}{\pgfqpoint{\pgf@x}{\pgf@y}}

\fi   
\endgroup
}
%<--------------------------------------------------------------------------–>
%                 intersection  de Ligne Cercle 
% #4 center #5 point sur le cercle
%<--------------------------------------------------------------------------–>
% \def\tkzInterLC(#1,#2)(#3,#4)#5#6{%
%     \begingroup
%     \tkz@@CalcLength(#3,#4){tkz@rad}
%     \tkzInterLCR(#1,#2)(#3,\tkz@rad pt){#5}{#6}
% \endgroup
% } 
%<--------------------------------------------------------------------------–>
%                 intersection  de Ligne Cercle rayon inconnu
%<--------------------------------------------------------------------------–>
\def\tkzInterLCWithNodes(#1,#2)(#3,#4,#5)#6#7{%
\begingroup
    \tkz@@CalcLength(#4,#5){tkz@radius}
    \tkzInterLCR(#1,#2)(#3,\tkz@radius pt){#6}{#7}
\endgroup
}
%<--------------------------------------------------------------------------–>
%  Intersection of 2 circles
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% méthode
% /* circle_circle_intersection() *
%  * Determine the points where 2 circles in a common plane intersect.
%  *
%  * int circle_circle_intersection(
%  *                                // center and radius of 1st circle
%  *                                double x0, double y0, double r0,
%  *                                // center and radius of 2nd circle
%  *                                double x1, double y1, double r1,
%  *                                // 1st intersection point      
%  *                                // 2nd intersection point
%  *
%  * This is a public domain work. 3/26/2005 Tim Voght
%  *
% int circle_circle_intersection(double x0, double y0, double r0,
%                                double x1, double y1, double r1,
%                                double *xi, double *yi,
%                                double *xi_prime, double *yi_prime)
% {
%   double a, dx, dy, d, h, rx, ry;
%   double x2, y2;
% 
%   /* dx and dy are the vertical and horizontal distances between
%    * the circle centers.
%    */
%   dx = x1 - x0;
%   dy = y1 - y0;
% 
%   /* Determine the straight-line distance between the centers. */
%   //d = sqrt((dy*dy) + (dx*dx));
%   d = hypot(dx,dy); // Suggested by Keith Briggs
% 
%   /* Check for solvability. */
%   if (d > (r0 + r1))
%   {
%     /* no solution. circles do not intersect. */
%     return 0;
%   }
%   if (d < fabs(r0 - r1))
%   {
%     /* no solution. one circle is contained in the other */
%     return 0;
%   }
% 
%   /* 'point 2' is the point where the line through the circle
%    * intersection points crosses the line between the circle
%    * centers.  
%    */
% 
%   /* Determine the distance from point 0 to point 2. */
%   a = ((r0*r0) - (r1*r1) + (d*d)) / (2.0 * d) ;
% 
%   /* Determine the coordinates of point 2. */
%   x2 = x0 + (dx * a/d);
%   y2 = y0 + (dy * a/d);
% 
%   /* Determine the distance from point 2 to either of the
%    * intersection points.
%    */
%   h = sqrt((r0*r0) - (a*a));
% 
%   /* Now determine the offsets of the intersection points from
%    * point 2.
%    */
%   rx = -dy * (h/d);
%   ry = dx * (h/d);
% 
%   /* Determine the absolute intersection points. */
%   *xi = x2 + rx;
%   *xi_prime = x2 - rx;
%   *yi = y2 + ry;
%   *yi_prime = y2 - ry;
% 
%   return 1;
% } 
%<--------------------------------------------------------------------------–>
%    Intersection de deux cercles  
%<--------------------------------------------------------------------------–>
%<---------- test ------------------------------------------------------–>
% test avec des nodes  R-r <= d <= R+r
\def\tkzTestInterCC(#1,#2)(#3,#4){%
\begingroup
\tkz@@CalcLength(#1,#3){tkz@mathLen}% distance entre les centres  
\tkz@@CalcLength(#2,#1){tkz@rA}%calcul du rayon
\tkz@@CalcLength(#4,#3){tkz@rB}%calcul du rayon
% test if d <= rA + rB ?
\edef\tkz@rS{\fpeval{\tkz@rA+\tkz@rB}}
\ifdim\tkz@mathLen pt > \tkz@rS pt\relax%
\global\tkzFlagCCfalse
\else
% now test if d>= rA - rB or rB-rA
  \ifdim \tkz@rA pt >  \tkz@rB pt\relax%
       \edef\tkz@rD{\fpeval{\tkz@rA-\tkz@rB}}
   \else
       \edef\tkz@rD{\fpeval{\tkz@rB-\tkz@rA}}
   \fi
\ifdim  \tkz@rD pt > \tkz@mathLen pt\relax%
 \global\tkzFlagCCfalse
\else
\global\tkzFlagCCtrue
\fi
\fi
\endgroup
}

\def\tkz@numcc{0}
\pgfkeys{
/circlecircle/.cd,
  node/.code           = \def\tkz@numcc{0},
  R/.code              = \def\tkz@numcc{1},
  with nodes/.code     = \def\tkz@numcc{2},
  common/.store in     = \tkz@common,
  common               = {},
  node
}
%<--------------------------------------------------------------------------–>
\def\tkzInterCC{\pgfutil@ifnextchar[{\tkz@InterCC}{\tkz@InterCC[]}}
\def\tkz@InterCC[#1](#2,#3)(#4,#5){%
\begingroup      
\pgfqkeys{/circlecircle}{#1}
\ifcase\tkz@numcc%
 % first case 0 
  \tkz@save@length 
  \tkz@@CalcLengthcm(#2,#3){tkz@rayA}
  \tkz@@CalcLengthcm(#4,#5){tkz@rayB}
   \tkz@restore@length
\tkzInterCCR(#2,\tkz@rayA)(#4,\tkz@rayB){tkzFirstPointResult}{tkzSecondPointResult}
  \or% 1
 \tkzInterCCR(#2,#3)(#4,#5){tkzFirstPointResult}{tkzSecondPointResult}%
  \or%2
 \tkzInterCCWithNodes(#2,#3)(#4,#5){tkzFirstPointResult}{tkzSecondPointResult}
\fi
 \ifx\tkz@common\tkzutil@empty
 \tkzFindAngle(#2,tkzFirstPointResult,#4)   \tkzGetAngle{tkz@an}
 \ifdim\tkz@an pt<180 pt\relax%
 \else
 \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
  \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
 \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
 \fi
 \else
\tkz@@CalcLength(\tkz@common,tkzSecondPointResult){tkz@mathLen}
 \ifdim\tkz@mathLen pt<0.05pt\relax%
 \else
  \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
   \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
  \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
  \fi
  \fi
\endgroup
} 
%<--------------------------------------------------------------------------–>

\def\tkzInterCCR(#1,#2)(#3,#4)#5#6{%
\begingroup
\pgfinterruptboundingbox  
\tkz@save@length  
\tkz@@CalcLength(#1,#3){tkz@dd}
\tkz@restore@length 
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}
\tkz@ax\pgf@x %
\tkz@ay\pgf@y %
\edef\tkzcax{\strip@pt\tkz@ax}%
\edef\tkzcay{\strip@pt\tkz@ay}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#3}{center}}
\tkz@bx\pgf@x %
\tkz@by\pgf@y %
\edef\tkzcbx{\strip@pt\tkz@bx}%
\edef\tkzcby{\strip@pt\tkz@by}%
\tkz@cx#2cm %
\tkz@cy#4cm %
\edef\tkzccx{\strip@pt\tkz@cx}%
\edef\tkzccy{\strip@pt\tkz@cy}%
\edef\tkz@aa{\tkz@Dec{((\tkzccx+\tkzccy)/(2*\tkz@dd))*(\tkzccx-(\tkzccy))+\tkz@dd/2}}
\edef\tkz@xx{\tkz@Dec{\tkzcax+\tkz@aa/\tkz@dd*(\tkzcbx - (\tkzcax))}}
\edef\tkz@yy{\tkz@Dec{\tkzcay+\tkz@aa/\tkz@dd*(\tkzcby - (\tkzcay))}}
\path[coordinate](\tkz@xx pt,\tkz@yy pt) coordinate (tkzRadialCenter);
\edef\tkz@hh{\tkz@Abs{(\tkzccx+\tkz@aa)*(\tkzccx-(\tkz@aa))}}
\edef\tkz@hh{\tkz@Dec{\tkz@Sqrt{\tkz@hh}}}
 \edef\tkz@rx{\tkz@Dec{\tkz@hh / \tkz@dd * (\tkzcay - (\tkzcby))}}
\edef\tkz@ry{\tkz@Dec{\tkz@hh / \tkz@dd * (\tkzcbx - (\tkzcax))}}
\edef\tkz@xs{\tkz@Dec{\tkz@xx + \tkz@rx}}
\edef\tkz@ys{\tkz@Dec{\tkz@yy + \tkz@ry}}
\path[coordinate](\tkz@xs pt,\tkz@ys pt) coordinate (#5);
\edef\tkz@xss{\tkz@Dec{\tkz@xx - \tkz@rx}}
\edef\tkz@yss{\tkz@Dec{\tkz@yy - \tkz@ry}}
\path[coordinate](\tkz@xss pt,\tkz@yss pt) coordinate (#6);
\endpgfinterruptboundingbox   
\endgroup
}
%<--------------------------------------------------------------------------–>
% #2 node #3 node #4 node #5 node
% \def\tkzInterCC(#1,#2)(#3,#4)#5#6{%
% \begingroup
%   \tkz@@CalcLength(#1,#2){tkz@rayA}
%   \tkz@@CalcLength(#3,#4){tkz@rayB}
%   \tkzInterCCR(#1,\tkz@rayA pt)(#3,\tkz@rayB pt){#5}{#6}
% \endgroup
% }  
%<--------------------------------------------------------------------------–>
%    Intersection de deux cercles   Avec deux points
%<--------------------------------------------------------------------------–>
% la première variante devrait être #2 #3  avec #4 #5
\def\tkzInterCCWithNodes(#1,#2,#3)(#4,#5,#6)#7#8{%
\begingroup
  \tkz@@CalcLengthcm(#2,#3){tkz@rayA}
  \tkz@@CalcLengthcm(#5,#6){tkz@rayB}
  \tkzInterCCR(#1,\tkz@rayA)(#4,\tkz@rayB){#7}{#8}
\endgroup
} 
\makeatother
\endinput

==> tikz-euclide/tools-lua/tkz-tools-lua-math.tex <==
% tkz-tools-lua-math.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-lua-math.tex}     
\makeatletter
%<-------------------------------------------------------------------------->
%<-------------------------------------------------------------------------->
%                           Lengths
%<-------------------------------------------------------------------------->
%<-------------------------------------------------------------------------->

\begin{luacode*} 
  function normalize(angleA,angleB)       
      if angleA > 0 then
       if angleA > angleB then
          angleA = angleA - 360
          end
      else
     if angleA > angleB then
          angleB = angleB + 360
        end
      end
      return angleA, angleB
  end
  
  function math.angle(x1, y1, x2, y2)
      local a = math.deg(math.atan(y2 - y1, x2 - x1))
      if a < 0 then
          return a + 360
      else
          return a
      end
  end
  
  function tkzop(...)
  inf = math.huge
  return ...
end
 
function tkzround(nb, ND)
  local p = 10^(ND or 0)
   return math.floor(nb * p + 0.5) / p
end   
\end{luacode*}

\def\tkz@Dec#1{%
     \directlua{tex.print(string.format('\@percentchar.6f',#1))}
     }
\def\tkz@Op#1{\directlua{tex.sprint(tostring(tkzop(#1)))}}
\def\tkz@Log#1{\directlua{tex.sprint(math.log(#1))}}
\def\tkz@Exp#1{\directlua{tex.sprint(math.exp(#1))}}
\def\tkz@Sqrt#1{\directlua{tex.sprint(math.sqrt(#1))}}
\def\tkz@Abs#1{\directlua{tex.sprint(math.abs(#1))}}
\def\tkz@Pi{\directlua{tex.sprint(math.pi)}}
\def\tkz@Cos#1{\directlua{tex.sprint(math.cos(#1))}}
\def\tkz@Sin#1{\directlua{tex.sprint(tostring(math.sin(#1)))}}
\def\tkz@Tan#1{\directlua{tex.sprint(math.tan(#1))}}
\def\tkz@Rad#1{\directlua{tex.sprint(math.rad(#1))}}
\def\tkz@Acos#1{\directlua{tex.sprint(math.acos(#1))}}
\def\tkz@Asin#1{\directlua{tex.sprint(math.asin(#1))}}
\def\tkz@Atan#1{\directlua{tex.sprint(math.atan(#1))}}
\def\tkz@Round#1#2{\directlua{tex.sprint(tostring(tkzround(#1,#2)))}}
\def\tkz@Angle#1#2#3#4{\directlua{tex.sprint(math.angle(#1,#2,#3,#4))}}
\def\tkz@Ceil#1{\directlua{tex.sprint(math.ceil(#1))}}
\def\tkz@Floor#1{\directlua{tex.sprint(math.floor(#1))}}
\def\tkz@Huge{\directlua{tex.sprint(math.huge)}}
\def\tkz@Max#1{\directlua{tex.sprint(math.max(#1))}}
\def\tkz@Min#1{\directlua{tex.sprint(math.min(#1))}}
\def\tkz@Random#1{\directlua{tex.sprint(math.random(#1))}}
\def\tkz@veclen#1#2{%
  \directlua{%
    tex.print(string.format('\@percentchar.6f',math.sqrt((#1)^2+(#2)^2)))%
  }%
}
\let\tkzSqrt\tkz@Sqrt
\let\tkzPi\tkz@Pi
\let\tkzExp\tkz@Exp
\let\tkzLog\tkz@Log
\let\tkzSin\tkz@Sin
\let\tkzCos\tkz@Cos

%  \tkzpointnormalised    normalise un point A-->A' tq ||v(OA')=1||
% example
% \tkzpointnormalised{%
% \pgfpointdiff{\pgfpointanchor{A}{center}}
%              {\pgfpointanchor{B}{center}}}

% or
% \pgf@x=1 cm
% \pgf@y=12 cm 
% \tkzpointnormalised{}
%<--------------------------------------------------------------------------
\def\tkzpointnormalised#1{%
\pgf@process{#1}%
\pgf@xa=\pgf@x%
\pgf@ya=\pgf@y%
\edef\tkz@temp@xa{\strip@pt\pgf@xa}%
\edef\tkz@temp@ya{\strip@pt\pgf@ya}%
\edef\tkz@den{\tkz@veclen{\tkz@temp@xa}{\tkz@temp@ya}}
\edef\tkz@coordx{\tkz@Op{\tkz@temp@xa/\tkz@den}}
\edef\tkz@coordx{\tkz@Dec{\tkz@Round{\tkz@coordx}{5}}}
\edef\tkz@coordy{\tkz@Op{\tkz@temp@ya/\tkz@den}}
\edef\tkz@coordy{\tkz@Dec{\tkz@Round{\tkz@coordy}{5}}}
\pgf@x = \tkz@coordx pt
\pgf@y = \tkz@coordy pt
}
%\def\tkz@Dec#1{\directlua{tex.print(string.format('\@percentchar.12f',#1))}}
%<-------------------------------------------------------------------------->
% restaure and save length
\def\tkz@save@length{\global\let\tkz@temp@length\tkzLengthResult}%
\def\tkz@restore@length{\global\let\tkzLengthResult\tkz@temp@length }% 
%<-------------------------------------------------------------------------->
%    \tkzCalcLength      Distance entre deux points en pt ou en cm  avec xfp 
% \veclen mais avec fp 
%  option cm le résultat est en cm sinon en pt with cm=false
%<-------------------------------------------------------------------------->
\pgfkeys{tkzcalclen/.cd,
       cm/.is if         = tkzLengthIncm,
       cm/.default       = true,
       cm                = true}   

\def\tkzCalcLength{\pgfutil@ifnextchar[{\tkz@CalcLength}{\tkz@CalcLength[]}}  
\def\tkz@CalcLength[#1](#2,#3){%
\pgfqkeys{/tkzcalclen}{#1}%   
\begingroup
\tkz@@CalcLength(#2,#3){tkzLengthResult}
\iftkzLengthIncm 
   \edef\tkz@xfpMathLen{\tkz@Dec{\tkz@Round{\tkzLengthResult/28.45274}{6}}}
   \global\let\tkzLengthResult\tkz@xfpMathLen  
\fi 
\endgroup
}%

\def\tkz@@CalcLength(#1,#2)#3{%
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\edef\tkz@xa{\strip@pt\pgf@x}%
\edef\tkz@ya{\strip@pt\pgf@y}%
\edef\tkz@xfpMathLen{\tkz@veclen{\tkz@xa}{\tkz@ya}}
\global\expandafter\edef\csname #3\endcsname{\tkz@xfpMathLen}
}

\def\tkz@@CalcLengthcm(#1,#2)#3{%
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\edef\tkz@xa{\strip@pt\pgf@x}%
\edef\tkz@ya{\strip@pt\pgf@y}%
\edef\tkz@xfpMathLen{\tkz@veclen{\tkz@xa}{\tkz@ya}}
\edef\tkz@xfpMathLen{\tkz@Dec{\tkz@Round{\tkz@xfpMathLen/28.45274}{6}}}
\global\expandafter\edef\csname #3\endcsname{\tkz@xfpMathLen}
}
\def\tkz@@CalcLengthb(#1,#2)#3{%
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\edef\tkz@xfpMathLen{\fpeval{sqrt((\pgf@x)^2+(\pgf@y)^2)}}
\edef\tkz@xfpMathLen{\fpeval{round(\tkz@xfpMathLen,6)}}
\global\expandafter\edef\csname #3\endcsname{\tkz@xfpMathLen}
}
%<-------------------------------------------------------------------------->
\def\tkzGetLength#1{%
\global\expandafter\edef\csname #1\endcsname{\tkzLengthResult}}  
%<-------------------------------------------------------------------------->
%     \tkzpttocm  passage de pt   cm div par 28.45274
%<-------------------------------------------------------------------------->
\def\tkzpttocm(#1)#2{%
\begingroup  
  \edef\tkz@mathresult{\tkz@Round{#1/28.45274}{6}}
 \global\expandafter\edef\csname #2\endcsname{\tkz@mathresult}%
\endgroup
}%
%<-------------------------------------------------------------------------->
%     \tkzcmtopt  passage de cm   pt mul par 28.45274
%<--------------------------------------------------------------------------
\def\tkzcmtopt(#1)#2{%
\begingroup 
  \edef\tkz@mathresult{\tkz@Round{#1*28.45274}{6}}
  \global\expandafter\edef\csname #2\endcsname{\tkz@mathresult}% 
\endgroup  
}% 
%<---------------------------------------------------------–>
 \def\tkzGetResult#1{%
   \global\expandafter\edef\csname #1\endcsname{\tkzMathResult}}
%<---------------------------------------------------------–>
%  Schrodinger's cat idea 03/01/20
\tikzset{veclen/.code={%
\pgfmathdeclarefunction*{veclen}{2}{%
\begingroup%
    \pgfmath@x##1pt\relax%
    \pgfmath@y##2pt\relax%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \edef\tkz@temp@xa{\strip@pt\pgf@xa}% 
    \edef\tkz@temp@ya{\strip@pt\pgf@ya}%
    \edef\tkz@xfpMathLen{\tkz@veclen{\tkz@temp@xa}{\tkz@temp@ya}}%
    \pgfmath@returnone\tkz@xfpMathLen pt%
\endgroup%
}}}%
%<---------------------------------------------------------–>
\def\tkzSwapPoints(#1,#2){
   \pgfnodealias{tkzPointTmp}{#2}
   \pgfnodealias{#2}{#1}
   \pgfnodealias{#1}{tkzPointTmp}}
%<---------------------------------------------------------–>
\def\tkzPermute(#1,#2,#3){
   \tkzURotateWithNodes(#1,#3,#2)(#3)  \tkzGetPoint{tkzpt}
   \tkzURotateWithNodes(#1,#2,#3)(#2)  \tkzGetPoint{#2}
   \tkzSwapPoints(tkzpt,#3)
}
%<---------------------------------------------------------–>
\def\tkzDotProduct(#1,#2,#3){%
\begingroup
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}% 
\edef\tkzax{\strip@pt\pgf@x}%
\edef\tkzay{\strip@pt\pgf@y}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}}% 
\edef\tkzbx{\strip@pt\pgf@x}%
\edef\tkzby{\strip@pt\pgf@y}%
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#3}{center}}% 
\edef\tkzcx{\strip@pt\pgf@x}%
\edef\tkzcy{\strip@pt\pgf@y}%
\edef\tkz@tmp{\tkz@Dec{\tkz@Round{((\tkzbx-(\tkzax))*(\tkzcx-(\tkzax))+(\tkzby-(\tkzay))*(\tkzcy-(\tkzay)))/809.55841}{6}}}
\global\let\tkzMathResult\tkz@tmp
\endgroup
}

% #1,#2 and #3 aligned
\def\tkzIsLinear(#1,#2,#3){%
\begingroup
\tkz@@CalcLengthcm(#1,#2){tkz@la}
\tkz@@CalcLengthcm(#1,#3){tkz@lb}
\tkzDotProduct(#1,#2,#3)
\edef\tkzResult{\tkz@Dec{\tkz@Abs{\tkzMathResult}-(\tkz@la)*(\tkz@lb)}}
\ifdim \tkzResult pt < 0.01 pt\relax%
\global\tkzLineartrue
\else
\global\tkzLinearfalse
\fi
\endgroup
}
%<---------------------------------------------------------–>
% syntax : vec(#2,#1) ortho vec(#3,#1)
\def\tkzIsOrtho(#1,#2,#3){%
\begingroup
\tkzDotProduct(#1,#2,#3)
\edef\tkzResult{\tkz@Dec{\tkz@Abs{\tkzMathResult}}}
\ifdim \tkzResult pt < 1 pt\relax%
\global\tkzOrthotrue
\else
\global\tkzOrthofalse
\fi
\endgroup
}
%<---------------------------------------------------------–>
% \tkzPowerCircle(M)(O,A) --> OM^2-OA^2
\def\tkzPowerCircle(#1)(#2,#3){%     
\begingroup 
\tkz@@CalcLengthcm(#2,#3){tkz@ra}
\tkz@@CalcLengthcm(#1,#2){tkz@om}
\gdef\tkzMathResult{\tkz@Dec{(\tkz@om)^2-(\tkz@ra)^2}}
\endgroup
}
%<---------------------------------------------------------–>
\def\tkzDefRadicalAxis(#1,#2)(#3,#4){%
\begingroup
\tkz@@CalcLengthcm(#1,#3){tkz@d}
\tkz@@CalcLengthcm(#1,#2){tkz@ra}
\tkz@@CalcLengthcm(#3,#4){tkz@rb}
\edef\tkzMathResult{\tkz@Dec{\tkz@d-(\tkz@ra+\tkz@rb)}}
\edef\tkzMathResultb{\tkz@Dec{\tkz@Abs{(\tkz@d-(\tkz@ra+\tkz@rb))}}}
\edef\tkzMathResultc{\tkz@Dec{\tkz@Abs{\tkz@d-\tkz@Abs{(\tkz@ra-(\tkz@rb))}}}}
\ifdim \tkzMathResultc pt < 0.1 pt\relax%
 \tkzURotateAngle(#2,90)(#3) \tkzGetPoint{tkzFirstPointResult}
  \tkzURotateAngle(#2,-90)(#3) \tkzGetPoint{tkzSecondPointResult}
\else
\ifdim \tkzMathResultb pt < 0.1 pt\relax%
 \tkzURotateAngle(#2,90)(#3) \tkzGetPoint{tkzFirstPointResult}
  \tkzURotateAngle(#2,-90)(#3) \tkzGetPoint{tkzSecondPointResult}
  \else
\ifdim \tkzMathResult pt > 1 pt\relax%
  \tkzURotateAngle(#1,60)(#3)    \tkzGetPoint{tkz@aux}
  \tkzInterCC(#1,#2)(tkz@aux,#1) \tkzGetPoints{tkz@pta}{tkz@ptb}
  \tkzInterCC(#3,#4)(tkz@aux,#1) \tkzGetPoints{tkz@ptc}{tkz@ptd}
  \tkzInterLL(tkz@pta,tkz@ptb)(tkz@ptc,tkz@ptd) \tkzGetPoint{tkz@pta}
  \tkzUProjection(#1,#3)(tkz@pta)  \tkzGetPoint{tkz@ptb}
  \pgfnodealias{tkzSecondPointResult}{tkz@ptb}
  \pgfnodealias{tkzFirstPointResult}{tkz@pta}
\else
\tkzInterCCR(#1,\tkz@ra)(#3,\tkz@rb){tkzFirstPointResult}{tkzSecondPointResult}
\fi
\fi
\fi
\endgroup
} 

\makeatother 
\endinput

==> tikz-euclide/tools/tkz-tools-eu-BB.tex <==
% tkz-tools-eu-BB.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c  tkz-obj-eu-BB.tex}  
\makeatletter
%<--------------------------------------------------------------------------–>
\def\tkzShowBB{\pgfutil@ifnextchar[{\tkz@ShowBB}{\tkz@ShowBB[]}} 
\def\tkz@ShowBB[#1]{%
 \draw[#1]  (current bounding box.south west) rectangle 
            (current bounding box.north east);
}
%<--------------------------------------------------------------------------–>
\def\tkzClipBB{%
\clip   (current bounding box.south west) rectangle 
        (current bounding box.north east);
}
%<--------------------------------------------------------------------------–>
\makeatother
\endinput

==> tikz-euclide/tools/tkz-tools-eu-angles.tex <==
% tkz-tools-angles.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-angles.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% thanks karu : http://tex.stackexchange.com/questions/151667/tkzgetangle-strange-behavior/196224#196224  
% \tkzGetAngle strange behavior
% defines \tkz@FirstAngle and \tkz@SecondAngle sens  trigo
%<--------------------------------------------------------------------------–>
\def\tkzNormalizeAngle(#1,#2){%
\begingroup
\pgfmathparse{#1}\xdef\tkz@FirstAngle{\pgfmathresult}%
\pgfmathparse{#2}\xdef\tkz@SecondAngle{\pgfmathresult}%
\pgfmathgreaterthan{\tkz@FirstAngle}{0}
\ifdim\pgfmathresult pt=1 pt\relax%
  \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
  \ifdim\pgfmathresult pt=1 pt\relax%
    \pgfmathsubtract{\tkz@FirstAngle}{360}
    \xdef\tkz@FirstAngle{\pgfmathresult}%
  \fi
\else
  \pgfmathgreaterthan{\tkz@FirstAngle}{\tkz@SecondAngle}
  \ifdim\pgfmathresult pt=1 pt\relax%
    \pgfmathadd{\tkz@SecondAngle}{360}
    \xdef\tkz@SecondAngle{\pgfmathresult}%
  \fi
\fi
 \endgroup
 }  
%<--------------------------------------------------------------------------–>
%                          Angle 
% Recherche l'angle formé par #1 et #2 par rapport à l'horizontale
%<--------------------------------------------------------------------------–>
\def\tkzFindSlopeAngle(#1,#2){%
\begingroup
  \pgfmathanglebetweenpoints{\pgfpointanchor{#1}{center}}{%
                             \pgfpointanchor{#2}{center}} 
  \global\let\tkzAngleResult\pgfmathresult  
\endgroup
}
%<--------------------------------------------------------------------------–>
%                          Angle  avec trois nodes
%<--------------------------------------------------------------------------–>
\def\tkzFindAngle(#1,#2,#3){% new code 2016
\begingroup
    \tkzFindSlopeAngle(#2,#1)\tkzGetAngle{tkz@FirstAngle}
    \tkzFindSlopeAngle(#2,#3)\tkzGetAngle{tkz@SecondAngle}
    \tkzNormalizeAngle(\tkz@FirstAngle,\tkz@SecondAngle)
    \edef\tkz@Angle{\fpeval{\tkz@SecondAngle-\tkz@FirstAngle}}
    \global\let\tkzAngleResult\tkz@Angle
\endgroup
}

%<--------------------------------------------------------------------------–>
% Find angle
%<--------------------------------------------------------------------------–>
\def\tkzGetAngle#1{%
  \global\expandafter\edef\csname #1\endcsname{\tkzAngleResult}
}  
\makeatother
\endinput

==> tikz-euclide/tools/tkz-tools-eu-base.tex <==
% tkz-tools-eu-base.tex    
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”. 
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-base.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
\global\let\tkz@tmp@xa\tkz@init@xmin% modif  2016
\global\let\tkz@tmp@xb\tkz@init@xmax% modif  2016
\global\let\tkz@tmp@ya\tkz@init@ymin% modif  2016
\global\let\tkz@tmp@yb\tkz@init@ymax% modif  2016 
%<--------------------------------------------------------------------------–>
\pgfkeys{
         /tkzInit/.cd,
         xmin/.store in     = \tkz@init@xmin,
         xmax/.store in     = \tkz@init@xmax,
         xstep/.store in    = \tkz@init@xstep,
         ymin/.store in     = \tkz@init@ymin,
         ymax/.store in     = \tkz@init@ymax,
         ystep/.store in    = \tkz@init@ystep, 
         NO/.is if          = tkz@init@NO,
         NO/.default        = true, 
         xmin               = 0,
         xmax               = 10,
         xstep              = 1,
         ymin               = 0,
         ymax               = 10,
         ystep              = 1,
         NO                 = false 
         } 
  
\def\tkzInit{\pgfutil@ifnextchar[{\tkz@Init}{\tkz@Init[]}} 
\def\tkz@Init[#1]{%
    \pgfqkeys{/tkzInit}{#1}
  \ifx\tkzfctloaded\undefined
    \else   
      \tkz@tkzf@fct=0 %  only if tkz-fct loaded
   \fi   
  \xdef\tkz@init@xorigine{0}
  \xdef\tkz@init@yorigine{0}
  \edef\@xsgmin{\fpeval{sign(\tkz@init@xmin)}} % -> -1 or 1
  \edef\@xsgmax{\fpeval{sign(\tkz@init@xmax)}}
  \edef\@ysgmin{\fpeval{sign(\tkz@init@ymin)}}
  \edef\@ysgmax{\fpeval{sign(\tkz@init@ymax)}}
  \let\tkz@tmp@xa\tkz@init@xmin %modif 2016
  \let\tkz@tmp@xb\tkz@init@xmax %modif 2016
  \let\tkz@tmp@ya\tkz@init@ymin %modif 2016
  \let\tkz@tmp@yb\tkz@init@ymax %modif 2016
  \tkz@init@NOfalse                   
  \ifx\@xsgmin\@xsgmax \tkz@init@NOtrue \fi
  \ifx\@ysgmin\@ysgmax \tkz@init@NOtrue \fi
  \iftkz@init@NO%
  \ifx\@xsgmin\@xsgmax
      \edef\tkz@init@xmax{\fpeval{\tkz@init@xmax-\tkz@init@xmin}}
      \edef\tkz@init@xorigine{\tkz@init@xmin}
      \edef\tkz@init@xmin{0}
  \fi
  \ifx\@ysgmin\@ysgmax
      \edef\tkz@init@ymax{\fpeval{\tkz@init@ymax-\tkz@init@ymin}}
      \edef\tkz@init@yorigine{\tkz@init@ymin}
      \edef\tkz@init@ymin{0}
  \fi
  \fi
  \edef\tkz@xa{\fpeval{\tkz@init@xmin/\tkz@init@xstep}}
  \edef\tkz@xb{\fpeval{\tkz@init@xmax/\tkz@init@xstep}}
  \edef\tkz@ya{\fpeval{\tkz@init@ymin/\tkz@init@ystep}}
  \edef\tkz@yb{\fpeval{\tkz@init@ymax/\tkz@init@ystep}}
  \tkz@getdecimal{\tkz@init@xstep} % amélioration nb dec et integer
  \xdef\tkz@init@xdec{\number\c@pgfmath@countb}
  \tkz@getdecimal{\tkz@init@ystep}
  \xdef\tkz@init@ydec{\number\c@pgfmath@countb}
}%
\def\tkzAddName{\pgfutil@ifnextchar[{\tkz@AddName}{\tkz@AddName[]}} 
\def\tkz@AddName[#1]#2{%
\node[above left,#1] at (\pgf@path@lastx,\pgf@path@lasty){#2};  
}% 
%<--------------------------------------------------------------------------–>
\makeatother 
\endinput

==> tikz-euclide/tools/tkz-tools-eu-colors.tex <==
% tkz-tools-eu-colors
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c  tkz-tools-eu-colors}  
\makeatletter

%<------  Initialisation of the colors with tkzSetUpColors  -----------------> 
% Première macro SetUpColors %%%%%%%%%%%%%%%%%%%%%
%Possible
\pgfkeys{/tkzsucolor/.is family}
\def\setupcolorkeys#1{%
   \pgfkeys{/tkzsucolor,#1}}
\setupcolorkeys{
   background/.estore in   =  \setupcolor@background,
   text/.estore in         =  \setupcolor@text,
   @initial/.style         =  {background=white,text=black},
   @apply/.code            =  {\pagecolor{\setupcolor@background}%
                                    \color{\setupcolor@text}%
 },
}
\def\tkzSetUpColors{\pgfutil@ifnextchar[{\tkz@SetUpColors}{\tkz@SetUpColors[]}}
\def\tkz@SetUpColors[#1]{\setupcolorkeys{@initial,#1,@apply}}

%<------  Initialisation of all colors   -----------------> 
\pgfkeys{/tkzsupallcol/.cd,
         background/.store in       = \tkz@suac@bkc,
         text/.store in             = \tkz@suac@txt,
         background                 = \tkz@backgroundcolor,% see tkz-euclide.cfg
         text                       = \tkz@textcolor% idem
        } 
\def\tkzSetUpAllColors{\pgfutil@ifnextchar[{\tkz@SetUpAllColors}{%
                                 \tkz@SetUpAllColors[]}} 
\def\tkz@SetUpAllColors[#1]{%
   \pgfqkeys{/tkzsupallcol}{#1} % now we redine the based colors
   \def\tkz@fillcolor{\tkz@suac@bkc}   
   \def\tkz@mainlinecolor{\tkz@suac@txt}
   \def\tkz@textcolor{\tkz@suac@txt}
   \def\tkz@otherlinecolor{\tkz@suac@txt!50}
   \def\tkz@sua@color{\tkz@suac@txt} 
   \tkzSetUpAxis[color=\tkz@suac@txt]
   \tkzSetUpGrid[color=\tkz@suac@txt]      
   \pagecolor{\tkz@suac@bkc}
   \color{\tkz@suac@txt}  
}
\makeatother
\endinput

==> tikz-euclide/tools/tkz-tools-eu-intersections.tex <==
% tkz-tools-intersections.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status “maintained”.
% 
% The Current Maintainer of this work is Alain Matthes.
%  utf8 encoding

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-intersections.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%                 intersection  de deux lignes
%<--------------------------------------------------------------------------–>
\def\tkzInterLL(#1,#2)(#3,#4){% méthode avec xfp
\tkz@InterLL(#1,#2)(#3,#4){tkzPointResult}
}

\def\tkz@InterLL(#1,#2)(#3,#4)#5{%
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}%
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}}
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#3}{center}}%
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#4}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#4}{center}}%
\tkz@dx\pgf@x%
\tkz@dy\pgf@y%
\edef\tkz@deltax{\fpeval{(\tkz@ax-\tkz@bx)/(28.45274)}}
\edef\tkz@deltaxx{\fpeval{(\tkz@cx-\tkz@dx)/(28.45274)}}
\edef\tkz@deltay{\fpeval{(\tkz@ay-\tkz@by)/(28.45274)}}
\edef\tkz@deltayy{\fpeval{(\tkz@cy-\tkz@dy)/(28.45274)}}
\edef\tkz@deltaxy{\fpeval{((\tkz@ax*\tkz@by)-(\tkz@ay*\tkz@bx))/(809.55841)}}
\edef\tkz@deltaxxyy{\fpeval{((\tkz@cx*\tkz@dy)-(\tkz@cy*\tkz@dx))/(809.55841)}}
\edef\tkz@div{\fpeval{(\tkz@deltax*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxx)}}
\edef\tkz@numx{\fpeval{(\tkz@deltaxy*\tkz@deltaxx)-(\tkz@deltax*\tkz@deltaxxyy)}}
\edef\tkz@numy{\fpeval{(\tkz@deltaxy*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxxyy)}}
\edef\tkz@xs{\fpeval{round(\tkz@numx/\tkz@div,5)}}
\edef\tkz@ys{\fpeval{round(\tkz@numy/\tkz@div,5)}}
\path[coordinate](\tkz@xs,\tkz@ys) coordinate (#5);
}


% méthode with coordinates
\def\tkzInterLLxy(#1,#2,#3,#4)(#5,#6,#7,#8){%
%\path (intersection of #1--#2 and #3--#4) coordinate(#5);%
\tkz@ax#1%
\tkz@ay#2%
\tkz@bx#3%
\tkz@by#4%
\tkz@cx#5%
\tkz@cy#6%
\tkz@dx#7%
\tkz@dy#8%
\edef\tkz@deltax{\fpeval{(\tkz@ax-\tkz@bx)/(28.45274)}}
\edef\tkz@deltaxx{\fpeval{(\tkz@cx-\tkz@dx)/(28.45274)}}
\edef\tkz@deltay{\fpeval{(\tkz@ay-\tkz@by)/(28.45274)}}
\edef\tkz@deltayy{\fpeval{(\tkz@cy-\tkz@dy)/(28.45274)}}
\edef\tkz@deltaxy{\fpeval{((\tkz@ax*\tkz@by)-(\tkz@ay*\tkz@bx))/(809.55841)}}
\edef\tkz@deltaxxyy{\fpeval{((\tkz@cx*\tkz@dy)-(\tkz@cy*\tkz@dx))/(809.55841)}}
\edef\tkz@div{\fpeval{(\tkz@deltax*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxx)}}
\edef\tkz@numx{\fpeval{(\tkz@deltaxy*\tkz@deltaxx)-(\tkz@deltax*\tkz@deltaxxyy)}}
\edef\tkz@numy{\fpeval{(\tkz@deltaxy*\tkz@deltayy)-(\tkz@deltay*\tkz@deltaxxyy)}}
\edef\tkz@xs{\fpeval{round(\tkz@numx/\tkz@div,5)}}
\edef\tkz@ys{\fpeval{round(\tkz@numy/\tkz@div,5)}}
\path[coordinate](\tkz@xs,\tkz@ys) coordinate (tkzPointResult);
}

%<--------------------------------------------------------------------------–>
%                 intersection  de Ligne Cercle rayon connu
%<--------------------------------------------------------------------------–>
% /*
%    Calculate the intersection of a ray and a sphere
%    The line segment is defined from p1 to p2
%    The sphere is of radius r and centered at sc
%    There are potentially two points of intersection given by
%    p = p1 + mu1 (p2 - p1)
%    p = p1 + mu2 (p2 - p1)
%    Return FALSE if the ray doesn't intersect the sphere.
% */
% int RaySphere(XYZ p1,XYZ p2,XYZ sc,double r,double *mu1,double *mu2)
% {
%    double a,b,c;
%    double bb4ac;
%    XYZ dp;
% 
%    dp.x = p2.x - p1.x;
%    dp.y = p2.y - p1.y;
%    dp.z = p2.z - p1.z;
%    a = dp.x * dp.x + dp.y * dp.y + dp.z * dp.z;
%    b = 2 * (dp.x * (p1.x - sc.x) + dp.y * (p1.y - sc.y) + dp.z * (p1.z - sc.z));
%    c = sc.x * sc.x + sc.y * sc.y + sc.z * sc.z;
%    c += p1.x * p1.x + p1.y * p1.y + p1.z * p1.z;
%    c -= 2 * (sc.x * p1.x + sc.y * p1.y + sc.z * p1.z);
%    c -= r * r;
%    bb4ac = b * b - 4 * a * c;
%    if (ABS(a) < EPS || bb4ac < 0) {
%       *mu1 = 0;
%       *mu2 = 0;
%       return(FALSE);
%    }
% 
%    *mu1 = (-b + sqrt(bb4ac)) / (2 * a);
%    *mu2 = (-b - sqrt(bb4ac)) / (2 * a);
% 
%    return(TRUE);
% }
%<---------- test ------------------------------------------------------–>
\def\tkzTestInterLC(#1,#2)(#3,#4){%
\begingroup
\tkz@Projection(#1,#2)(#3){tkz@pth}% distance centre à la ligne
\tkz@@CalcLength(#3,tkz@pth){tkz@mathLen}%  
\tkz@@CalcLength(#3,#4){tkzLengthResult}%calcul du rayon
\ifdim\tkz@mathLen pt>\tkzLengthResult pt\relax%
\global\tkzFlagLCfalse
\else
\global\tkzFlagLCtrue
\fi
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkz@numlc{0}
\pgfkeys{/linecircle/.cd,
  node/.code               = \def\tkz@numlc{0},
  R/.code                  = \def\tkz@numlc{1}, 
  with nodes/.code         = \def\tkz@numlc{2},
  common/.store in         = \tkz@common,
  common                   = {},
  near/.is if              =  tkz@near,
  near/.default            =  true,
  near                     =  false,
  next to/.store in        = \tkz@nextto,
  next to/.initial         = {},
  next/.default            = {},
  next to                  = {},
  next to/.value required,
  node  
 }
%<--------------------------------------------------------------------------–>
\def\tkzInterLC{\pgfutil@ifnextchar[{\tkz@InterLC}{\tkz@InterLC[]}}
\def\tkz@InterLC[#1](#2,#3)(#4,#5){%
\begingroup      
\pgfqkeys{/linecircle}{#1}
 \pgfinterruptboundingbox 
\ifcase\tkz@numlc%
    % first case 0
  \tkz@@CalcLength(#4,#5){tkzLengthResult}
  \tkzInterLCR(#2,#3)(#4,\tkzLengthResult pt){tkzFirstPointResult}%
                         {tkzSecondPointResult}
\or% 1
    \tkzInterLCR(#2,#3)(#4,#5 cm){tkzFirstPointResult}
                   {tkzSecondPointResult}%  
\or% 2
    \tkzInterLCWithNodes(#2,#3)(#4,#5){tkzFirstPointResult}%
                        {tkzSecondPointResult}% 
\fi
\iftkz@near
  \tkz@@CalcLength(#2,tkzFirstPointResult){tkzLengthFirst}
  \tkz@@CalcLength(#2,tkzSecondPointResult){tkzLengthSecond}
      \ifdim \tkzLengthFirst pt < \tkzLengthSecond pt\relax%
      \else
       \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
       \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
       \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
      \fi
\else
    \ifx\tkz@common\tkzutil@empty 
      \ifx\tkz@nextto\tkzutil@empty 
         \tkzFindAngle(tkzSecondPointResult,tkzFirstPointResult,#4)   
         \tkzGetAngle{tkz@an}
          \ifdim\tkz@an pt<180 pt\relax%
          \else
           \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
           \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
           \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
          \fi
      \else
         \tkz@@CalcLength(\tkz@nextto,tkzFirstPointResult){tkzLengthFirst}
         \tkz@@CalcLength(\tkz@nextto,tkzSecondPointResult){tkzLengthSecond}
             \ifdim \tkzLengthFirst pt < \tkzLengthSecond pt\relax%
             \else
              \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
              \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
              \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
             \fi
       \fi
    \else 
         \tkz@@CalcLength(\tkz@common,tkzSecondPointResult){tkz@mathLen}
         \ifdim\tkz@mathLen pt<1pt\relax%
         \else
          \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
          \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
          \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
         \fi
     \fi
\fi%near
\endpgfinterruptboundingbox    
\endgroup
}
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzInterLCR(#1,#2)(#3,#4)#5#6{%
\begingroup
\tkz@radi=#4%
\tkz@@extractxy{#3}
\tkz@bx =\pgf@x\relax%
\tkz@by =\pgf@y\relax%
\tkz@Projection(#1,#2)(#3){tkz@pth}
\tkz@@CalcLength(#3,tkz@pth){tkz@mathLen}
 \ifdim\tkz@mathLen pt<0.05pt\relax%
        \pgfpointdiff{\pgfpointanchor{#1}{center}}%
                     {\pgfpointanchor{#2}{center}}%
        \tkz@ax=\pgf@x%
        \tkz@ay=\pgf@y%
        \pgfpointborderellipse{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                              {\pgfpoint{\tkz@radi}{\tkz@radi}}
        \tkz@ax=\pgf@x\relax%
        \tkz@ay=\pgf@y\relax%
        \advance\tkz@bx by\tkz@ax\relax%
        \advance\tkz@by by\tkz@ay\relax%
        \pgfcoordinate{#6}{\pgfqpoint{\tkz@bx}{\tkz@by}}
        \tkzCSym(#3)(#6){#5} 
  \else  
       \edef\pgfmathresult{\fpeval{\tkz@mathLen/\tkz@radi}} 
      % \edef\tkz@angle{\fpeval{acosd(\pgfmathresult)}}
        \pgfmathacos@{\pgfmathresult}%
        \let\tkz@angle\pgfmathresult%
        \pgfpointdiff{\pgfpointanchor{#3}{center}}%
                     {\pgfpointanchor{tkz@pth}{center}}%
        \tkz@ax=\pgf@x%
        \tkz@ay=\pgf@y%  
        \pgfpointborderellipse{\pgfpoint{\tkz@ax}{\tkz@ay}}%
                              {\pgfpoint{\tkz@radi}{\tkz@radi}}
        \tkz@ax =\pgf@x\relax%
        \tkz@ay =\pgf@y\relax%
        \advance\tkz@bx by\tkz@ax\relax%
        \advance\tkz@by by\tkz@ay\relax%
        \tkz@@extractxy{#3}
        \tkz@ax =\pgf@x\relax%
        \tkz@ay =\pgf@y\relax%
        \tkz@@extractxy{tkz@pth}
        \pgfmathrotatepointaround{\pgfpoint{\tkz@bx}{\tkz@by}}%
                                 {\pgfpoint{\tkz@ax}{\tkz@ay}}%
                                 {\tkz@angle}
         \pgfcoordinate{#5}{\pgfqpoint{\pgf@x}{\pgf@y}}
        \pgfmathrotatepointaround{\pgfpoint{\tkz@bx}{\tkz@by}}%
                                 {\pgfpoint{\tkz@ax}{\tkz@ay}}%
                                 {-\tkz@angle}
  \pgfcoordinate{#6}{\pgfqpoint{\pgf@x}{\pgf@y}}

\fi        
\endgroup
}
%<--------------------------------------------------------------------------–>
%                 intersection  de Ligne Cercle 
% #4 center #5 point sur le cercle
%<--------------------------------------------------------------------------–>
% \def\tkzInterLC(#1,#2)(#3,#4)#5#6{%
%     \begingroup
%     \tkz@@CalcLength(#3,#4){tkz@rad}
%     \tkzInterLCR(#1,#2)(#3,\tkz@rad pt){#5}{#6}
% \endgroup
% } 
%<--------------------------------------------------------------------------–>
%                 intersection  de Ligne Cercle rayon inconnu
%<--------------------------------------------------------------------------–>
\def\tkzInterLCWithNodes(#1,#2)(#3,#4,#5)#6#7{%
\begingroup
    \tkz@@CalcLength(#4,#5){tkz@radius}
    \tkzInterLCR(#1,#2)(#3,\tkz@radius pt){#6}{#7}
\endgroup
}
%<--------------------------------------------------------------------------–>
%  Intersection of 2 circles
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% méthode
% /* circle_circle_intersection() *
%  * Determine the points where 2 circles in a common plane intersect.
%  *
%  * int circle_circle_intersection(
%  *                                // center and radius of 1st circle
%  *                                double x0, double y0, double r0,
%  *                                // center and radius of 2nd circle
%  *                                double x1, double y1, double r1,
%  *                                // 1st intersection point      
%  *                                // 2nd intersection point
%  *
%  * This is a public domain work. 3/26/2005 Tim Voght
%  *
% int circle_circle_intersection(double x0, double y0, double r0,
%                                double x1, double y1, double r1,
%                                double *xi, double *yi,
%                                double *xi_prime, double *yi_prime)
% {
%   double a, dx, dy, d, h, rx, ry;
%   double x2, y2;
% 
%   /* dx and dy are the vertical and horizontal distances between
%    * the circle centers.
%    */
%   dx = x1 - x0;
%   dy = y1 - y0;
% 
%   /* Determine the straight-line distance between the centers. */
%   //d = sqrt((dy*dy) + (dx*dx));
%   d = hypot(dx,dy); // Suggested by Keith Briggs
% 
%   /* Check for solvability. */
%   if (d > (r0 + r1))
%   {
%     /* no solution. circles do not intersect. */
%     return 0;
%   }
%   if (d < fabs(r0 - r1))
%   {
%     /* no solution. one circle is contained in the other */
%     return 0;
%   }
% 
%   /* 'point 2' is the point where the line through the circle
%    * intersection points crosses the line between the circle
%    * centers.  
%    */
% 
%   /* Determine the distance from point 0 to point 2. */
%   a = ((r0*r0) - (r1*r1) + (d*d)) / (2.0 * d) ;
% 
%   /* Determine the coordinates of point 2. */
%   x2 = x0 + (dx * a/d);
%   y2 = y0 + (dy * a/d);
% 
%   /* Determine the distance from point 2 to either of the
%    * intersection points.
%    */
%   h = sqrt((r0*r0) - (a*a));
% 
%   /* Now determine the offsets of the intersection points from
%    * point 2.
%    */
%   rx = -dy * (h/d);
%   ry = dx * (h/d);
% 
%   /* Determine the absolute intersection points. */
%   *xi = x2 + rx;
%   *xi_prime = x2 - rx;
%   *yi = y2 + ry;
%   *yi_prime = y2 - ry;
% 
%   return 1;
% } 
%<--------------------------------------------------------------------------–>
%    Intersection de deux cercles  
%<--------------------------------------------------------------------------–>
%<---------- test ------------------------------------------------------–>
% test avec des nodes  R-r <= d <= R+r
\def\tkzTestInterCC(#1,#2)(#3,#4){%
\begingroup
\tkz@@CalcLength(#1,#3){tkz@mathLen}% distance entre les centres  
\tkz@@CalcLength(#2,#1){tkz@rA}%calcul du rayon
\tkz@@CalcLength(#4,#3){tkz@rB}%calcul du rayon
% test if d <= rA + rB ?
\edef\tkz@rS{\fpeval{\tkz@rA+\tkz@rB}}
\ifdim\tkz@mathLen pt > \tkz@rS pt\relax%
\global\tkzFlagCCfalse
\else
% now test if d>= rA - rB or rB-rA
  \ifdim \tkz@rA pt >  \tkz@rB pt\relax%
       \edef\tkz@rD{\fpeval{\tkz@rA-\tkz@rB}}
   \else
       \edef\tkz@rD{\fpeval{\tkz@rB-\tkz@rA}}
   \fi
\ifdim  \tkz@rD pt > \tkz@mathLen pt\relax%
 \global\tkzFlagCCfalse
\else
\global\tkzFlagCCtrue
\fi
\fi
\endgroup
}

\def\tkz@numcc{0}
\pgfkeys{
/circlecircle/.cd,
  node/.code           = \def\tkz@numcc{0},
  R/.code              = \def\tkz@numcc{1},
  with nodes/.code     = \def\tkz@numcc{2},
  common/.store in     = \tkz@common,
  common               = {},
  node
}
%<--------------------------------------------------------------------------–>
\def\tkzInterCC{\pgfutil@ifnextchar[{\tkz@InterCC}{\tkz@InterCC[]}}
\def\tkz@InterCC[#1](#2,#3)(#4,#5){%
\begingroup      
\pgfqkeys{/circlecircle}{#1}
\ifcase\tkz@numcc%
 % first case 0 
  \tkz@save@length 
  \tkz@@CalcLengthcm(#2,#3){tkz@rayA}
  \tkz@@CalcLengthcm(#4,#5){tkz@rayB}
  \tkz@restore@length     
  \tkzInterCCR(#2,\tkz@rayA)(#4,\tkz@rayB){tkzFirstPointResult}{tkzSecondPointResult}  
  \or% 1
 \tkzInterCCR(#2,#3)(#4,#5){tkzFirstPointResult}{tkzSecondPointResult}%
  \or%2
 \tkzInterCCWithNodes(#2,#3)(#4,#5){tkzFirstPointResult}{tkzSecondPointResult}    
\fi 
 \ifx\tkz@common\tkzutil@empty 
 \tkzFindAngle(#2,tkzFirstPointResult,#4)   \tkzGetAngle{tkz@an}
 \ifdim\tkz@an pt<180 pt\relax%
 \else
 \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
  \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
 \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
 \fi
 \else
\tkz@@CalcLength(\tkz@common,tkzSecondPointResult){tkz@mathLen}
 \ifdim\tkz@mathLen pt<0.05pt\relax%
 \else
  \pgfnodealias{tkzPointTmp}{tkzSecondPointResult}
   \pgfnodealias{tkzSecondPointResult}{tkzFirstPointResult}
  \pgfnodealias{tkzFirstPointResult}{tkzPointTmp}
  \fi
  \fi
\endgroup
} 
%<--------------------------------------------------------------------------–>

\def\tkzInterCCR(#1,#2)(#3,#4)#5#6{%
\begingroup
\pgfinterruptboundingbox  
\tkz@save@length  
\tkz@@CalcLength(#1,#3){tkz@dd}
\tkz@restore@length 
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}} 
\tkz@ax\pgf@x %
\tkz@ay\pgf@y %
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#3}{center}} 
\tkz@bx\pgf@x %
\tkz@by\pgf@y %
\tkz@cx#2cm %
\tkz@cy#4cm %
\edef\tkz@aa{\fpeval{((\tkz@cx+\tkz@cy)/(2*\tkz@dd))*(\tkz@cx-\tkz@cy)+\tkz@dd/2}}
 \edef\tkz@xx{\fpeval{\tkz@ax+\tkz@aa/\tkz@dd*(\tkz@bx - \tkz@ax)}}
\edef\tkz@yy{\fpeval{\tkz@ay+\tkz@aa/\tkz@dd*(\tkz@by - \tkz@ay)}} 
\path[coordinate](\tkz@xx pt,\tkz@yy pt) coordinate (tkzRadialCenter);
\edef\tkz@hh{\fpeval{sqrt(abs((\tkz@cx+\tkz@aa)*(\tkz@cx-\tkz@aa)))}}% abs !2023
\edef\tkz@rx{\fpeval{\tkz@hh / \tkz@dd * (\tkz@ay - \tkz@by)}}
\edef\tkz@ry{\fpeval{\tkz@hh / \tkz@dd * (\tkz@bx - \tkz@ax)}}
\edef\tkz@xs{\fpeval{\tkz@xx + \tkz@rx}}
\edef\tkz@ys{\fpeval{\tkz@yy + \tkz@ry}}
\path[coordinate](\tkz@xs pt,\tkz@ys pt) coordinate (#5);
\edef\tkz@xss{\fpeval{\tkz@xx - \tkz@rx}}
\edef\tkz@yss{\fpeval{\tkz@yy - \tkz@ry}}
\path[coordinate](\tkz@xss pt,\tkz@yss pt) coordinate (#6); 
\endpgfinterruptboundingbox   
\endgroup
}
%<--------------------------------------------------------------------------–>
% #2 node #3 node #4 node #5 node
% \def\tkzInterCC(#1,#2)(#3,#4)#5#6{%
% \begingroup
%   \tkz@@CalcLength(#1,#2){tkz@rayA}
%   \tkz@@CalcLength(#3,#4){tkz@rayB}
%   \tkzInterCCR(#1,\tkz@rayA pt)(#3,\tkz@rayB pt){#5}{#6}
% \endgroup
% }  
%<--------------------------------------------------------------------------–>
%    Intersection de deux cercles   Avec deux points
%<--------------------------------------------------------------------------–>
% la première variante devrait être #2 #3  avec #4 #5
\def\tkzInterCCWithNodes(#1,#2,#3)(#4,#5,#6)#7#8{%
\begingroup
  \tkz@@CalcLengthcm(#2,#3){tkz@rayA}
  \tkz@@CalcLengthcm(#5,#6){tkz@rayB}
  \tkzInterCCR(#1,\tkz@rayA)(#4,\tkz@rayB){#7}{#8}
\endgroup
} 
\makeatother
\endinput

==> tikz-euclide/tools/tkz-tools-eu-math.tex <==
% tkz-tools-eu-math.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-math.tex}     
\makeatletter
%<-------------------------------------------------------------------------->
% \tkzpointnormalised#
% tkzCalcLength
% \tkzGetLength
% \tkzpttocm
% \tkzcmtopt
% \tkzFindSlope
% option xfp

%  \tkzpointnormalised    normalise un point A-->A' tq ||v(OA')=1||
% Ã©quivalent de \pgfpointnormalised avec fp
% example
% \tkzpointnormalised{%
% \pgfpointdiff{\pgfpointanchor{A}{center}}
%              {\pgfpointanchor{B}{center}}}

% or
% \pgf@x=1 cm
% \pgf@y=12 cm 
% \tkzpointnormalised{}
%<--------------------------------------------------------------------------
\def\tkzpointnormalised#1{%
\pgf@process{#1}%
\edef\tkz@den{\fpeval{sqrt((\pgf@x)^2+(\pgf@y)^2)}}
\edef\tkz@coordx{\fpeval{\pgf@x/\tkz@den}}
\edef\tkz@coordx{\fpeval{round(\tkz@coordx,5)}}
\edef\tkz@coordy{\fpeval{\pgf@y/\tkz@den}}
\edef\tkz@coordy{\fpeval{round(\tkz@coordy,5)}}
\pgf@x = \tkz@coordx pt
\pgf@y = \tkz@coordy pt
}
%<-------------------------------------------------------------------------->
% restaure and save length
\def\tkz@save@length{\global\let\tkz@temp@length\tkzLengthResult}%
\def\tkz@restore@length{\global\let\tkzLengthResult\tkz@temp@length }% 
%<-------------------------------------------------------------------------->
%    \tkzCalcLength      Distance entre deux points en pt ou en cm  avec xfp 
% \veclen mais avec fp 
%  option cm le résultat est en cm sinon en pt with cm=false
%<-------------------------------------------------------------------------->
\pgfkeys{tkzcalclen/.cd,
       cm/.is if         = tkzLengthIncm,
       cm/.default       = true,
       cm                = true}   

\def\tkzCalcLength{\pgfutil@ifnextchar[{\tkz@CalcLength}{\tkz@CalcLength[]}}  
\def\tkz@CalcLength[#1](#2,#3){%
%\pgfkeys{tkzcalclen/.cd, cm = true}
\pgfqkeys{/tkzcalclen}{#1}%   
\begingroup
\tkz@@CalcLength(#2,#3){tkzLengthResult}
\iftkzLengthIncm 
   \pgfmathparse{\tkzLengthResult pt/1cm}
   \edef\tkz@xfpMathLen{\fpeval{round(\pgfmathresult,6)}}
   \global\let\tkzLengthResult\tkz@xfpMathLen  
\fi 
\endgroup
}%
\def\tkz@@CalcLength(#1,#2)#3{%
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\edef\tkz@xfpMathLen{\fpeval{sqrt((\pgf@x)^2+(\pgf@y)^2)}}
\edef\tkz@xfpMathLen{\fpeval{round(\tkz@xfpMathLen,6)}}
\global\expandafter\edef\csname #3\endcsname{\tkz@xfpMathLen}
}
\def\tkz@@CalcLengthcm(#1,#2)#3{%
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\edef\tkz@xfpMathLen{\fpeval{sqrt((\pgf@x)^2+(\pgf@y)^2)}}
\edef\tkz@xfpMathLen{\fpeval{round(\tkz@xfpMathLen/28.45274,6)}}
\global\expandafter\edef\csname #3\endcsname{\tkz@xfpMathLen}
}
%<-------------------------------------------------------------------------->
\def\tkzGetLength#1{%
\global\expandafter\edef\csname #1\endcsname{\tkzLengthResult}}  
%<-------------------------------------------------------------------------->
%     \tkzpttocm  passage de pt   cm div par 28.45274
%<-------------------------------------------------------------------------->
\def\tkzpttocm(#1)#2{%
\begingroup  
  \pgfmathparse{#1/1cm}
  \edef\tkz@mathresult{\fpeval{round(\pgfmathresult,5)}}
  \global\let\tkz@mathresult\tkz@mathresult
  \global\expandafter\edef\csname #2\endcsname{\tkz@mathresult}% 
\endgroup
}%
%<-------------------------------------------------------------------------->
%     \tkzcmtopt  passage de cm   pt mul par 28.45274
%<--------------------------------------------------------------------------
\def\tkzcmtopt(#1)#2{%
\begingroup 
   \pgfmathparse{#1*1cm}
  \edef\tkz@mathresult{\fpeval{round(\pgfmathresult,5)}}
  \global\let\tkz@mathresult\tkz@mathresult
  \global\expandafter\edef\csname #2\endcsname{\tkz@mathresult}% 
\endgroup  
}% 

%  Schrodinger's cat idea 03/01/20
\tikzset{veclen/.code={%
\pgfmathdeclarefunction*{veclen}{2}{%
\begingroup%
    \pgfmath@x##1pt\relax%
    \pgfmath@y##2pt\relax%
    \edef\tkz@xfpMathLen{\fpeval{sqrt((\pgf@x)^2+(\pgf@y)^2)}}   
    \pgfmath@returnone\tkz@xfpMathLen pt%
\endgroup%
}}}%
%<---------------------------------------------------------–>
\def\tkzSwapPoints(#1,#2){
  \pgfnodealias{tkzPointTmp}{#2}
   \pgfnodealias{#2}{#1}
  \pgfnodealias{#1}{tkzPointTmp}}
%<---------------------------------------------------------–>
\def\tkzPermute(#1,#2,#3){
\tkzURotateWithNodes(#1,#3,#2)(#3)  \tkzGetPoint{tkzpt}
\tkzURotateWithNodes(#1,#2,#3)(#2) \tkzGetPoint{#2}
\tkzSwapPoints(tkzpt,#3)}
%<---------------------------------------------------------–>
\def\tkzDotProduct(#1,#2,#3){%
\begingroup
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}% 
\tkz@ax\pgf@x%
\tkz@ay\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#2}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#2}{center}} 
\tkz@bx\pgf@x%
\tkz@by\pgf@y%
\pgfextractx{\pgf@x}{\pgfpointanchor{#3}{center}}%
\pgfextracty{\pgf@y}{\pgfpointanchor{#3}{center}}% 
\tkz@cx\pgf@x%
\tkz@cy\pgf@y%
\edef\tkz@@dotprod{\fpeval{round(((\tkz@bx-\tkz@ax)*(\tkz@cx-\tkz@ax)+(\tkz@by-\tkz@ay)*(\tkz@cy-\tkz@ay))/(809.55841),5)}}
\global\let\tkzMathResult\tkz@@dotprod
\endgroup}
%<---------------------------------------------------------–>
 \def\tkzGetResult#1{%
   \global\expandafter\edef\csname #1\endcsname{\tkzMathResult}}
%<---------------------------------------------------------–>
% #1,#2 and #3 aligned
\def\tkzIsLinear(#1,#2,#3){%
\begingroup
\tkz@@CalcLengthcm(#1,#2){tkz@la}
\tkz@@CalcLengthcm(#1,#3){tkz@lb}
\tkzDotProduct(#1,#2,#3)
\edef\tkzResult{\fpeval{abs(\tkzMathResult)-(\tkz@la)*(\tkz@lb)}}
\ifdim \tkzResult pt < 0.01 pt\relax%
\global\tkzLineartrue
\else
\global\tkzLinearfalse
\fi
\endgroup
}
%<---------------------------------------------------------–>
% syntax : vec(#2,#1) ortho vec(#3,#1)
\def\tkzIsOrtho(#1,#2,#3){%
\begingroup
\tkzDotProduct(#1,#2,#3)
\edef\tkzResult{\fpeval{abs(\tkzMathResult)}}
\ifdim \tkzResult pt < 1 pt\relax%
\global\tkzOrthotrue
\else
\global\tkzOrthofalse
\fi
\endgroup
}
%<---------------------------------------------------------–>
%<---------------------------------------------------------–>
% \tkzPowerCircle(M)(O,A) --> OM^2-OA^2
\def\tkzPowerCircle(#1)(#2,#3){%     
\begingroup 
\tkz@@CalcLengthcm(#2,#3){tkz@ra}
\tkz@@CalcLengthcm(#1,#2){tkz@om}
\gdef\tkzMathResult{\fpeval{round(\tkz@om*\tkz@om -\tkz@ra*\tkz@ra,5)}}
\endgroup
}
%<---------------------------------------------------------–>
\def\tkzDefRadicalAxis(#1,#2)(#3,#4){%
\begingroup
\tkz@@CalcLengthcm(#1,#3){tkz@d}
\tkz@@CalcLengthcm(#1,#2){tkz@ra}
\tkz@@CalcLengthcm(#3,#4){tkz@rb}
\edef\tkzMathResult{\fpeval{\tkz@d-(\tkz@ra+\tkz@rb)}}
\edef\tkzMathResultb{\fpeval{abs(\tkz@d-(\tkz@ra+\tkz@rb))}}
\edef\tkzMathResultc{\fpeval{abs(\tkz@d-abs(\tkz@ra-\tkz@rb))}}
\ifdim \tkzMathResultc pt < 0.1 pt\relax%
 \tkzURotateAngle(#2,90)(#3) \tkzGetPoint{tkzFirstPointResult}
  \tkzURotateAngle(#2,-90)(#3) \tkzGetPoint{tkzSecondPointResult}
\else
\ifdim \tkzMathResultb pt < 0.1 pt\relax%
 \tkzURotateAngle(#2,90)(#3) \tkzGetPoint{tkzFirstPointResult}
  \tkzURotateAngle(#2,-90)(#3) \tkzGetPoint{tkzSecondPointResult}
  \else
\ifdim \tkzMathResult pt > 1 pt\relax%
  \tkzURotateAngle(#1,60)(#3)    \tkzGetPoint{tkz@aux}
  \tkzInterCC(#1,#2)(tkz@aux,#1) \tkzGetPoints{tkz@pta}{tkz@ptb}
  \tkzInterCC(#3,#4)(tkz@aux,#1) \tkzGetPoints{tkz@ptc}{tkz@ptd}
  \tkzInterLL(tkz@pta,tkz@ptb)(tkz@ptc,tkz@ptd) \tkzGetPoint{tkz@pta}
  \tkzUProjection(#1,#3)(tkz@pta)  \tkzGetPoint{tkz@ptb}
  \pgfnodealias{tkzSecondPointResult}{tkz@ptb}
  \pgfnodealias{tkzFirstPointResult}{tkz@pta}
\else
\tkzInterCCR(#1,\tkz@ra)(#3,\tkz@rb){tkzFirstPointResult}{tkzSecondPointResult}
\fi
\fi
\fi
\endgroup
} 
\def\tkzmathrotatepointaround#1#2#3{%
  \pgf@process{%
    \pgf@process{#1}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@process{#2}%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    \pgf@x=\pgf@xc%
    \pgf@y=\pgf@yc%
    \advance\pgf@x-\pgf@xa%
    \advance\pgf@y-\pgf@ya%
    \pgfmathsetmacro\angle{#3}%
    \mathSin{\mathRad{\angle}}%
    \let\sineangle\pgfmathresult%
    \mathCos{\mathRad{\angle}}%
    \let\cosineangle\pgfmathresult%
    \pgf@xa\cosineangle\pgf@x%
    \advance\pgf@xa-\sineangle\pgf@y%
    \pgf@ya\sineangle\pgf@x%
    \advance\pgf@ya\cosineangle\pgf@y%
    \pgf@x\pgf@xb%
    \pgf@y\pgf@yb%
    \advance\pgf@x\pgf@xa%
    \advance\pgf@y\pgf@ya%
  }%
}
\makeatother 
\endinput

==> tikz-euclide/tools/tkz-tools-eu-modules.tex <==
% tkz-tools-modules
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-utilities.tex}  
\makeatletter
%<------------- % chargement des modules ---------------------------------->
\def\tkz@obj@all{angles,arcs,compass,defcircles,deflines,defpoints,defpointsby,defpointsrnd,defpointswith,polygons,protractor,sectors,show,triangles}%
\def\tkz@obj@txt{all}
\def\usetkzobj{\pgfutil@ifnextchar[{\use@usetkzobj}{\use@@usetkzobj}}%}
\def\use@usetkzobj[#1]{\use@@usetkzobj{#1}}
\def\use@@usetkzobj#1{% 
  \def\tkz@list{#1}
  \ifx\tkz@obj@txt\tkz@list \edef\tkz@list{\tkz@obj@all}% 
      \else  
      \edef\tkz@list{#1}%
    \fi
  \pgfutil@for\tkz@temp:=\tkz@list\do{%
    \expandafter\ifx\csname tkz@library@\tkz@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tkz@library@\tkz@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tkz@obj@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tkz@obj@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12   
      \input tkz-obj-\tkz@temp.tex 
      \catcode`\@=\csname tkz@obj@#1@atcode\endcsname
      \catcode`\|=\csname tkz@obj@#1@barcode\endcsname  
    \fi%
  }%
}%
%<---------------------------------------------------------–>
\def\tkz@tool@all{math-xfp}
\def\tkz@tool@txt{all}

\def\usetkztool{\pgfutil@ifnextchar[{\use@usetkztool}{\use@@usetkztool}}%}
\def\use@usetkztool[#1]{\use@@usetkztool{#1}}
\def\use@@usetkztool#1{% 
  \def\tkz@list{#1}
  \ifx\tkz@tool@txt\tkz@list \edef\tkz@list{\tkz@tool@all}%
      \else
      \edef\tkz@list{#1}%
    \fi
  \pgfutil@for\tkz@temp:=\tkz@list\do{%
    \expandafter\ifx\csname tkz@library@\tkz@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tkz@library@\tkz@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tkz@tool@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tkz@tool@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \input tkz-tools-\tkz@temp.tex
      \catcode`\@=\csname tkz@tool@#1@atcode\endcsname
      \catcode`\|=\csname tkz@tool@#1@barcode\endcsname
    \fi%
  }%
}%
\makeatother
\endinput

==> tikz-euclide/tools/tkz-tools-eu-text.tex <==
% tkz-tools-eu-text.tex
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c tkz-tools-eu-text.tex}   
\makeatletter
%<--------------------------------------------------------------------------–>
%                                         tkzText
%<--------------------------------------------------------------------------–>
\def\tkz@parsenode#1{%
\tkz@getvirg#1,\@nil
\iftkz@node  
\else
  \tkz@getfromcart#1\@nil   
\fi  
}   
\def\tkz@getvirg#1,#2\@nil{%
\ifx\tkzempty#2\tkzempty%
   \tkz@nodetrue 
\else
   \tkz@nodefalse  
\fi
}      
\def\tkzText{\pgfutil@ifnextchar[{\tkz@Text}{\tkz@Text[]}}
\def\tkz@Text[#1](#2)#3{%
 \begingroup
    \tkz@parsenode{#2} 
 \iftkz@node 
   \node[#1] at (#2){#3}; 
 \else
  \edef\tkzpt@xa{\fpeval{(\tkz@absc-\tkz@init@xorigine)/\tkz@init@xstep}}
  \edef\tkzpt@ya{\fpeval{(\tkz@ord-\tkz@init@yorigine)/\tkz@init@ystep}}
  \node[#1] at (\tkzpt@xa,\tkzpt@ya){#3};% 
  \fi
\endgroup
}%
% %<--------------------------------------------------------------------------–>
% %                                    légende
% %<--------------------------------------------------------------------------–>
\pgfkeys{/tkzlegend/.cd,  
   line/.is if                 =    tkz@legend@line,
   line/.default               =    true,
   line                        =    false,
   /tkzlegend/.search also     =    {/tikz}, 
}
\def\tkzLegend{\pgfutil@ifnextchar[{\tkz@Legend}{\tkz@Legend[]}} 
\def\tkz@Legend[#1](#2,#3)#4{%
\pgfqkeys{/tkzlegend}{#1}
\begingroup  
  \c@pgfmath@counta=0 %
  \edef\tkzpt@xa{\fpeval{(#2-\tkz@init@xorigine)/\tkz@init@xstep}}
  \edef\tkzpt@ya{\fpeval{(#3-\tkz@init@yorigine)/\tkz@init@ystep}}
  \node[/tkzlegend/.cd,#1] at (\tkzpt@xa,\tkzpt@ya) {%
\begin{tikzpicture}
   \foreach \motif/\size/\col/\mtext in {#4}{%
       \iftkz@legend@line
          \draw[color      = \col,
                line width = \size,
                style      = \motif,
                text       = \tkz@mainlinecolor]%
          (0cm ,\the\c@pgfmath@counta ex)--%
               (\tkz@legend@line@len,\the\c@pgfmath@counta ex) 
       \else  
          \draw plot[mark size    = \size,%
                     mark         = \motif,%
                     mark options = {color=\col}]%
           coordinates{(0 ex,\the\c@pgfmath@counta ex)}%
         \fi
           node[right=1ex] {\mtext};
          \global\advance\c@pgfmath@counta by 3 %  
       }% 

\end{tikzpicture}%
};% 
\endgroup
}   
\makeatother
\endinput

==> tikz-euclide/tools/tkz-tools-eu-utilities.tex <==
% tkz-tools-eu-utilities
% Copyright 2023  Alain Matthes
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% This work has the LPPL maintenance status “maintained”.
% The Current Maintainer of this work is Alain Matthes.

\def\fileversion{5.02c}
\def\filedate{2023/02/03} 
\typeout{2023/02/03 5.02c  tkz-tools-eu-utilities.tex}  
\makeatletter
\pgfkeys{/tkzClip/.cd, 
space/.store in    = {\tkz@CLI@space},
space    = {}} 

\def\tkzClip{\pgfutil@ifnextchar[{\tkz@Clip}{\tkz@Clip[]}} 
\def\tkz@Clip[#1]{%

\pgfqkeys{/tkzClip}{#1} 
\ifx\tkzutil@empty\tkz@CLI@space
    \clip (\tkz@xa,\tkz@ya) rectangle (\tkz@xb,\tkz@yb);
 \else
 \edef\tkz@xxa{\fpeval{\tkz@xa-\tkz@CLI@space}}
 \edef\tkz@yya{\fpeval{\tkz@ya-\tkz@CLI@space}}
 \edef\tkz@xxb{\fpeval{\tkz@xb+\tkz@CLI@space}} % correction bug 2020
 \edef\tkz@yyb{\fpeval{\tkz@yb+\tkz@CLI@space}}
 \clip (\tkz@xxa,\tkz@yya) rectangle (\tkz@xxb,\tkz@yyb);
\fi
} 

% for testing results
\def\extractxy#1{%
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}
} 
%<-------------- some tools -------------------------------------------------> 
\def\tkzutil@empty{}
\def\tkzutil@firstofone#1{#1}
\def\tkzutil@firstoftwo#1#2{#1}
\def\tkzutil@secondoftwo#1#2{#2}
%<--------------------------------------------------------------------------–>
\long\def\tkzutil@ifundefined#1{%
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\tkzutil@firstoftwo
  \else
    \expandafter\tkzutil@secondoftwo
  \fi} 
%<--------------------------------------------------------------------------–>
\long\def\iftkznodedefined#1#2#3{%
    \tkzutil@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%<--------------------------------------------------------------------------–>
\gdef\tkzActivOff{%
   \edef\tkzTwoPtCode{\the\catcode`\:} 
   \edef\tkzPtExCode{\the\catcode`\!} 
   \edef\tkzPtVirCode{\the\catcode`\;} 
   \catcode`\:=12 \catcode`\!=12 \catcode`\;=12
   }%
\gdef\tkzActivOn{%
   \catcode`\:=\tkzTwoPtCode\relax
   \catcode`\!=\tkzPtExCode\relax
   \catcode`\;=\tkzPtVirCode\relax
}% 
%<--------------------------------------------------------------------------–>
%              Pour savoir le nombre de décimales d'un nombre
% le nombre dans #1 et le résultat dans \c@pgfmath@countb
%<--------------------------------------------------------------------------–>
\newcommand\tkz@getdecimal[1]{\expandafter\@getdecimal#1.\@nil}
\def\@getdecimal#1.#2\@nil{%
  \ifx\empty#2\empty
    % Si #2 est vide, c'est qu'il n'y avait pas de point
    % dans la chaîne initiale
    \c@pgfmath@countb0 %
   \gdef\tkz@decpart{}%
  \else
    % sinon c'est la chaîne qui suit le point décimal...
    \CountToken{#2}%
    % ... y compris le point en trop ajouté par \tkz@getdecimal  :-)
    \advance\c@pgfmath@countb by-1 %
    \@@getdecimal#2\@nil
  \fi
}
\def\@@getdecimal#1.\@nil{\gdef\tkz@decpart{#1}}
%<---------------------------------------------------------–>
% code from JCC modifi
\newcommand\CountToken[1]{%
 \c@pgfmath@countb0 %
  \expandafter\C@untToken#1\@nil
%modifi ajout du expandafter
}
\newcommand\C@untToken{%
  \afterassignment\C@untT@ken\let\CurrT@ken=
}
\newcommand\C@untT@ken{%
 \ifx\CurrT@ken\@nil \else
   \advance\c@pgfmath@countb by1 %
   \expandafter\C@untToken
 \fi
}
%<---------------------------------------------------------–>
\def\tkz@recuplast(#1,#2){\def\tkz@last{#1}}
\def\tkz@stop{\tkz@stop}
% end code from JCC    
%<---------------------------------------------------------–>
%            Tools
%<---------------------------------------------------------–>
%<–––––––– code from TeX in Practice ––––––––>
\def\SubStringConditional #1#2{%
    TT\fi
    \edef\@MainString{#1}%
    \edef\@SubStringConditionalTemp{{#1}{#2}}%
    \expandafter\@SubStringConditional\@SubStringConditionalTemp
}
\def\@SubStringConditional #1#2{% 
    \def\@TestSubS ##1#2##2\\{% 
        \def\@TestTemp{##1}% 
    }% 
    \@TestSubS #1#2\\
    \ifx\@MainString\@TestTemp
        \tkz@TestSubStringfalse
    \else
        \tkz@TestSubStringtrue
    \fi
    \iftkz@TestSubString
}
\def\RecursionMacroEnd #1#2#3{% 
    #1\relax
        \def\@RecursionMacroEndNext{#2}% 
    \else
        \def\@RecursionMacroEndNext{#3}% 
    \fi
    \@RecursionMacroEndNext
}
\def\ReplaceSubStrings #1#2#3#4{%
    \def\@ReplaceResult{#1}%
    \edef\@ReplaceMain{#2}%
    \edef\@ReplaceSub{#3}%
    \edef\@ReplaceSubRep{#4}%
    \@ReplaceSubStrings
}
\def\@ReplaceSubStrings{% 
    \RecursionMacroEnd
        {\if\SubStringConditional{\@ReplaceMain}{\@ReplaceSub}}%
      {\@ReplaceSubStringsDo}{\expandafter\edef\@ReplaceResult{\@ReplaceMain}}%
}
\def\@ReplaceSubStringsDoX{%
    \def\@ReplaceSubStringsDoA ##1%
}%
\def\@ReplaceSubStringsDo{% 
    \expandafter\@ReplaceSubStringsDoX \@ReplaceSub
                                    ##2\@EndReplaceSubStrings{%
        \edef\@ReplaceMain{##1\@ReplaceSubRep ##2}%
    }%
    \expandafter\@ReplaceSubStringsDoA\@ReplaceMain
        \@EndReplaceSubStrings
    \@ReplaceSubStrings
}
%<---------------------------------------------------------–>
\def\DisabledNumprint{%
      \let\tkz@numprint\numprint
      \let\numprint\relax
      }
\def\EnabledNumprint{\let\numprint\tkz@numprint} 
%<---------------------------------------------------------–>

%<---------------------------------------------------------–>
  \def\tkzHelpGrid{%
   \draw[help lines] (current bounding box.south west) grid
          (current bounding box.north east);
  }
   
\makeatother
\endinput
